Which Invariance Should We Transfer? A Causal Minimax Learning Approach

A major barrier to deploying current machine learning models lies in their non-reliability to dataset shifts. To resolve this problem, most existing studies attempted to transfer stable information to unseen environments. Particularly, independent causal mechanisms-based methods proposed to remove mutable causal mechanisms via the do-operator. Compared to previous methods, the obtained stable predictors are more effective in identifying stable information. However, a key question remains: which subset of this whole stable information should the model transfer, in order to achieve optimal generalization ability? To answer this question, we present a comprehensive minimax analysis from a causal perspective. Specifically, we first provide a graphical condition for the whole stable set to be optimal. When this condition fails, we surprisingly find with an example that this whole stable set, although can fully exploit stable information, is not the optimal one to transfer. To identify the optimal subset under this case, we propose to estimate the worst-case risk with a novel optimization scheme over the intervention functions on mutable causal mechanisms. We then propose an efficient algorithm to search for the subset with minimal worst-case risk, based on a newly defined equivalence relation between stable subsets. Compared to the exponential cost of exhaustively searching over all subsets, our searching strategy enjoys a polynomial complexity. The effectiveness and efficiency of our methods are demonstrated on synthetic data and the diagnosis of Alzheimer's disease.

==> icml23_paras/background_xw_v3.tex <==
\section{Preliminaries and background} 
\label{sec.background}

\textbf{Problem setup \& Notations.} We consider the supervised regression scenario, where the system includes a target variable $Y \!\in\! \mathcal{Y}$, covariates $\mathbf{X}\!:=\! [X_1,...,X_d] \!\in\! \mathcal{X}$, and data collected from heterogeneous environments. In practice, different ``environments" can refer to different groups of subjects or different experimental settings. We denote the set of training environments as $\mathcal{E}_{\mathrm{tr}}$, and the broader set of environments for deployment as $\mathcal{E}$. We denote $E$ as the environmental indicator variable with support $\mathcal{E}$. Our data are collected from multiple training environments $\{\mathcal{D}_{e}\}_{e\in\mathcal{E}_{\text{tr}}}$, where ${\mathcal{D}_{e}\!:=\!\{(\boldsymbol{x}_{k}^e, {y}_{k}^e)\}_{k=1}^{n_e} \sim_{i.i.d} P^e(\mathbf{X},Y)}$ are data collected from environment $e$. In a directed acyclic graph (DAG) $G$, we denote the parents, children, neighbors, and descendants of the vertex $V_i$ as $\mathbf{Pa}(V_i)$, $\mathbf{Ch}(V_i)$, $\mathbf{Neig}(V_i)$, and $\mathbf{De}(V_i)$, respectively. We denote $G_{\overline{V_i}}$ as the graph attained via deleting all arrows pointing into $V_i$. % Define $\mathrm{deg}(V_i)$ as the degree of $V_i$. 


Our goal is to find the most robust predictor $f^*$ among stable predictors with data from $\mathcal{E}_{\mathrm{tr}}$. Here, we say a predictor $f \!:\! \mathcal{X} \to \mathcal{Y}$ is stable if it is independent of $E$. We denote the set of stable predictors as $\mathcal{F}_S$. For robustness, a commonly adopted measurement \cite{peters2016causal,ahuja2021invariance} is to investigate a predictor's worst-case risk, which provides a safeguard for deployment in unseen environments. That is, we want $f^*$ to have the following minimax property:
\begin{align}
    f^{*}(\boldsymbol{x})=\mathop{\mathrm{argmin}}\limits_{f \in \mathcal{F}_S}        \max_{e\in\mathcal{E}}
    \mathbb{E}_{P^e}[(Y-f(\boldsymbol{x}))^2].
\label{eq.robust}
\end{align}
Next, we introduce some basic assumptions, which are commonly made in causal inference and learning \cite{pearl2009causality,spirtes2000causation,arjovsky2019invariant}.
\begin{assumption}[Structural causal model]
\label{eq:assum-dag}
We assume that $P^e(\mathbf{X},Y)$ is entailed by an \emph{unknown} DAG $G$ over $\mathbf{V}$ for all $e \in \mathcal{E}$, where $\mathbf{V}:= \mathbf{X} \cup Y$. Each variable $V_i \in \mathbf{V}$ is generated via a structural equation $V_i=g^e_{i}(\mathbf{Pa}({V_i}), U_i)$, where $U_i$ denotes an exogenous variable. We assume  
each $g^e_{i}$ is continuous and bounded. Each edge $V_i \to V_j$ in $G$ means $V_i$ is a direct causal of $V_j$. Besides, we assume the model is Markovian which states that $\mathbf{A} \ind_G \mathbf{B} | \mathbf{Z} \Rightarrow \mathbf{A} \ind \mathbf{B} | \mathbf{Z}$ for disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, where $\ind_G$ denotes \emph{d}-separation in $G$. 
\end{assumption}

According to the Causal Markov Condition theorem \cite{pearl2009causality}, the joint distribution can be causally factorized into $P^e(\mathbf{V})=\prod_i P^e(V_i|\mathbf{Pa}(V_i)))$, where $P^e(V_i|\mathbf{Pa}(V_i)))$ denotes the causal factor of $V_i$. Based on the principle of independent causal mechanisms \cite{scholkopf2021toward}, these causal factors are autonomous of each other. On the basis of this, the interventional distribution is defined as $P(\mathbf{V}|do(V_i\!=\!v_i)):=\prod_{j \neq i} P^e(V_j|\mathbf{Pa}(V_j)))\mathbbm{1}_{V_i=v_i}$. Here $do(V_i\!=\!v_i)$ means lifting $V_i$ from its original causal mechanism $g_{i}(\mathbf{Pa}({V_i}), U_i)$ and setting it to a constant value $v_i$. 

In addition to the Markovian assumption, we also assume the causal faithfulness assumption, which enables us to infer the graph structure from probability properties:

\begin{assumption}[Causal faithfulness]
\label{asm:faithfulness}
    For disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, $\mathbf{A} \ind \mathbf{B} | \mathbf{Z} \Rightarrow \mathbf{A} \ind_G \mathbf{B} | \mathbf{Z}$. 
\end{assumption}


\textbf{Sparse mechanism shift hypothesis across $\mathcal{E}$.} To build the connection between seen and unseen environments for transfer, we adopt the \emph{sparse mechanism shift hypothesis} \cite{scholkopf2021toward}, \emph{i.e.}, distributional shifts in $P^e(\mathbf{X},Y)$ are the results of changes in only a subset of causal factors. Formally, 
\begin{align}
\label{eq: causal factorization}
    & P^e(\mathbf{X},Y) = P(Y|\mathbf{Pa}(Y)) \prod_{i \in S} P\left(X_i|\mathbf{Pa}(X_i)\right) \nonumber \\
    & \prod_{i \in M} P^e(X_i|\mathbf{Pa}(X_i)), d_S:=|S|, d_M:=|M|,
\end{align}
where $S, M$ respectively denote stable and mutable sets such that each $X_i \in \mathbf{X}_S$ has invariant causal mechanism $P(X_i|\mathbf{Pa}(X_i))$; while the mechanism of each $X_i \in \mathbf{X}_M$ varies across $\mathcal{E}$. Correspondingly, we call $\mathbf{X}_S$ as stable variables and $\mathbf{X}_M$ as mutable variables. In addition to $\mathbf{X}_S$, we also assume the causal mechanism of $Y$ keeps invariant across $\mathcal{E}$, as widely adopted by the existing literature \cite{arjovsky2019invariant,sun2021recovering,mitrovic2021representation}.


To recover the $\mathbf{X}_M$ from the training distribution, it is also necessary to assume that $\mathcal{E}_{\mathrm{tr}}$ can reflect the mutation of $\mathbf{X}_M$ across $\mathcal{E}$. This is formally stated as follows:
\begin{assumption}[Consistent heterogeneity]
\label{assum:e-train}
For each $X_i \in \mathbf{X}_M$, there exists two different environments $e, e^\prime \in \mathcal{E}_{\mathrm{tr}}$ such that $P^{e}(X_i|\mathbf{Pa}(X_i)) \neq P^{e^\prime}(X_i|\mathbf{Pa}(X_i))$.
\end{assumption}


\textbf{Surgery estimator.} The surgery estimator \citep{subbaswamy2019preventing} proposed to remove the mutation in $P^e(\mathbf{X},Y)$ by intervening on $\mathbf{X}_M$ and obtained a set of stable predictors $\mathcal{F}_S:=\{f_{S^\prime}(\boldsymbol{x})|S^\prime\!\subseteq \!{S}\}, f_{S^\prime}(\boldsymbol{x})\!:=\!\mathbb{E}[Y|\boldsymbol{x}_{S^\prime}, do(\boldsymbol{x}_M)]$ over the interventional distribution. In this regard, identifying the minimax optimal predictor in Eq.~\ref{eq.robust} is equivalent to selecting the optimal subset $S^*$ such that $f_{S^*}=f^*$. 


To identify $S^*$, they first proved that the whole stable set $S$ is optimal under the \emph{degeneration condition}: the interventional distribution $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution  $P(Y|\mathbf{X}^\prime)$ for some $\mathbf{X}^\prime \subseteq \mathbf{X}$. However, they did not provide an approach to \textbf{test this condition}, limiting the utility of the theory. In practice, they compared each subset $S^\prime \subseteq S$ and selected the $S^*$ as the one with minimal loss on a held-out validation set. This method \textbf{lacks} a theoretical guarantee. Indeed, we observe from Fig. \ref{fig:adni-intro} that the selected subset is not optimal, because the validation loss does not necessarily reflect the worst-case risk over deployed environments. In the subsequent section, we propose to remedy the above problems of the surgery estimator, by considering the following questions: \textbf{i)} \emph{can we test the degeneration condition, or some of its equivalent conditions, in order to determine whether $S^* = S$?} \textbf{ii)} \emph{can we identify the optimal subset with theoretical guarantees under general scenarios?}



==> icml23_paras/introduction.tex <==
\vspace{-0.7cm}
\section{Introduction}
\vspace{-0.1cm}

Current machine learning systems, which are commonly deployed based on their in-distribution performance, often encounter \emph{dataset shifts} \cite{subbaswamy2019preventing} such as covariate shift, due to changes in the data generating process. When such a shift exists in deployment environments, the model may give unreliable prediction results, which can cause severe consequences in safe-critical tasks such as healthcare \citep{hendrycks2021many}. At the heart of this unreliability issue are \emph{stability} and \emph{robustness} aspects, which respectively denote the insensitivity of prediction behavior and generalization errors to dataset shifts. 

For example, consider the system deployed to predict the Functional Activities Questionnaire (FAQ) score that is commonly adopted \cite{mayo2016use} to measure the severity of Alzheimer's disease (AD). During the prediction, the system can only access biomarkers or volumes of brain regions as covariates, with demographic information anonymous for privacy consideration. However, the changes in such demographics can cause shifts in covariates. To achieve reliability for the deployed model, its prediction is desired to be stable against demographic changes, and meanwhile to be constantly accurate across all populations. For this purpose, this paper aims to find the most robust (\emph{i.e.}, minimax optimal) predictor, among the set of stable predictors across all deployed environments. 

To achieve this goal, many studies attempted to learn invariance to transfer to unseen data. Examples include ICP \cite{peters2016causal} and  \citep{arjovsky2019invariant, liu2021heterogeneous, ahuja2021invariance} that assumed the prediction mechanism given causal features or representations to be invariant; or Anchor regression \cite{rothenhausler2021anchor} that explicitly attributed the variation to exogenous variables. Particularly, \cite{subbaswamy2019preventing,subbaswamy2020spec} causally decomposed the joint distribution into the mutable ($M$) set and the stable ($S$) set, which contains variables with changed and unchanged causal mechanisms, respectively. By intervening on $M$, they can obtain a set of stable predictors, each of which is based on a stable subset in $S$. To further find the most robust predictor, the following question remains: \emph{which subset of $S$ should the model transfer, in order to be most robust against dataset shifts?} In \cite{subbaswamy2019preventing}, this optimal subset is simply taken as the one with the minimal validation loss, which lacks theoretical guarantees as the validation environment may not reflect the worst-case risk over deployed environments, as shown by Fig.~\ref{fig:adni-intro} (b). 


\begin{figure*}
\centering
\includegraphics[width=0.76\textwidth]{icml23_figs2/ad_results.png}
\caption{FAQ prediction in Alzheimer's disease. (a) Comparison of maximal mean square error (max. MSE) over deployed environments. (b) Max. MSE of subsets that are ranked in ascending order from left to right, respectively according to the estimated worst-case risk of our method (marked by red) and the validation loss of the surgery estimator \cite{subbaswamy2019preventing} (marked by blue). }
\vspace{-0.2cm}
\label{fig:adni-intro}
\end{figure*}


In this paper, we give a more comprehensive answer from the perspective of structural causal models. Specifically, we first provide a graphical condition that is sufficient for the whole stable set to be optimal. This condition can be easily tested via causal discovery. When this condition fails, we construct an example that counter-intuitively shows that this whole stable set, although keeps all stable information, is \textbf{NOT} the optimal one to transfer. Under these cases,
we investigate the mutable mechanisms and propose to optimize the intervention on the mutable set, in order to mimic the worst-case deployed environment. We show that such an optimization-based approach can attain the worst-case risk for each stable subset, which is crucial to select the optimal subset in a more accurate way. Back to the FAQ prediction example, Fig.~\ref{fig:adni-intro} (b) shows that our method is more reflective of the maximal mean squared error (max. MSE) than \cite{subbaswamy2019preventing}, which explains our advantage in predicting FAQ across patient groups shown in Fig.~\ref{fig:adni-intro} (a). 

To efficiently search for the optimal subset, we define an equivalence relation between stable subsets via $d$-separation such that two equivalent subsets share the same worst-case risk. We theoretically show that compared to exhaustive searching over all subsets, searching over only equivalence classes can reduce the exponential complexity to the polynomial complexity. The effectiveness and efficiency of our methods are demonstrated by improved robustness, stability, and computation efficiency achieved on a synthetic dataset and the diagnosis of Alzheimer's disease. 

\textbf{Contributions.} We summarize our contributions as follows: 
\begin{enumerate}[noitemsep,topsep=0.1pt]
    \item We propose to identify the optimal subset of invariance to transfer, guided by a comprehensive minimax analysis from a causal perspective. To the best of our knowledge, this is the \emph{first} work to comprehensively study the problem of \emph{which invariance should we transfer}, in the literature of robust learning. 
    \item We define an equivalence relation between stable subsets, and accordingly propose to search over only equivalence classes. This new search algorithm can be efficiently solved in polynomial time. 
    \item We achieve better robustness and stability than others on synthetic data and Alzheimer's disease diagnosis. 
\end{enumerate}




==> icml23_paras/minimax.tex <==
\section{Minimax analysis for the optimal subset}
\label{sec.identify}

In this section, we provide a comprehensive minimax analysis to resolve the problems of the surgery estimator. First, we provide a graphical condition for the whole stable set to be optimal, \emph{i.e.}, $S^* = S$. Compared to the degeneration condition, our condition enjoys a better intuition from the perspective of graph structure, thus facilitating an easy approach for testing via causal discovery. Second, when this condition is not met, we propose an optimization scheme that is provable to identify the worst-case risk for each subset, equipped with which we can pick up the $S^*$ as the one with minimal worst-case risk. 

In the following, we first introduce the graphical condition for $S^*=S$, which is equivalent to the degeneration condition, as summarized in Thm.~\ref{thm:graph degenerate}. 


\begin{theorem}[Graphical condition for $S^*\!=\!S$]
\label{thm:graph degenerate}
Suppose Asm.~\ref{eq:assum-dag} holds. Denote $\mathbf{X}_{M}^{0}\!:=\!\mathbf{X}_{M}\cap \mathbf{Ch}(Y)$ as mutable variables in $Y$'s children, and $\mathbf{W}:=\mathbf{De}(\mathbf{X}_{M}^{0}) \backslash \mathbf{X}_M^0$ as descendants of $\mathbf{X}_{M}^{0}$. Then, the $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution if and only if $Y$ does not point to any vertex in $\mathbf{W}$. Further, we have $S^*=S$ if the graphical condition holds.
\end{theorem}

The proof is left in Appx.~\ref{sec: appendix causal minimax theories}. To understand this equivalence, note that if $Y \not \to \mathbf{W}$, we can use the inference rules \citep{pearl2009causality} to remove the ``do" in $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ and degenerate it into $P(Y|\mathbf{X}\backslash(\mathbf{X}_M^0 \cup \mathbf{De}(\mathbf{X}_M^0)))$. On the contrary, if $Y \to \mathbf{W}$, there will a collider in $\mathbf{W}$ in some paths between $Y$ and $\mathbf{X}_M^0$, making it incapable to remove the ``do''. 

\begin{example}
For illustration, consider the causal graph that is shown in Fig.~\ref{fig: example graphical condition} (a), where $Y \not\to \mathbf{W}$. We thus have {\small $Y\ind_{G_{\overline{X_M}}}\! X_1,X_M|X_2$} and hence  {\small $P(Y|X_1,X_2,do(x_M))=P(Y|X_2)$}.  In contrast, for the causal graph shown in Fig.~\ref{fig: example graphical condition} (b), the collider $X_1$ causes {\small $Y \not \ind_{G_{\overline{X_M}}} X_M | X_1$} and prevents the removing of the ``do'' in {\small $P(Y|X_1,do(x_M))$}.
\end{example}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{icml23_figs2/thm3.1_example.pdf}
    \caption{Illustration of the graphical condition in Thm.~\ref{thm:graph degenerate}. Stable and mutable variables are respectively marked blue and red. In both (a) and (b), we have $\mathbf{X}_M^0=\{X_M\}, \mathbf{W}=\{X_1\}$.}
    \label{fig: example graphical condition}
\end{figure}


The following proposition guarantees the testability of this graphical condition, thus enabling it to be used in practice. 


\begin{proposition}[Testability of Thm.~\ref{thm:graph degenerate}]
    \label{prop.thm3.2 justifiability}
    Under Asm.~\ref{eq:assum-dag}-\ref{assum:e-train}, we have that \textbf{i)} the $\mathbf{W}$ is identifiable; and \textbf{ii)} the condition $Y \to \mathbf{W}$ is testable from $\{\mathcal{D}_e\}_{e \in \mathcal{E}_{\mathrm{tr}}}$.
\end{proposition}


Compared to exhaustively running the inference rules to check the degeneration condition in \cite{subbaswamy2019preventing}, our graphical condition can be effectively tested via causal discovery. This can be achieved by firstly learning the skeleton of $G$, followed by detecting $\mathbf{X}_M^0$ and $\mathbf{W}$ by leveraging the heterogeneity in $\mathcal{E}_{\mathrm{tr}}$ \cite{huang2020causal}. Finally, we have $Y \to \mathbf{W}$ if and only if $Y$ is adjacent to any vertices of $\mathbf{W}$ since $\mathbf{W} \subseteq \mathbf{De}(Y)$ according to the definition of $\mathbf{W}$. More details are left to Appx.~\ref{sec: appendix discovery}. 

On the other hand, we show that the whole stable set may not be optimal when this condition does not hold. To be specific, we construct an example with the DAG of Fig.~\ref{fig: example graphical condition} (b), in which $Y, X_M, X_{1}$ are binary variables. We then have the following result:
\begin{claim}
\label{prop:counter}
There exists $P(Y)$ and $P(X_{1}|X_M, Y)$, such that $f_{S}(\boldsymbol{x}):=\mathbb{E}[Y|x_{1},do(x_M)]$ has larger worst-case risk than $f_{\emptyset}(\boldsymbol{x}) := \mathbb{E}[Y|do(x_M)]$: 
\begin{align*}
    \max_{P^e} \mathbb{E}_{P^e}[(Y-f_S(\boldsymbol{x}))^2] > \max_{P^e} \mathbb{E}_{P^e}[(Y-f_\emptyset(\boldsymbol{x}))^2].
\end{align*}
\end{claim}

\begin{remark}
This result seems surprising as intuitively the whole stable set should be optimal since it fully exploits the stable information, according to existing minimax results in \cite{peters2016causal, rojas2018invariant}. To explain, we should note that these results are built on \emph{conditional} distributions, where one can construct a $P^e$ to make any other predictor having a larger quadratic loss than $f_S$. However, when the \emph{interventional} distribution can not degenerate, such a construction is generally not feasible. Please refer to Appx.~\ref{sec: counter example appendix new} for a more detailed analysis. 
\end{remark}

% MZ change at 0114
% To explain, we should note that these results are built on \emph{conditional} distributions, where one can construct a $P^e$ to make any other predictor having a larger quadratic loss than $f_S$. However, when the \emph{interventional} distribution can not degenerate, such a construction is generally not feasible. Please refer to Appx.~\ref{sec: counter example appendix new} for a more detailed analysis. 

% XW version
% To explain, we should note that these results for conditional distribution may not hold on intervened distribution (\emph{i.e.}, $P(Y|\mathbf{X}_S,do(\boldsymbol{x}_M))$), under which case it is unable to construct $P^e$ to make any other predictor have larger population loss than $f_S$.

Under the general cases where the whole stable set may not be optimal, it remains unknown that \emph{which subset of stable information is the optimal one to transfer?} To answer this question, we propose to estimate the worst-case risk $\mathcal{R}_{S^\prime}\!:=\!\max_{e \in \mathcal{E}} \mathbb{E}_{P^e}[\left(Y \!-\! f_{S^\prime}(\boldsymbol{x})\right)^2]$ for each subset $S^\prime$; then the $S^*$ corresponds to the subset with minimal $\mathcal{R}$. To estimate $\mathcal{R}_{S^\prime}$ for each $S^\prime \subseteq S$, we consider a distribution family $\{P_h\}_{h}$, where $h$ maps from $\mathcal{P}a(\mathcal{X}_M)$ to $\mathcal{X}_M$ and $P_h\! :=\! P(Y,\mathbf{X}_S| do(\boldsymbol{x}_M\!=\!h(\boldsymbol{pa}(\boldsymbol{x}_M)))$. This distribution set keeps the invariant mechanisms of $Y$ and $\mathbf{X}_S$ unchanged while allowing the $\mathbf{X}_M$ given their parents to vary arbitrarily, which can well mimic the distributional shifts among deployed environments in $\{P^e\}_{e \in \mathcal{E}}$. Particularly, we show that the worst-case risk $\mathcal{R}_{S^\prime}$ can be attained at some $P_h$, where $h$ is a Borel measurable function. Formally, denote $\mathcal{B}$ as the Borel function set, we have: 

\begin{theorem}[Identify the worst-case risk]
\label{thm:min-max}
Let $\mathcal{L}_{S^\prime}:=\max_{h \in  \mathcal{B}}\mathbb{E}_{P_h}[(Y \!-\! f_{S^\prime}(\boldsymbol{x}))^2]$ be the maximal population loss over $\{P_h\}_{h \in \mathcal{B}}$ for subset $S^\prime$. Then, we have $\mathcal{L}_{S^\prime}=\mathcal{R}_{S^\prime}$ for each $S^\prime \subseteq S$. Therefore, we have $S^*= \mathop{\mathrm{argmin}}_{S^\prime \subseteq S} \mathcal{L}_{S^\prime}$.
\end{theorem}


This result inspires the following optimization problem over the function $h \in  \mathcal{B}$ to estimate $\mathcal{R}_{S^\prime}$: 
\begin{align*}
    \max_{h \in  \mathcal{B}} \mathcal{L}_{S^\prime}(h) := \mathbb{E}_{P_h}[(Y \!-\! f_{S^\prime}(\boldsymbol{x}))^2],
\end{align*}
as the optimality of which is assured to attain $\mathcal{R}_{S^\prime}$. To implement, we parameterize the $h:\mathcal{P}a(\mathcal{X}_M)\!\to\!\mathcal{X}_M$ with a multilayer perceptron (MLP) for optimization, due to the ability of MLP to approximate any Borel function \cite{hornik1989multilayer}. To show the tractability of this optimization, we have the following identifiability result for $\mathcal{L}_{S^\prime}(h)$. 


\begin{proposition}
	\label{prop.thm3.3 justifiability}
	Under Asm.~\ref{eq:assum-dag}-\ref{assum:e-train}, the  $P_h$, $f_{S^\prime}$, and hence $\mathcal{L}_{S^\prime}(h)$ are identifiable. 
\end{proposition}


\textbf{Summary.} Our results answer the two questions raised in Sec.~\ref{sec.background}. Specifically, Thm.~\ref{thm:graph degenerate} provides an equivalent but a more intuitive graphical condition for $S^*=S$; while Thm.~\ref{thm:min-max} motivates an optimization-based approach to identify the optimal subset $S^*$ with theoretical guarantees. 






==> icml23_paras/old_method_mz/background_mz_v1.tex <==
\section{Preliminaries and Background} 
\label{sec.background}

\textbf{Problem Setup \& Notations.} We consider the supervised regression scenario, where the system includes a target variable $Y \!\in\! \mathcal{Y}$, covariates $\mathbf{X}\!:=\! [X_1,...,X_d] \!\in\! \mathcal{X}$, and data collected from heterogeneous environments. In practice, different ``environments" can refer to different groups of subjects or different experimental settings. We denote the environmental indicator variable as $E$, the set of training environments as $\mathcal{E}_{\mathrm{tr}}$, and the broader set of environments for deployment as $\mathcal{E}$. We use $\{D_{e}|e\in\mathcal{E}_{\text{tr}}\}$ to denote our training data, with ${D_{e}\!:=\!\{(\boldsymbol{x}_{k}^e, {y}_{k}^e)\}_{k=1}^{n_e} \sim_{i.i.d} P^e(\mathbf{X},Y)}$ being the data sampled from environment $e$. In a directed acyclic graph (DAG) $G$, we denote the parents, children, neighbors, and descendants of the vertices set $\mathbf{V}$ as $\mathrm{Pa}({\mathbf{V}})$, $\mathrm{Ch}({\mathbf{V}})$, $\mathrm{Neig}(\mathbf{V})$, and $\mathrm{De}({\mathbf{V}})$, respectively. Define $\mathrm{deg}(V_i):=|\mathrm{Neig}(V_i)|$. We use $\perp$ to denote conditional independence, and $(\perp)_G$ to denote \emph{d}-separation in $G$. We denote $G_{\overline{\mathbf{V}}}$ as the graph deleting all arrows pointing into vertices in $\mathbf{V}$. 


Our goal is to find the most robust predictor $f^*$ among stable predictors with data from $\mathcal{E}_{\mathrm{tr}}$. Here, we say a predictor $f \!:\! \mathcal{X} \to \mathcal{Y}$ is stable if it is independent of $E$. We denote the set of stable predictors as $\mathcal{F}_S$. For robustness, a commonly adopted measurement \cite{peters2016causal,ahuja2021invariance} is to investigate a predictor's worst-case risk, which provides a safeguard for deployment in unseen environments. That is, we want $f^*$ to have the following minimax property:
\begin{align}
    f^{*}(\boldsymbol{x})=\mathop{\mathrm{argmin}}\limits_{f \in \mathcal{F}_S}        \max_{e\in\mathcal{E}}
    \mathbb{E}_{P^e}[(Y-f(\boldsymbol{x}))^2].
\label{eq.robust}
\end{align}
Next, we introduce some assumptions that our methods are based on. These assumptions are commonly made in the literature of causal inference and learning \cite{pearl2009causality,spirtes2000causation,arjovsky2019invariant}.
\begin{assumption}[Structural Causal Model]
\label{eq:assum-dag}
We assume that $P^e(\mathbf{X},Y)$ is entailed by an \emph{unknown} DAG $G$ over $\mathbf{V}$ for all $e \in \mathcal{E}$, where $\mathbf{V}:= \mathbf{X} \cup Y$. Each variable $V_i \in \mathbf{V}$ is generated via a structural equation $V_i=g^e_{i}(\mathrm{Pa}({V_i}), U_i)$, where $U_i$ denotes a exogenous variable. We assume  
each $g^e_{i}$ is continuous and bounded. Each edge $V_i \to V_j$ in $G$ represents a direct causal influence from $V_i$ on $V_j$. 
\end{assumption}


Equipped with the autonomous property of structural equations, we introduce the definition of \emph{intervention} \cite{pearl2009causality}. The intervention $do(V_i\!=\!v_i)$ means lifting $V_i$ from its original generating mechanism $V_i\!=\!\!g_{i}(\mathrm{Pa}({V_i}), U_i)$ and setting it to a constant value $v_i$. Under the following Markovian assumption, the intervention distribution $P(\mathbf{V}\backslash V_i| do(v_i)):=P(\mathbf{V})/ P(V_i|\mathrm{Pa}(V_i))$.

\begin{assumption}[Markovian and Faithfulness]
\label{eq:assum-markov-faithfulness}
The Markovian assumes $\{U_i\}$ are mutually independent. This means {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Rightarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}, $\forall$ disjoint sets {\small $\mathbf{V}_i, \mathbf{V}_j, \mathbf{V}_k$}. The faithfulness assumes {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Leftarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}. In combination, we assume {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Leftrightarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}.
\end{assumption}

According to the Causal Markov condition \citep{pearl2009causality}, we have the causal factorization of the joint probability $P^e(\mathbf{V}) = \prod_i P^e(V_i|\mathrm{Pa}(V_i)))$, where each term $P^e(V_i|\mathrm{Pa}(V_i))$ represents the generation of $V_i$ given its parents $\mathrm{Pa}(V_i)$. In our scenario, the $P^e(\mathbf{X},Y)$ has:
\begin{align}
\label{eq: causal factorization}
    & P^e(\mathbf{X},Y) = P(Y|\mathrm{Pa}(Y)) \prod_{i \in S} P\left(X_i|\mathrm{Pa}(X_i)\right) \nonumber \\
    & \prod_{i \in M} P^e(X_i|\mathrm{Pa}(X_i)), d_S:=|S|, d_M:=|M|,
\end{align}
where $S, M$ respectively denote stable and mutable sets such that each $X_i \in \mathbf{X}_S$ has invariant causal factor $P(X_i|\mathrm{Pa}(X_i))$; while the factor of each $X_i \in \mathbf{X}_M$ varies across $\mathcal{E}$. Correspondingly, we call $\mathbf{X}_S$ as stable variables and $\mathbf{X}_M$ as mutable variables. In addition to $\mathbf{X}_S$, we also assume the causal factor of $Y$ keeps invariant across $\mathcal{E}$, as widely adopted by the existing literature \cite{arjovsky2019invariant,sun2021recovering,mitrovic2021representation}. Besides, we assume that $\mathcal{E}_{\mathrm{tr}}$ can consistently reflect the heterogeneity in $\mathcal{E}$, which is formally stated as follows: 
\begin{assumption}[Consistent Heterogeneity]
\label{assum:e-train}
For each $X_i \in \mathbf{X}_M$, we assume that there exists $e_1, e_2 \in \mathcal{E}_{\mathrm{tr}}$ with $e_1 \neq e_2$ such that $P^{e_1}(X_i|\mathrm{Pa}(X_i)) \neq P^{e_1}(X_i|\mathrm{Pa}(X_i))$.
\end{assumption}

This assumption requires $\mathcal{E}_{\mathrm{tr}}$ to be large and diverse enough to reflect the mutation of $\mathbf{X}_M$ across $\mathcal{E}$, which is necessary to recover $\mathbf{X}_M$ from training data. 


\textbf{Surgery Estimator.} The surgery estimator \citep{subbaswamy2019preventing} proposed to remove the mutation in $P^e(\mathbf{X},Y)$ by intervening on $\mathbf{X}_M$ and obtained a set of stable predictors $\mathcal{F}_S:=\{f_{S^\prime}(\boldsymbol{x})|S^\prime\!\subseteq \!{S}\}, f_{S^\prime}(\boldsymbol{x})\!:=\!\mathbb{E}[Y|\boldsymbol{x}_{S^\prime}, do(\boldsymbol{x}_M)]$ over the interventional distribution. In this regard, identifying the minimax optimal predictor in Eq.~\ref{eq.robust} is equivalent to selecting the optimal subset $S^*$ such that $f_{S^*}$ is min-max optimal among $\mathcal{F}_S$. 


%\textcolor{blue}{is equivalent to selecting the optimal subset $S^* := \arg\min_{S^\prime \subseteq S} \mathcal{R}_{S^\prime}$, where $\mathcal{R}_{S^\prime}\!:=\!\max_{e \in \mathcal{E}} \mathbb{E}_{P^e}[\left(Y \!-\! f_{S^\prime}(\boldsymbol{x})\right)^2]$ denotes the worst-case risk of the subset $S^\prime$}. 

For this purpose, they first proved that the whole stable set $S$ is optimal under the \emph{degeneration condition}: the interventional distribution $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution  $P(Y|\mathbf{X}^\prime)$ for some $\mathbf{X}^\prime \subseteq \mathbf{X}$. However, the authors did not provide an approach to \textbf{test this condition}, limiting the utility of the theory. In practice, they compared each subset $S^\prime \subseteq S$ and selected the $S^*$ as the one with minimal loss on a held-out validation set. This method \textbf{lacks} a theoretical guarantee. Indeed, we observe from Fig. \ref{fig:adni-intro} that the selected subset is not optimal, because the validation loss does not necessarily reflect the worst-case risk among deployed environments. In the subsequent section, we propose to remedy the above problems of the Surgery estimator, by considering the following questions: \textbf{i)} \emph{Can we test the degeneration condition, or some of its equivalent conditions, in order to determine whether $S^* = S$?} \textbf{ii)} \emph{Can we provide an approach to identify the optimal subset with theoretical guarantees under general scenarios?}



==> icml23_paras/old_method_mz/background_mz_v2.tex <==
\section{Preliminaries and Background} 
\label{sec.background}

\textbf{Problem Setup \& Notations.} We consider the supervised regression scenario, where the system includes a target variable $Y \!\in\! \mathcal{Y}$, covariates $\mathbf{X}\!:=\! [X_1,...,X_d] \!\in\! \mathcal{X}$, and data collected from heterogeneous environments. In practice, different ``environments" can refer to different groups of subjects or different experimental settings. We denote the set of training environments as $\mathcal{E}_{\mathrm{tr}}$, and the broader set of environments for deployment as $\mathcal{E}$. We denote $E$ as the environmental indicator variable with suppose $\mathcal{E}$. We use $\{\mathcal{D}_{e}|e\in\mathcal{E}_{\text{tr}}\}$ to denote our training data, with ${\mathcal{D}_{e}\!:=\!\{(\boldsymbol{x}_{k}^e, {y}_{k}^e)\}_{k=1}^{n_e} \sim_{i.i.d} P^e(\mathbf{X},Y)}$ being the data sampled from environment $e$. In a directed acyclic graph (DAG) $G$, we denote the parents, children, neighbors, and descendants of the vertex $V_i$ as $\mathbf{Pa}(V_i)$, $\mathbf{Ch}(V_i)$, $\mathbf{Neig}(V_i)$, and $\mathbf{De}(V_i)$, respectively. Define $\mathrm{deg}(V_i):=|\mathbf{Neig}(V_i)|$. We denote $G_{\overline{V_i}}$ as the graph attained via deleting all arrows pointing into $V_i$.  We use $\ind_G$ to denote \emph{d}-separation in $G$. 


Our goal is to find the most robust predictor $f^*$ among stable predictors with data from $\mathcal{E}_{\mathrm{tr}}$. Here, we say a predictor $f \!:\! \mathcal{X} \to \mathcal{Y}$ is stable if it is independent of $E$. We denote the set of stable predictors as $\mathcal{F}_S$. For robustness, a commonly adopted measurement \cite{peters2016causal,ahuja2021invariance} is to investigate a predictor's worst-case risk, which provides a safeguard for deployment in unseen environments. That is, we want $f^*$ to have the following minimax property:
\begin{align}
    f^{*}(\boldsymbol{x})=\mathop{\mathrm{argmin}}\limits_{f \in \mathcal{F}_S}        \max_{e\in\mathcal{E}}
    \mathbb{E}_{P^e}[(Y-f(\boldsymbol{x}))^2].
\label{eq.robust}
\end{align}
Next, we introduce some assumptions that our methods are based on. These assumptions are commonly made in the literature of causal inference and learning \cite{pearl2009causality,spirtes2000causation,arjovsky2019invariant}.
\begin{assumption}[Structural Causal Model]
\label{eq:assum-dag}
We assume that $P^e(\mathbf{X},Y)$ is entailed by an \emph{unknown} DAG $G$ over $\mathbf{V}$ for all $e \in \mathcal{E}$, where $\mathbf{V}:= \mathbf{X} \cup Y$. Each variable $V_i \in \mathbf{V}$ is generated via a structural equation $V_i=g^e_{i}(\mathrm{Pa}({V_i}), U_i)$, where $U_i$ denotes an exogenous variable. We assume  
each $g^e_{i}$ is continuous and bounded. Each edge $V_i \to V_j$ in $G$ means $V_i$ is a direct causal of $V_j$. 
\end{assumption}

Under the following Markovian assumption, we can factorize the joint probability \emph{causally} over $G$: $P^e(\mathbf{V}) = \prod_i P^e(V_i|\mathrm{Pa}(V_i)))$, where $P^e(V_i|\mathrm{Pa}(V_i)))$ is the causal mechanism of $V_i$.


\begin{assumption}[Markovian]
\label{asm: markovian}
    The exogenous variables $\{U_i\}$ are mutually independent. This means for disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, $\mathbf{A} \ind_G \mathbf{B} | \mathbf{Z} \Rightarrow \mathbf{A} \ind \mathbf{B} | \mathbf{Z}$.
\end{assumption}

Based on the idea of independence causal mechanisms \cite{pearl2009causality}, we posits the distributional shifts in $P^e(\mathbf{X},Y)$ are the results of changes in a subsets of the causal model's mechanisms \cite{scholkopf2021toward}. That is:
\begin{align}
\label{eq: causal factorization}
    & P^e(\mathbf{X},Y) = P(Y|\mathrm{Pa}(Y)) \prod_{i \in S} P\left(X_i|\mathrm{Pa}(X_i)\right) \nonumber \\
    & \prod_{i \in M} P^e(X_i|\mathrm{Pa}(X_i)), d_S:=|S|, d_M:=|M|,
\end{align}
where $S, M$ respectively denote stable and mutable sets such that each $X_i \in \mathbf{X}_S$ has invariant causal mechanism $P(X_i|\mathrm{Pa}(X_i))$; while the mechanism of each $X_i \in \mathbf{X}_M$ varies across $\mathcal{E}$. Correspondingly, we call $\mathbf{X}_S$ as stable variables and $\mathbf{X}_M$ as mutable variables. In addition to $\mathbf{X}_S$, we also assume the causal mechanism of $Y$ keeps invariant across $\mathcal{E}$, as widely adopted by the existing literature \cite{arjovsky2019invariant,sun2021recovering,mitrovic2021representation}.

While the Markovian assumption allows us to drive distributional properties from the DAG, the following faithfulness assumptions allow us to recover the DAG from the distributional properties:
\begin{assumption}[Faithfulness]
    For disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, $\mathbf{A} \ind \mathbf{B} | \mathbf{Z} \Rightarrow \mathbf{A} \ind_G \mathbf{B} | \mathbf{Z}$. 
\end{assumption}
To recover the $\mathbf{X}_M$ from the training distribution, we also assume that $\mathcal{E}_{\mathrm{tr}}$ is large and diverse enough to reflect the mutation of $\mathbf{X}_M$ across $\mathcal{E}$. This is formally stated as follows:
\begin{assumption}[Consistent Heterogeneity]
\label{assum:e-train}
For each $X_i \in \mathbf{X}_M$, there exists $e, e^\prime \in \mathcal{E}_{\mathrm{tr}}, e \neq e^\prime$, s.t. $P^{e}(X_i|\mathrm{Pa}(X_i)) \neq P^{e^\prime}(X_i|\mathrm{Pa}(X_i))$.
\end{assumption}

\textbf{Intervention.} The intervention $do(V_i\!=\!v_i)$ ($do(v_i)$ for abbreviation) means lifting $V_i$ from its original causal mechanism $V_i\!=\!\!g_{i}(\mathrm{Pa}({V_i}), U_i)$ and setting it to a constant value $v_i$ \cite{pearl2009causality}. Under Asm.~\ref{asm: markovian}, the interventional distribution $P(\mathbf{V}\backslash V_i| do(v_i)):= \prod_{j \neq i} P^e(V_j|\mathrm{Pa}(V_j)))$.

\textbf{Surgery Estimator.} The surgery estimator \citep{subbaswamy2019preventing} proposed to remove the mutation in $P^e(\mathbf{X},Y)$ by intervening on $\mathbf{X}_M$ and obtained a set of stable predictors $\mathcal{F}_S:=\{f_{S^\prime}(\boldsymbol{x})|S^\prime\!\subseteq \!{S}\}, f_{S^\prime}(\boldsymbol{x})\!:=\!\mathbb{E}[Y|\boldsymbol{x}_{S^\prime}, do(\boldsymbol{x}_M)]$ over the interventional distribution. In this regard, identifying the minimax optimal predictor in Eq.~\ref{eq.robust} is equivalent to selecting the optimal subset $S^*$ such that $f_{S^*}=f^*$. 

% Equipped with the autonomous property of structural equations, we introduce the definition of \emph{intervention} \cite{pearl2009causality}. The intervention $do(V_i\!=\!v_i)$ means lifting $V_i$ from its original generating mechanism $V_i\!=\!\!g_{i}(\mathrm{Pa}({V_i}), U_i)$ and setting it to a constant value $v_i$. Under the following Markovian assumption, the intervention distribution $P(\mathbf{V}\backslash V_i| do(v_i)):=P(\mathbf{V})/ P(V_i|\mathrm{Pa}(V_i))$.

% \begin{assumption}[Markovian and Faithfulness]
% \label{eq:assum-markov-faithfulness}
% The Markovian assumes $\{U_i\}$ are mutually independent. This means {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Rightarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}, $\forall$ disjoint sets {\small $\mathbf{V}_i, \mathbf{V}_j, \mathbf{V}_k$}. The faithfulness assumes {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Leftarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}. In combination, we assume {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Leftrightarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}.
% \end{assumption}

% According to the Causal Markov condition \citep{pearl2009causality}, we have the causal factorization of the joint probability $P^e(\mathbf{V}) = \prod_i P^e(V_i|\mathrm{Pa}(V_i)))$, where each term $P^e(V_i|\mathrm{Pa}(V_i))$ represents the generation of $V_i$ given its parents $\mathrm{Pa}(V_i)$. In our scenario, the $P^e(\mathbf{X},Y)$ has:
% \begin{align}
% \label{eq: causal factorization}
%     & P^e(\mathbf{X},Y) = P(Y|\mathrm{Pa}(Y)) \prod_{i \in S} P\left(X_i|\mathrm{Pa}(X_i)\right) \nonumber \\
%     & \prod_{i \in M} P^e(X_i|\mathrm{Pa}(X_i)), d_S:=|S|, d_M:=|M|,
% \end{align}
% where $S, M$ respectively denote stable and mutable sets such that each $X_i \in \mathbf{X}_S$ has invariant causal factor $P(X_i|\mathrm{Pa}(X_i))$; while the factor of each $X_i \in \mathbf{X}_M$ varies across $\mathcal{E}$. Correspondingly, we call $\mathbf{X}_S$ as stable variables and $\mathbf{X}_M$ as mutable variables. In addition to $\mathbf{X}_S$, we also assume the causal factor of $Y$ keeps invariant across $\mathcal{E}$, as widely adopted by the existing literature \cite{arjovsky2019invariant,sun2021recovering,mitrovic2021representation}. Besides, we assume that $\mathcal{E}_{\mathrm{tr}}$ can consistently reflect the heterogeneity in $\mathcal{E}$, which is formally stated as follows: 
% \begin{assumption}[Consistent Heterogeneity]
% \label{assum:e-train}
% For each $X_i \in \mathbf{X}_M$, we assume that there exists $e_1, e_2 \in \mathcal{E}_{\mathrm{tr}}$ with $e_1 \neq e_2$ such that $P^{e_1}(X_i|\mathrm{Pa}(X_i)) \neq P^{e_1}(X_i|\mathrm{Pa}(X_i))$.
% \end{assumption}

% This assumption requires $\mathcal{E}_{\mathrm{tr}}$ to be large and diverse enough to reflect the mutation of $\mathbf{X}_M$ across $\mathcal{E}$, which is necessary to recover $\mathbf{X}_M$ from training data. 


% \textbf{Surgery Estimator.} The surgery estimator \citep{subbaswamy2019preventing} proposed to remove the mutation in $P^e(\mathbf{X},Y)$ by intervening on $\mathbf{X}_M$ and obtained a set of stable predictors $\mathcal{F}_S:=\{f_{S^\prime}(\boldsymbol{x})|S^\prime\!\subseteq \!{S}\}, f_{S^\prime}(\boldsymbol{x})\!:=\!\mathbb{E}[Y|\boldsymbol{x}_{S^\prime}, do(\boldsymbol{x}_M)]$ over the interventional distribution. In this regard, identifying the minimax optimal predictor in Eq.~\ref{eq.robust} is equivalent to selecting the optimal subset $S^*$ such that $f_{S^*}$ is min-max optimal among $\mathcal{F}_S$. 

For this purpose, they first proved that the whole stable set $S$ is optimal under the \emph{degeneration condition}: the interventional distribution $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution  $P(Y|\mathbf{X}^\prime)$ for some $\mathbf{X}^\prime \subseteq \mathbf{X}$. However, the authors did not provide an approach to \textbf{test this condition}, limiting the utility of the theory. In practice, they compared each subset $S^\prime \subseteq S$ and selected the $S^*$ as the one with minimal loss on a held-out validation set. This method \textbf{lacks} a theoretical guarantee. Indeed, we observe from Fig. \ref{fig:adni-intro} that the selected subset is not optimal, because the validation loss does not necessarily reflect the worst-case risk among deployed environments. In the subsequent section, we propose to remedy the above problems of the Surgery estimator, by considering the following questions: \textbf{i)} \emph{Can we test the degeneration condition, or some of its equivalent conditions, in order to determine whether $S^* = S$?} \textbf{ii)} \emph{Can we provide an approach to identify the optimal subset with theoretical guarantees under general scenarios?}



==> icml23_paras/old_method_mz/complexity_mz_v1.tex <==
\section{Searching Complexity Analysis}
\label{sec.complex}

In this section, we discuss the searching complexity over $N_G$ \emph{g}-equivalent classes. We show that this \emph{g}-equivalence can reduce the exponential complexity $O(2^{d_S})$ to a polynomial one $\mathrm{P}(d_S)$ in some cases.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\textwidth]{icml23_figs/simg3_ad_causal_graphs.pdf}
    \caption{(a) The causal graph for synthetic data generation. The dashed line $M_1 \to S_1$ does not exist (resp. exist) in setting-1 (resp. setting-2). (b) The learned causal graph on ADNI. $\leftrightarrow$ denotes undirected edges.}
    \label{fig:simg3_ad_causal_graphs}
\end{figure*}

Our observation is that the chain, as shown in Fig.~\ref{fig:complexity_chain_tree} (a), is the key structure that \emph{g}-equivalence can reduce the cost. This is because in the chain, one vertex can block the other far-ends variables from $Y$, inducing all the far-ends subsets to be \emph{g}-equivalence. For example, in Fig.~\ref{fig:complexity_chain_tree} (a), we have $(Y \perp \mathbf{X}_{S_2 \cdots S_6} | \mathbf{X}_{S_1})_{G_S}$ and thus the equivalent class $[S_1]=\{S_1 \cup S_- | S_- \in \mathrm{Pow}(\{S_2,...,S_6\})\}$. Formally, we have:

\begin{claim}[Chain]
For a chain with $d_S$ vertices, $N_G=d_S+1$ equals to the length of the chain.
\end{claim}

\begin{remark}
For multiple chains, \emph{e.g.}, Fig.~\ref{fig:complexity_chain_tree} (b), the $N_G$ is the product of the chains' lengths, which means the more dispersive chains are, the larger the complexity will be.
\end{remark}

To conclude, we find that the more vertices distributed in chains, and the more intensive the chains are, the smaller $N_G$ will be. Since vertices in chains have $\mathrm{deg} \leq 2$, we can use the $d_{\leq 2}:=\sum_i {1}(\mathrm{deg}(X_i) \leq 2)$ to measure their proportion. To measure the intensity of chains, we introduce a new metric $F_G$, which is an extension of the products of chains' lengths. We first illustrate $F_G$ in trees, as follows:

\begin{claim}[Tree]
For a $Y$-rooted tree, let
\begin{equation*}
    F_G:=\prod_{c \in \mathrm{Ch}(Y)} f(c), \,\, f(c):=\mathrm{len}(c)+\prod_{\tilde{c} \in \mathrm{Ch}(c)} f(\tilde{c}),
\end{equation*}
where $\tilde{c} \in \mathrm{Ch}(c)$ means $\tilde{c}$ is the child of $c$ in the tree. Then, $N_G=\mathrm{P}(d_S)$ iff $d_S - d_{\leq 2}=O(\mathrm{log}(d_S))$ and $F_G=\mathrm{P}(d_S)$. 
\end{claim}

For example, in Fig.~\ref{fig:complexity_chain_tree} (c), we have $d_S - d_{\leq 2}=2$ and $F_G=(l_1+l_3 l_4)(l_2+l_5 l_6)$, $l_i:=\mathrm{len}(c_i)$. In this regard, we can compare $F_G$ with $d_S$ to decide the complexity.

In general cases where $G_S$ has cycles, we can break the cycles via deleting edges and convert it into a series of subtrees, as shown in Fig.~\ref{fig:complexity_chain_tree} (d). Specifically, for each chain $c$ that is adjacent to $Y$, define a set of edge-deletion operators $\mathrm{opt}_c:=\{\text{delete} \, e^{1:i}|i=1,...,\mathrm{len}(c)\}$, with $e^{1:i}$ the $1:i$ edges in $c$, we have the following proposition:

\begin{proposition}[Informal] For a stable graph $G_S$, let
\begin{equation*}
    F_{G_S}:=\prod_{\substack{c\in \mathrm{Neig}(Y) \\ \mathrm{Neig}(c) = \varnothing}} \mathrm{len}(c) \sum_{\mathrm{opt}\in \prod_{c\in \mathrm{Neig}(Y)}\mathrm{opt}_{c}} F_{\mathrm{opt}(G_S)},
\end{equation*}
with $\mathrm{Neig}(c) = \varnothing$ if $c$ is disjoint with the other chains. Then, $N_G=\mathrm{P}(d_S)$ iff $d_S - d_{\leq 2}=O(\mathrm{log}(d_S))$ and $F_G=\mathrm{P}(d_S)$. 
\end{proposition}



==> icml23_paras/old_method_mz/complexity_mz_v2.tex <==
\section{Searching Complexity Analysis}
\label{sec.complex}

In this section, we discuss the searching complexity of Alg.~\ref{alg:identify-f-star}. We show that our proposed equivalent relation can reduce the exponential searching complexity $O(2^{d_S})$ to a polynomial one $\mathrm{P}(d_S)$.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\textwidth]{icml23_figs/simg3_ad_causal_graphs.pdf}
    \caption{(a) The causal graph for synthetic data generation. The dashed line $M_1 \to S_1$ does not exist (resp. exist) in setting-1 (resp. setting-2). (b) The learned causal graph on ADNI. $\leftrightarrow$ denotes undirected edges.}
    \label{fig:simg3_ad_causal_graphs}
\end{figure*}

To begin, we first look at a special graph structure: the chain (Fig.~\ref{fig:complexity_chain_tree} (a)), which is important in reducing the complexity. To see the reason, note that each vertex in the chain can block the other far-ends vertices from $Y$, \textcolor{blue}{making each subset equivalent to the ones that append the other far-end vertices.} For example, in Fig.~\ref{fig:complexity_chain_tree} (a), we have $\{S_i\} \sim_G \{S_i\} \cup S^\prime$ for each $S^\prime \subseteq \{S_i,S_{i+1},...,S_6\}$ since $\{S_i\}$ blocks the far-ends vertices $\{S_i,S_{i+1},...,S_6\}$ from $Y$. As a result, we have $\mathrm{Pow}(S)/ \! \sim_G = \{[S_1],...,[S_6],\{\varnothing\}\}$. Formally, we have: 

\begin{claim}[Chain]
For a chain with $d_S$ vertices, there are $d_S+1$ equivalent classes.
\end{claim}

This means, for each chain, the equivalent relation can reduce the complexity from $O(2^{d_S})$ to $O(d_S)$. Therefore, intuitively the searching cost of the whole graph will be reduced more significantly, if more vertices are distributed in chains. \textcolor{blue}{Formally, we split the vertices in $G_S$ into chain vertices and non-chain vertices, with the former ones distributed in chains and having $\mathrm{deg}\leq 2$. Correspondingly, we use $d_{\leq 2}$ and $d_{>2}$ to denote the number of chain vertices and non-chain vertices, respectively.} We show that when $d_{>2} = O(\log({d_S}))$, which means the chain vertices take a major proportion in $G_S$, the $N_G$ can be reflected by the $F_G$, which is roughly speaking the product of chain's lengths. 

To ease the understanding, we first introduce the $F_G$ for the tree structure (Fig.~\ref{fig:complexity_chain_tree} (c)), which means the skeleton of $G_S$ does not contain cycles. \textcolor{blue}{In a $Y$-rooted tree, define the parent of a chain $c$ as the chain adjacent to $c$ on the path to the root $Y$. Denote $\mathrm{Pa}^\prime(c), \mathrm{Ch}^\prime(c)$ as the set of $c$'s parent and children, respectively.} Then, we have:

\begin{claim}[Tree]
For a $Y$-rooted tree, let
\begin{align*}
    F_G:=\prod_{c \in \mathrm{Ch}^{\prime}(Y)} f(c), \,\, f(c):=\mathrm{len}(c)+\prod_{\tilde{c} \in \mathrm{Ch}^{\prime}(c)} f(\tilde{c}).
\end{align*}
Then, {\small $N_G=\mathrm{P}(d_S)$} iff {\small $d_{>2}=O(\mathrm{log}(d_S))$} and {\small $F_G=\mathrm{P}(d_S)$}. 
\end{claim}

\textcolor{blue}{For example, in Fig.~\ref{fig:complexity_chain_tree} (c), we have 
$d_{>2}=2$, $\mathrm{Ch}^\prime(Y):=\{c_1, c_2\}$, $\mathrm{Ch}^{\prime}(c_1):=\{c_3, c_4\}$, $\mathrm{Ch}^{\prime}(c_2):=\{c_5, c_6\}$, and the $F_G:=(l_1+l_3 l_4)(l_2+l_5 l_6)$ with $l_i:=\mathrm{len}(c_i)$.} 


Now, we consider the general cases where $G_S$ has cycles (Fig.~\ref{fig:complexity_chain_tree} (d)). To extend the $F_G$, we can break the cycles via deleting edges and convert $G_S$ into a series of subtrees. \textcolor{blue}{Formally, define $c\in \mathrm{Neig}^\prime(Y)$ if there is no other chain on the shortest path from $c$ to $Y$. Let $\mathrm{Neig}^\prime(c)=\varnothing$ if $c$ is disjoint with the other chains. For each chain $c\in \mathrm{Neig}^\prime(Y)$, define a set of edge-deletion operators $\mathrm{opt}_c:=\{\text{delete the}\, 1-i \,\text{edges in } c| i=1,...,\mathrm{len}(c)\}$.} Then,


\begin{proposition}[Informal] For a stable graph, let
\begin{align*}
    F_{G}:=\prod_{\substack{c\in \mathrm{Neig}^{\prime}(Y) \\ \mathrm{Neig}^{\prime}(c) = \varnothing}} \mathrm{len}(c) \sum_{\mathrm{opt}\in \prod_{c\in \mathrm{Neig}^{\prime}(Y)}\mathrm{opt}_{c}} F_{\mathrm{opt}(G)},
\end{align*}
Then, {\small $N_G=\mathrm{P}(d_S)$} iff {\small $d_{>2}=O(\mathrm{log}(d_S))$} and {\small $F_G=\mathrm{P}(d_S)$}. 
\end{proposition}

\begin{remark}
    This result means when $d_{>2}=O(\mathrm{log}(d_S))$, the equivalent relation can reduce the searching complexity to a polynomial level. 
\end{remark}

==> icml23_paras/old_method_mz/complexity_mz_v3.tex <==


% This result means when $d_{>2}=O(\mathrm{log}(d_S))$, the equivalent relation can reduce the searching complexity to a polynomial level. 


\section{Searching Complexity Analysis}
\label{sec.complex}

In this section, we show that the equivalent relation can reduce the searching complexity of Alg.~\ref{alg:identify-f-star} from exponential $O(2^{d_S})$ to polynomial $\mathrm{P}(d_S)$.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\textwidth]{icml23_figs/simg3_ad_causal_graphs.pdf}
    \caption{(a) The causal graph for synthetic data generation. The dashed line $M_1 \to S_1$ does not exist (resp. exist) in setting-1 (resp. setting-2). (b) The learned causal graph on ADNI. $\leftrightarrow$ denotes undirected edges.}
    \label{fig:simg3_ad_causal_graphs}
\end{figure*}

To begin, we first look at a special graph structure: the \emph{chain} (Fig.~\ref{fig:complexity_chain_tree} (a)), which is important in reducing the complexity. To see the reason, note that each vertex in the chain can block the other far-ends vertices from $Y$, making each subset equivalent to ones that append any other far-end vertices. For example, in Fig.~\ref{fig:complexity_chain_tree} (a), we have $\{S_i\} \sim_G \{S_i\} \cup S^\prime$ for each $S^\prime \subseteq \{S_i,S_{i+1},...,S_6\}$ since $\{S_i\}$ blocks the far-ends vertices $\{S_i,S_{i+1},...,S_6\}$ from $Y$. As a result, we have $\mathrm{Pow}(S)/ \! \sim_G = \{[S_1],...,[S_6],\{\varnothing\}\}$. Formally, 

\begin{claim}[Chain]
A chain with $d_S$ vertices has $d_S+1$ equivalent classes.
\end{claim}

This means, for each chain, the equivalent relation can reduce the complexity from $O(2^{d_S})$ to $O(d_S)$. Therefore, for the whole graph, the more vertices distributed in chains, the more complexity can be reduced. Formally, we split the vertices in $G_S$ into chain vertices and non-chain vertices, with chain vertices (resp. non-chain vertices) referring to those vertices with $\mathrm{deg} \leq 2$ (resp. $\mathrm{deg} > 2$). We use $d_{\leq 2}$ and $d_{>2}$ to respectively denote the number of chain vertices and non-chain vertices. We show that when $d_{>2} = O(\log({d_S}))$, which means the chain vertices take a major proportion in $G_S$, the complexity of $N_G$ is reflected by a graphical metric called $F_G$. 

Roughly speaking, $F_G$ measures the product of chains' lengths in the graph. To ease the understanding, we first introduce $F_G$ for the tree structure (Fig.~\ref{fig:complexity_chain_tree} (c)), which does not contain cycles. In a $Y$-rooted tree and a chain $c$ in the tree, we denote $V^{\mathrm{end}}_c$ (resp. $V^{\mathrm{sta}}_c$) as the node of $c$ that has the largest (resp. smallest) distance to $Y$. We say $c' \in \mathrm{Ch}^\prime(c)$ for two chains $c$ and $c'$, if $V^{\mathrm{sta}}_{c'} \in \mathrm{Ch}(V^{\mathrm{end}}_c)$. We introduce $F_G$ and its relation to the complexity as follows: 
%define the parent of a chain $c$ as the chain adjacent to $c$ on the path to the root $Y$. Denote $\mathrm{Pa}^\prime(c), \mathrm{Ch}^\prime(c)$ as the set of $c$'s parent and children, respectively. Then, we have:
\begin{claim}[Tree]
\label{prop:tree-complexity}
For a $Y$-rooted tree, let
\begin{align*}
    F_G:=\prod_{c \in \mathrm{Ch}^{\prime}(Y)} f(c), \,\, f(c):=\mathrm{len}(c)+\prod_{\tilde{c} \in \mathrm{Ch}^{\prime}(c)} f(\tilde{c}).
\end{align*}
Then, {\small $N_G=\mathrm{P}(d_S)$} iff {\small $d_{>2}=O(\mathrm{log}(d_S))$} and {\small $F_G=\mathrm{P}(d_S)$}. 
\end{claim}

For example, in Fig.~\ref{fig:complexity_chain_tree} (c), we have 
$d_{>2}=2$, $\mathrm{Ch}^\prime(Y):=\{c_1, c_2\}$, $\mathrm{Ch}^{\prime}(c_1):=\{c_3, c_4\}$, $\mathrm{Ch}^{\prime}(c_2):=\{c_5, c_6\}$, and the $F_G:=(l_1+l_3 l_4)(l_2+l_5 l_6)$ with $l_i:=\mathrm{len}(c_i)$.


Now, we consider the general cases where $G_S$ has cycles (Fig.~\ref{fig:complexity_chain_tree} (d)). To extend the $F_G$, we can break the cycles via deleting edges and convert $G_S$ into a series of subtrees. Formally, we say $c\in \mathrm{Neig}^\prime(Y)$ for a chain $c$, if there is no other chain node that does not belong to $c$ such that it has a smaller distance than $V^{\mathrm{sta}}_c$ from $Y$. Let $\mathrm{Neig}^\prime(c)=\varnothing$ if $c$ is disjoint with the other chains. For each $k$-length chain $\{c(1),...,c(k)\}:=c\in \mathrm{Neig}^\prime(Y)$, define a set of edge-deletion operators $\mathrm{opt}_c:=\{\text{delete } e_c(1) \text{ to } e_c(i)| i=1,...,\mathrm{len}(c)\}$, where $e_c(i)$ denotes the edge between $c(i-1)$ to $c(i)$ for $i > 1$ or the edge between $Y$ and $c(1)$ for $i=1$. 

\begin{proposition}[Informal] For a stable graph, let
\label{prop:general-complexity}
\begin{align*}
    F_{G}:=\prod_{\substack{c\in \mathrm{Neig}^{\prime}(Y) \\ \mathrm{Neig}^{\prime}(c) = \varnothing}} \mathrm{len}(c) \sum_{\mathrm{opt}\in \prod_{c\in \mathrm{Neig}^{\prime}(Y)}\mathrm{opt}_{c}} F_{\mathrm{opt}(G)},
\end{align*}
Then, {\small $N_G=\mathrm{P}(d_S)$} iff {\small $d_{>2}=O(\mathrm{log}(d_S))$} and {\small $F_G=\mathrm{P}(d_S)$}. 
\end{proposition}

% \begin{remark}
%     When the general graph degenerates to the tree, the $F_G$ defined in Prop.~\ref{prop:general-complexity} is the same as the one defined in Prop.~\ref{prop:tree-complexity}.
% \end{remark}

% This result means when $d_{>2}=O(\mathrm{log}(d_S))$, the equivalent relation can reduce the searching complexity to a polynomial level. 

==> icml23_paras/old_method_mz/complexity_mz_v4.tex <==
\subsection{Searching complexity analysis} 

In the following, we analyze the time complexity of searching $N_G$ equivalence classes. We show that compared to the exponential cost $O(2^{d_S})$ of going over $S^\prime \in \mathrm{Pow}(S)$, our search strategy enjoys a polynomial cost $\mathrm{P}(d_S)$ in cases where the causal graph is sparse. Specifically, split the vertices in $G_S$ into chain vertices and non-chain vertices, with chain vertices (resp. non-chain vertices) referring to those vertices of $\text{deg} \leq 2$ (resp. $\text{deg} > 2$). Denote the number of chain vertices and non-chain vertices as $d_{\leq 2}$ and $d_{>2}$, respectively. Then, we have the following result:
\begin{proposition}[Complexity (informal)]
    \label{prop:complexity(informal)}
    Let $G_S$ the subgraph of $G$ over $\mathbf{X}_S \cup Y$. When the chain vertices in $G_S$ are distributed intensively, $N_G=\mathrm{P}(d_S)$ iff $d_{>2}=O(\log(d_S))$.
\end{proposition}

\textbf{Discussions.} The chain vertices are distributed intensively means they belongs to a few chains (resp. many different chains). Here, a chain is a sequence of adjacent and distinct chain vertices, \emph{e.g.}, $X_1\!-\!X_2\!-\cdots-\!X_l$. This intensive distribution requires the maximum degree of $G_S$ to be bounded by $O(\log(d_S))$. We provide a graphical metric to measure the intensity of chain vertices in the formal version of Prop.~\ref{prop:complexity(informal)}, which is left in Appx.?? due to space limit.


==> icml23_paras/old_method_mz/equivalence_mz_v1.tex <==
\section{Searching $S^*$ among $g$-Equivalence}
\label{sec.learn}

In this section, we provide an optimal subset selection algorithm. Alg.~\ref{alg:identify-f-star} is composed of two parts, respectively inspired by Thm.~\ref{thm:graph degenerate} and Thm.~\ref{thm:min-max}. Specifically, when the graphical condition $Y \not \to \mathbf{W}$ is tested true, Alg.~\ref{alg:identify-f-star} selects the whole stable set $S$ as optimal. When the condition fails, an intuitive strategy is to search all stable subsets and select the one with minimal $\mathcal{L}_{S_-}$, as similarly adopted by \cite{rojas2018invariant,magliacane2018domain,subbaswamy2019preventing,subbaswamy2020spec}. 

However, we find the exhaustive search can be redundant, since some subsets are equivalent in terms of the worst-case risk. Formally, denote the stable graph of $G$ over $\mathbf{X}_S \cup Y$ as $G_S$, we introduce the \emph{g}-equivalence as follows:

\newpage
\begin{algorithm}[tb]
   \caption{Optimal Subset Selection.}
\label{alg:identify-f-star}
\vspace{-0.2cm}
\begin{flushleft}
    \textbf{Input:} The training data $\{D_{e}|e\in\mathcal{E}_{\text{tr}}\}$. \\
    \textbf{Output:} The optimal subset $S^*$.
\end{flushleft}
\vspace{-0.2cm}
\begin{algorithmic}[1]
   \STATE Causal discovery of $G, \mathbf{W}$, and whether $Y \to \mathbf{W}$.
   \STATE \textbf{if} {$Y \not \to \mathbf{W}$} \textbf{then}
        \STATE \quad $S^* \leftarrow S$. \hfill{\# Thm.~\ref{thm:graph degenerate}} 
   \STATE \textbf{else}
    \STATE \quad  Recover $\mathrm{Pow}(S)\backslash\!\sim_G$ by Alg.~\ref{alg: recover g-equivalence}.
    \STATE \quad  $\mathcal{L}_{\min}\leftarrow \infty$.
        \STATE \quad \textbf{for} {$[S_{-}]$ \textbf{in} $\mathrm{Pow}(S)\backslash \!\sim_G$} \textbf{do}
        \STATE \quad \quad \textbf{if} {$\mathcal{L}_{S_{-}} <\mathcal{L}_{\min}$} \textbf{then}
            \STATE \quad \quad \quad $\mathcal{L}_{\min} \leftarrow \mathcal{L}_{S_{-}}$, $S^* \leftarrow S_{-}$. \hfill{\# Thm.~\ref{thm:min-max}} 
            \STATE \quad \quad \textbf{end if}
        \STATE \quad \textbf{end for}
    \STATE \textbf{end if} \textbf{return} $S^*$.
\end{algorithmic}
\end{algorithm}

\begin{definition}[\emph{g}-Equivalence]
    Two subsets $S_-$, $S_+$ are \emph{g}-equivalent if $\exists \, S_{\cap} \subseteq S_- \cap S_+$ \emph{s.t.} $(Y \perp \mathbf{X}_{S_\cap^c} | \mathbf{X}_{S_\cap})_{G_S}$, with $S_\cap^c:=(S_-\cup S_+) \backslash S_\cap$ the complementary set of $S_\cap$. \emph{g}-Equivalent subsets have the same $\mathcal{R}_{S_-}$.
\end{definition}

\begin{remark}
    Denote the \emph{g}-equivalence as $\sim_G$. Call elements of the quotient space $\mathrm{Pow}(S)\backslash\!\sim_G$ as \emph{g}-equivalent classes, and denote their number as $N_G$. Denote the \emph{g}-equivalent class of subset $S_-$ as $[S_-]$.
\end{remark}

Intuitively, two subsets are \emph{g}-equivalent if they share an intersection set $S_\cap$, such that the $S_\cap$ itself is sufficient to provide all information about $Y$ in $S_-$ and $S_+$. In other words, $P(Y|\mathbf{X}_{S_-},do(\boldsymbol{x}_M)) \!=\! P(Y|\mathbf{X}_{S_\cap},do(\boldsymbol{x}_M)) = P(Y|\mathbf{X}_{S_+},do(\boldsymbol{x}_M))$ and thus $\mathcal{R}_{S_-}\!=\!\mathcal{R}_{S_+}$. Graphically, this means $S_\cap$ can block (\emph{i.e.}, \emph{d}-separate) $S_\cap^c$ from $Y$. For example, in the stable graph of Fig.~\ref{fig: example graphical condition} (a), $S_2$ can block $S_2^c:=\{S_1,S_2\}\backslash S_2=S_1$ from $Y$. Thus, we have $S_2 \sim_G \{S_1,S_2\}$ and $\mathcal{R}_{S_2}=\mathcal{R}_{\{S_1,S_2\}}$. 

\begin{algorithm}[h]
   \caption{(Informal) \emph{g}-Equivalence Recovery\protect \footnote{We omit the subscript $S$ for brevity. We only require the input to be Markovian equivalent to $G$. The formal version is at Alg.~\ref{alg: recover g-equivalence detail}.}}
   \label{alg: recover g-equivalence}
\vspace{-0.2cm}
\begin{flushleft}
    \textbf{Input:} The stable graph $G$. \\
    \textbf{Output:} The \emph{g}-equivalent classes $\mathrm{Pow}(S)\backslash\!\sim_G$.
\end{flushleft}
\vspace{-0.2cm}
\begin{algorithmic}[1]
       \FUNCTION{$\text{Recover}(G)$}
        \IF{$\mathrm{Neig}(Y)=\varnothing$}
        \STATE \textbf{return} $\{\mathrm{Pow}(S)\}$.
        \ELSE
        \STATE $\mathrm{Pow}(S)\backslash\!\sim_G \leftarrow \varnothing$.
        \FOR{$S_-$ \textbf{in} $\mathrm{Pow}(\mathrm{Neig}(Y))$}
        \STATE Construct a MAG $\tilde{G}$ from $G$ over $S \backslash \mathrm{Neig}(Y)$, with $S_-$ as the selection set, $\mathrm{Neig}(Y)\backslash S_-$ as the latent set.
        \vspace{+0.1cm}
        \STATE $\mathrm{Pow}(S)\backslash\!\sim_G\text{.add}(\{S_-\} \cup \text{Recover}(\tilde{G}))$.
        \ENDFOR
        \STATE\textbf{return} $\mathrm{Pow}(S)\backslash\!\sim_G$.
        \ENDIF
       \ENDFUNCTION
\end{algorithmic}
\end{algorithm}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{icml23_figs/complexity_chain_tree.pdf}
    \caption{Illustration of the searching complexity. (a) A chain, where $N_G=6+1=7$. (b) A graph consisting disjoint chains, where $N_G=(2+1)^3=27$. (c) A tree consisting six chains, where $F_G=(l_1+l_3 l_4)(l_2+l_5 l_6)$. (d) A graph with cycle can be converted to subtrees by deleting edges to break the cycle, where $c_1^i$ is attained by deleting the $1:i$ edges in $c_1$.}
    \label{fig:complexity_chain_tree}
    \vspace{-0.4cm}
\end{figure}

With \emph{g}-equivalence, we can reduce the exhaustive search over $\mathrm{Pow}(S)$ to a search over $\mathrm{Pow}(S)\backslash\!\sim_G$. To enable the search, we provide a $\mathrm{Pow}(S)\backslash\!\sim_G$ recovery method in Alg.~\ref{alg: recover g-equivalence}. Given the input stable graph, Alg.~\ref{alg: recover g-equivalence} first finds $Y$'s neighbors. When $\mathrm{Neig}(Y)=\varnothing$, all subsets of $S$ are blocked from $Y$ and \emph{g}-equivalent. Thus, the algorithm returns a single \emph{g}-equivalent class $[S]=\mathrm{Pow}(S)$. When $\mathrm{Neig}(Y)\neq \varnothing$, Alg.~\ref{alg: recover g-equivalence} goes over $S_-\subseteq \mathrm{Neig}(Y)$ to include them into the prediction set. It then constructs Maximal Ancestral Graphs (MAGs) over $S\backslash\mathrm{Neig}(Y)$ to explore variable beyond $\mathrm{Neig}(Y)$ and repeats the procedure until $\mathrm{Neig}(Y)$ is empty. We use the MAGs because they can represent \emph{d}-separations when selection (\emph{i.e.}, variables included into the prediction set) and latent (\emph{i.e.}, variables excluded from the prediction set) variables exist.

\begin{proposition}
\label{prop:recover}
    Under Asm.~\ref{eq:assum-markov-faithfulness}, for each input graph that is Markov equivalent to the stable graph $G_S$, Alg.~\ref{alg: recover g-equivalence} can correctly recover the $\mathrm{Pow}(S)\backslash\! \sim_G$ in $O(N_G)$ time.
\end{proposition}





==> icml23_paras/old_method_mz/equivalence_mz_v2.tex <==
\section{Searching $S^*$ among equivalence classes}
\label{sec.learn}

In this section, we provide an optimal subset selection algorithm in Alg.~\ref{alg:identify-f-star} that combines Thm.~\ref{thm:graph degenerate} and Thm.~\ref{thm:min-max}. Specifically, Alg.~\ref{alg:identify-f-star} (line 3) selects the whole stable set as $S^*$, if the graphical condition $Y \not\to \mathbf{W}$ is tested true. If this condition fails, a simple strategy is to \emph{exhaustively} compare the worst-case risk of all subsets, which is commonly adopted in the literature \cite{rojas2018invariant,magliacane2018domain,subbaswamy2019preventing,subbaswamy2020spec}. 

In the following, we will provide a new search strategy with better efficiency, by noticing that the exhaustive search can be redundant for subsets that have the same worst-case risk. Formally, we introduce the equivalence relation as follows:


\begin{definition}[Equivalence relation]
\label{def:equi}
    Let $G_S$ be a causal graph over $\mathbf{X}_S \cup Y$. Let $\sim_G$ be an equivalence relation on all subsets of $S$: two subsets $S^{\prime}, S^{\prime \prime}$ are equivalent if $\exists \, S_{\cap} \subseteq S^\prime \cap S^{\prime \prime}$ s.t.
    \begin{align*}
    Y \ind_{G_S}  \mathbf{X}_{S_\cap^c} | \mathbf{X}_{S_\cap},
    \end{align*}
    with $S_\cap^c:=(S^\prime\cup S^{\prime \prime}) \backslash S_\cap$ the complementary set of $S_\cap$. Here, the $G_S$ can a DAG or a Maximal Ancestral Graph (MAG) \cite{spirtes2000causation}. Accordingly, the $\ind_{G_S}$ denotes \emph{d}-separation or \emph{m}-separation in $G_S$. We call elements of the quotient space $\mathrm{Pow}(S)/\!\sim_G$ as equivalence classes. We use $[S^\prime] :=\{S^{\prime \prime}|S^{\prime \prime} \sim_G S^\prime\}$ to denote the equivalence class of $S^\prime$ and $N_G:=|\mathrm{Pow}(S)/\!\sim_G\!|$ to denote the number of equivalence classes. 
\end{definition}

\begin{algorithm}[tb]
   \caption{Optimal subset $S^*$ selection.}
\label{alg:identify-f-star}
\vspace{-0.1cm}
\begin{flushleft}
    \textbf{Input:} The training data $\{\mathcal{D}_{e}\}_{e\in\mathcal{E}_{\text{tr}}}$.
\end{flushleft}
\vspace{-0.2cm}
\begin{algorithmic}[1]
   \STATE Causal discovery of $G, \mathbf{W}$, and whether $Y \to \mathbf{W}$.
   \STATE \textbf{if} {$Y \not \to \mathbf{W}$} \textbf{then}
        \STATE \quad $S^* \leftarrow S$. \hfill{\# Thm.~\ref{thm:graph degenerate}} 
   \STATE \textbf{else}
    \STATE \quad  Recover $\mathrm{Pow}(S)/\!\sim_G$ with Alg.~\ref{alg: recover g-equivalence}.
    \STATE \quad  $\mathcal{L}_{\min}\leftarrow \infty$.
        \STATE \quad \textbf{for} {$[S^\prime]$ \textbf{in} $\mathrm{Pow}(S)/ \!\sim_G$} \textbf{do}
        \STATE \quad \quad \textbf{if} {$\mathcal{L}_{S^\prime} <\mathcal{L}_{\min}$} \textbf{then}
            \STATE \quad \quad \quad $\mathcal{L}_{\min} \leftarrow \mathcal{L}_{S^\prime}$, $S^* \leftarrow S^\prime$. \hfill{\# Thm.~\ref{thm:min-max}} 
            \STATE \quad \quad \textbf{end if}
        \STATE \quad \textbf{end for}
    \STATE \textbf{end if} 
    \STATE \textbf{return} $S^*$.
\end{algorithmic}
\end{algorithm} 


Intuitively, two subsets $S^\prime$ and $S^{\prime \prime}$ are equivalent if they share an intersection set $S_\cap$ that can blocks (\emph{d}-separate or \emph{m}-separate) vertices in $S_\cap^c$ from $Y$. As a result, we have {$P(Y|\mathbf{X}_{S^\prime},do(\boldsymbol{x}_M)) \!=\! P(Y|\mathbf{X}_{S_\cap},do(\boldsymbol{x}_M)) = P(Y|\mathbf{X}_{S^{\prime \prime}},do(\boldsymbol{x}_M))$} and hence $\mathcal{R}_{S^\prime}\!=\!\mathcal{R}_{S_\cap}\!=\!\mathcal{R}_{S^{\prime \prime}}$. For example, in Fig.~\ref{fig: example graphical condition} (a), we have {$\{X_2\} \sim_G \{X_1,X_2\}$} because {$\mathbf{X}_{S_\cap}=\{X_2\}$} can d-separate {$\mathbf{X}_{S_\cap^c}=\{X_1,X_2\}\backslash \{X_2\}=\{X_1\}$ from $Y$}.

With Def.~\ref{def:equi}, we can reduce the exhaustive search over $\mathrm{Pow}(S)$ to a search over $\mathrm{Pow}(S)/\!\sim_G$. To enable the search, we provide a equivalence classes recovery method in Alg.~\ref{alg: recover g-equivalence}. Given the input graph $G$\footnote{We only require the input to be Markov equivalent to $G$.} \addtocounter{footnote}{-1}\addtocounter{Hfootnote}{-1}, Alg.~\ref{alg: recover g-equivalence} first finds $Y$'s neighbors. If $\mathrm{Neig}(Y)=\emptyset$, then all subsets of $S$ are blocked from $Y$ and hence equivalent. As a result, the algorithm returns $\mathrm{Pow}(S)/\!\sim_G=\{[S]\}$ with a single element $[S]=\mathrm{Pow}(S)$. When $\mathrm{Neig}(Y)$ is not empty, Alg.~\ref{alg: recover g-equivalence} goes over $S^\prime \subseteq \mathrm{Neig}(Y)$ to include them into the selection set. Here, the \emph{selection} set contains variables used to predict $Y$; while the \emph{latent} set contains those excluded from prediction. To explore vertices beyond $\mathrm{Neig}(Y)$, Alg.~\ref{alg: recover g-equivalence} constructs MAGs over $S\backslash\mathrm{Neig}(Y)$ and recursively explore equivalence in the MAGs until $\mathrm{Neig}(Y)$ becomes empty. We use the MAG representation because for disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{X}_{S\backslash \mathrm{Neig}(Y)}$, the MAG $M_G$ can preserve separation properties in $G$, \emph{i.e.}, $\mathbf{A} \ind_{G} \mathbf{B} | \mathbf{Z}, \mathbf{X}_{S^\prime} \Leftrightarrow \mathbf{A} \ind_{M_G} \mathbf{B} | \mathbf{Z}$ \cite{zhang2008completeness}.

\begin{algorithm}[t!]
   \caption{Equivalence classes recovery.}
   \label{alg: recover g-equivalence}
\begin{algorithmic}[1]
       \FUNCTION{$\text{recover}(G)$}
        \IF{$\mathrm{Neig}(Y)=\emptyset$}
        \STATE \textbf{return} $\{\mathrm{Pow}(S)\}$.
        \ELSE
        \STATE $\mathrm{Pow}(S)/\!\sim_G \leftarrow \emptyset$.
        \FOR{$S^\prime$ \textbf{in} $\mathrm{Pow}(\mathrm{Neig}(Y))$}
        \STATE {\small Construct a $\mathrm{MAG}$ $M_G$ over $S \backslash \mathrm{Neig}(Y)$, with $S^\prime$ as the selection set, $\mathrm{Neig}(Y)\backslash S^\prime$ as the latent set.}
        \vspace{+0.05cm}
        \STATE {\small $\mathrm{Pow}(S\backslash \mathrm{Neig}(Y))/\!\sim_{M_G} \leftarrow \textbf{\textbf{recover}}(M_G)$.}
        \vspace{+0.05cm}
        \STATE {\small Add $S^\prime$ to each subset in $\mathrm{Pow}(S\backslash \mathrm{Neig}(Y))/\!\sim_{M_G}$.}
        \STATE {\small $\mathrm{Pow}(S)/\!\sim_G\text{.append}(\mathrm{Pow}(S\backslash \mathrm{Neig}(Y))/\!\sim_{M_G})$.}
        \ENDFOR
        \STATE\textbf{return} $\mathrm{Pow}(S)/\!\sim_G$.
        \ENDIF
       \ENDFUNCTION
\end{algorithmic}
\vspace{-0.1cm}
\begin{flushleft}
\textbf{Input:} The causal graph $G$\footnotemark.
\end{flushleft}
\vspace{-0.2cm}
\begin{algorithmic}[1]
    \STATE Let $G_S$ the subgraph of $G$ over $\mathbf{X}_S\cup Y$.
    \STATE \textbf{return} \textbf{recover}$(G_S)$.
\end{algorithmic}
\end{algorithm}

\begin{example}
    In order to see how Alg.~\ref{alg: recover g-equivalence} works, consider the example shown in Fig.~\ref{fig:alg_recover_example}. In $G_S$, we have $\mathrm{Neig}(Y)=\{X_1,X_3\}$. Hence, Alg.~\ref{alg: recover g-equivalence} goes over $S^\prime \in \{\{X_1,X_3\},\}\{X_1\},\{X_3\},\emptyset\}$ in the first recursion level. The induced MAGs are respectively shown in Fig.~\ref{fig:alg_recover_example} (a)-(b), by noticing that \textbf{i)}$X_1$ is a non-collider on any path through it, which means once $X_1$ is in the selection set, any path through $X_1$ will be blocked; \textbf{ii)} $X_2$ is a collider, which means any path through $X_2$ will be blocked if $X_2$ is in the latent set. Further, for the MAG in (a), we have $\mathrm{Neig}(Y)=\{X_4\}$ and the induced subMAGs for $S^\prime=\{X_4\}$ and $\emptyset$ in (e). In Fig.~\ref{fig:alg_recover_example} (e), $\mathrm{Neig}(Y)$ becomes empty, which means we have two equivalence classes $[X_1,X_3,X_4]$ and $[X_1,X_3]$. For the MAG in (b), we have $\mathrm{Neig}(Y)=\emptyset$ and hence one equivalence class $[X_1]$. For the MAGs in (c) and (d), the $\mathrm{Neig}(Y)$ are both $\{X_2,X_4\}$. We show the induced subMAGs in Fig.~\ref{fig:alg_recover_example} (f), which indicates there are four equivalence classes in (c) ($[X_2,X_3,X_4],[X_2,X_3],[X_3,X_4],[X_3]$) and four equivalence classes (d) ($[X_2,X_4],[X_2],[X_4],[\emptyset]$). To summery, there are in total $7$ equivalent classes out of the $2^5=32$ subsets. Details are left in Appx.??.
\end{example}



\begin{proposition}
\label{prop:recover}
    Under Asm.~\ref{eq:assum-markov-faithfulness}, for each input graph that is Markov equivalent to the ground-truth $G$, Alg.~\ref{alg: recover g-equivalence} can correctly recover the $\mathrm{Pow}(S)/\! \sim_G$ in $O(N_G)$ time.
\end{proposition}


\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{icml23_figs/alg_recover_example.pdf}
    \vspace{+0.05cm}
    \caption{An example for Alg.\ref{alg: recover g-equivalence}. The stable and mutable variables are marked blue and red, respectively.}
    \label{fig:alg_recover_example}
\end{figure}




==> icml23_paras/old_method_mz/experiment.tex <==
\section{Experiment}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.55\columnwidth]{icml23_figs2/synthetic_causal_graph.pdf}
%     \caption{The causal graph for synthetic data generation. Stable and mutable variables are respectively marked blue and red. The dashed line $X_{M_1} \to X_1$ does not exist (resp. exist) in setting-1 (resp. setting-2).}
%     \label{fig:synthetic_causal_graph}
% \end{figure}

\begin{table*}[t!]
\caption{Evaluation on synthetic and ADNI datasets. The first column notes the methods we compare. The second and third columns respectively represent the maximal MSE and standard deviation of MSE over deployment environments. The best results are \textbf{boldfaced}.}
    \label{tab: numerical value, sythetic and ad}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Method} &  \multicolumn{3}{c|}{max. MSE ($\downarrow$)} & \multicolumn{3}{c}{std. MSE ($\downarrow$)}\\
    \cline{2-7} 
     & Syn1 & Syn2 & ADNI & Syn1 & Syn2 & ADNI \\
    \hline
    Vanilla & $1.336_{\pm 0.4}$ & $1.861_{\pm 0.4}$ & $1.399_{\pm 0.1}$ & $0.240_{\pm 0.2}$ & $0.481_{\pm 0.1}$ & $0.299_{\pm 0.0}$ \\ 
    ICP \cite{peters2016causal} & $1.855_{\pm 0.7}$ & $2.331_{\pm 0.2}$ & $1.176_{\pm 0.0}$ & $0.130_{\pm 0.1}$ & $0.230_{\pm 0.0}$ & $0.155_{\pm 0.0}$  \\ 
    IC \cite{rojas2018invariant}  & $1.211_{\pm 0.4}$ & $1.254_{\pm 0.1}$ & $1.165_{\pm 0.2}$ &  $0.176_{\pm 0.2}$ & $0.194_{\pm 0.1}$ & $0.198_{\pm 0.1}$\\ 
    DRO \cite{sinha2018certifiable}  & $1.364_{\pm 0.5}$ & $1.495_{\pm 0.1}$ & $1.181_{\pm 0.0}$ & $0.250_{\pm 0.2}$ & $0.326_{\pm 0.0}$ & $0.145_{\pm 0.0}$  \\ 
    Surgery \cite{subbaswamy2019preventing}  & ${0.926_{\pm 0.0}}$ & $1.101_{\pm 0.1}$ & $1.069_{\pm 0.1}$ & ${0.028_{\pm 0.0}}$ & $0.057_{\pm 0.0}$ & $0.129_{\pm 0.0}$  \\ 
    \hline
    IRM \cite{arjovsky2019invariant}  & $1.106_{\pm 0.2}$ & $1.246_{\pm 0.1}$ & $1.223_{\pm 0.0}$ & $0.127_{\pm 0.1}$ & $0.164_{\pm 0.1}$  & $0.177_{\pm 0.0}$ \\ 
    HRM \cite{liu2021heterogeneous}  & $0.975_{\pm 0.0}$ & $1.494_{\pm 0.1}$ & $1.272_{\pm 0.1}$ & $0.046_{\pm 0.0}$ & $0.312_{\pm 0.1}$ & $0.194_{\pm 0.1}$  \\ 
    IB-IRM \cite{ahuja2021invariance}  & $1.076_{\pm 0.0}$ & ${1.079_{\pm 0.0}}$ & $1.222_{\pm 0.2}$ & $0.056_{\pm 0.0}$ & $0.040_{\pm 0.0}$ & $0.113_{\pm 0.1}$  \\ 
    AncReg \cite{rothenhausler2021anchor}  & $0.938_{\pm 0.0}$ & $1.377_{\pm 0.2}$ & $1.138_{\pm 0.1}$ & $0.033_{\pm 0.0}$ & $0.257_{\pm 0.1}$ & $0.159_{\pm 0.0}$ \\ 
    \hline
    Ours (Alg.~\ref{alg:identify-f-star})  & $\mathbf{0.926_{\pm 0.0}}$ & $\mathbf{1.079_{\pm 0.0}}$ & $\mathbf{0.890_{\pm 0.1}}$ & $\mathbf{0.028_{\pm 0.0}}$ & $\mathbf{0.034_{\pm 0.0}}$ & $\mathbf{0.038_{\pm 0.0}}$ \\ 
    \hline
    \end{tabular}}
\end{table*}


\begin{table}[t!]
\caption{Verification of equivalence relation on synthetic data.}
    \label{tab: numerical value, sythetic and ad}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c c}
    \hline
    Metric \quad \quad \quad \quad  & Value \\
    \hline
     Inter-class std. \quad \quad \quad \quad  & $1.000$ \\
     Intra-class std. \quad \quad \quad \quad  & $0.008$ \\
    \hline
    \end{tabular}}
\end{table}


We evaluate our method on synthetic data and a real-world application, \emph{i.e.}, diagnosis of Alzheimer's disease\footnote{We consider an extra task of gene function prediction in Appx.??}.

\noindent \textbf{Compared baselines.} We compare our methods with the following baselines: \textbf{i)} Vanilla that uses $\mathbb{E}[Y|x]$ to predict $Y$; \textbf{ii)} ICP \citep{peters2016causal} that assumed and utilized the invariance of parental features $P(Y|\mathbf{Pa}(Y))$; \textbf{iii)} IC \citep{rojas2018invariant} that extended ICP to features beyond $\mathbf{Pa}(Y)$; \textbf{iv)} DRO \cite{sinha2018certifiable} that constrained the distance between training and deployment distributions and conducted optimization for minimax optimum; \textbf{v)} Surgery estimator \cite{subbaswamy2019preventing} that used validation's loss to identify the optimal subset. \textbf{vi)} IRM \citep{arjovsky2019invariant} that learned an invariant representation to transfer; \textbf{vii)} HRM \citep{liu2021heterogeneous} that extended IRM to the case with unknown environment indices, by exploring the heterogeneity in data via clustering; \textbf{viii)} IB-IRM \citep{ahuja2021invariance} that leveraged the information bottleneck regularization to supplement the invariance principle in IRM; and \textbf{ix)} Anchor regression \citep{rothenhausler2021anchor} that interpolated between ordinary least square (LS) and causal minimax LS.

\noindent \textbf{Implementation details.} We use two-layer nonlinear neural networks to parameterize $f_{S^\prime}$ and $h_\theta$. More details are left in Appx.~\ref{sec. appendix-exp}. 

\subsection{Synthetic data}

\noindent\textbf{Data generation.} We follow the causal graph in Fig.~\ref{fig:simg3_ad_causal_graphs} (a) and the following structural equations to generate data: {\small $V_i = \alpha_i^e g_i\left(\sum_{V_j \in \mathbf{Pa}(V_i)} \beta_{i,j} V_j\right) + \epsilon_i$}, where the coefficient $\alpha_i^e$ keeps constant, \emph{i.e.}, $\alpha_i^e \equiv \alpha_i$ for all $e$ if $V_i$ is a stable variable; or varies with $e$ if $V_i$ is a mutable variable. For each $i$, the function $g_i$ is randomly chosen from $\{\mathrm{identity}, \mathrm{tanh}, \mathrm{sinc}, \mathrm{sigmoid}\}$. The linear parameters $\beta_{i,j}$ is randomly drawn from a uniformed distribution $\mathcal{U}([-2,-0.5]\cup [0.5,2])$ and the noise item $\epsilon_i$ follows $\mathcal{N}(0,0.1)$. We generate $20$ environments and $n_e=100$ samples in each environment. To remove the randomness effect, we repeat for $5$ times: each time we randomly pick $10$ environments for training and others for testing. 


We consider two different settings, with the graphical condition holds (resp. not hold) in setting-1 (resp. setting-2). Specifically, according to the definition, $\mathbf{X}_M^0$ refers to $M_1$. In setting-1, the dashed line $M_1 \to S_1$ does not exist, hence $\mathbf{W}$ is empty and the graphical condition $Y \not\to \mathbf{W}$ in Thm.~\ref{thm:graph degenerate} holds. In this regard, the whole stable set is expected to be optimal. In setting-2, the edge $M_1 \to S_1$ exists, hence $\mathbf{W}:=\{S_1,S_2,S_3,S_4,M_2\}$ and $Y \to \mathbf{W}$ that violates the graphical condition. According to Alg.~\ref{alg:identify-f-star}, we select $S^*$ with minimal population loss on $\{P_h\}_{h\in \mathcal{B}}$. 


\noindent\textbf{Results analysis.} We report the maximal mean square error (\emph{a.k.a}, max. MSE) and the standard deviation of MSE (\emph{a.k.a}, std. MSE) over test environments in Tab.~\ref{tab: numerical value, sythetic and ad}. As shown, our methods outperform others in all settings, indicating better robustness (max. MSE) and stability (std. MSE) than other methods. Besides, we report the max. MSE of different subsets in Fig.~\ref{fig:simg3_scatters_search_cost}. As shown, in setting-1, the whole stable set $S$ has minimal max. MSE as expected; in setting-2, the subset $\{X_7\}$ with minimal population loss on $P_h$ also has the minimal max. MSE over test environments. Besides, we can observe that the max. MSE shows an approximate increasing trend in subsets ranked by our method, however a decreasing one in those ranked by the surgery estimator. This observation suggests that, compared with the heuristic validation loss, our method can be more consistently reflective of the worst-case risk.


\textbf{Analysis of equivalence relation} To show to effectiveness of Alg.~\ref{alg: recover g-equivalence} in recovering equivalence classes, we compute the \emph{intra-class standard deviation}, and compare it with \emph{inter-class std}, in terms of max. MSE. For intra-class std., we first compute the standard deviation max. MSE over all subsets in each equivalence class, and take the average over all equivalence classes. For inter-class std, we first compute the average max. MSE over all subsets in each equivalence class; then we compute the std. of the mean max. MSE over equivalence classes. In Fig.~\ref{fig: std g-equivalence} (Synthetic), we observe that the intra-class std. is much smaller than the inter-class std. This result suggests that our learned equivalent subsets have comparable performance, which enables us to search over equivalence classes rather than all subsets. 


\begin{table}[t!]
\caption{Comparison of computation complexity on ADNI dataset.}
    \label{tab:ad search cost}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c c c}
    \hline
    Method & Searching cost & Time \\
    \hline
    Exhaustive ($\mathrm{Pow}(S)$) & $2^{25}$ & about 6.4y\\
    Ours ($\mathrm{Pow}(S)/\!\sim_G$) & $25307$ & 42h\\
    \hline
    \end{tabular}}
\end{table}

\textbf{Searching complexity analysis.} We first generate a sequence of causal graphs $G_1$-$G_5$ as $d_{\geq 3}$ grows, by adding edges in the graph shown in Fig. 3 (\emph{i.e.}, $G_3$); and then compute the searching cost for these graphs. We can see in Fig.~\ref{fig:simg3_scatters_search_cost} (c) that \textbf{i}) compared with exhaustively searching over all subsets, our method can significantly save the searching cost in both sparse and dense graphs; \textbf{ii}) the searching cost among equivalence classes decreases when as $d_{\geq 3}$ decreases. 

% \begin{figure}[b!]
%     \centering
%     \includegraphics[width=\columnwidth]{icml23_figs2/ad25_causal_graph.pdf}
%     \caption{The learned causal graph on ADNI. Stable and mutable variables are respectively marked blue and red. The target (FAQ) and demographics (ApE, GEN, EDU) are placed in the bottom right. Brain regions are placed at their positions in the brain.}
%     \label{fig:ad25_causal_graph}
% \end{figure}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{icml23_figs2/synthetic_results.pdf}
    \caption{Results on synthetic data. (a) Setting-1: max. MSE of different subsets, where the whole stable set $S$ is optimal. (b) Setting-2: max. MSE of subsets ranked in the ascending order from left to right, respectively according to the estimated $\mathcal{L}_{S_{-}}$ of our method and the validation's loss of the surgery estimator. (c) Comparison of Searching cost when $d_{\geq 3}$ increases.}
    \label{fig:simg3_scatters_search_cost}
\end{figure*}

\subsection{Alzheimer's disease diagnosis}

We evaluate our method on Alzheimer's Disease Neuroimaging Initiative (ADNI) dataset \cite{petersen2010alzheimer}. 

\noindent\textbf{Dataset \& preprocessing.} In ADNI dataset, we consider structural Magnetic Resonance Imaging (sMRI) data. We apply Dartel VBM \cite{ashburner2007fast} for data processing and Statistical Parametric Mapping (SPM) for segmenting the brain regions. Then we implement the Automatic Anatomical Labeling (AAL) atlas \cite{tzourio2002automated} and region indices provided by \cite{young2018uncovering} to partition the whole brain into nine regions: frontal lobe (FL), medial temporal lobe (MTL), parietal lobe (PL), occipital lobe (OL), cingulum (CIN), insula (INS), amygdala (AMY), hippocampus (HP), and pallidum (PL). In addition to brain volumes, other covariates include age, gender (GED), and the number of ApoE-4 alleles (ApE) that have been found to be highly correlated with AD. With these covariates, we predict the Functional Activities Questionnaire (FAQ) score \cite{mayo2016use} for each patient. We split the dataset into seven environments according to age ($<$60, 60-65, 65-70, 70-75, 75-80, 80-85, $>$85), which respectively contain $n_e=27,59,90,240,182,117,42$ samples. We repeat 15 times, with each time randomly taking four environments for training and the rest for testing. 

\noindent\textbf{Causal discovery and $\mathrm{Pow}(S) \!/\!\sim_G\!$ recovery.} The learned causal graph is shown in Fig.~\ref{fig:simg3_ad_causal_graphs} (b). As we can see, the affection of AD (\emph{i.e.}, FAQ) first shows in the medial temporal lobe (MTL) and hippocampus (HP), then propagates to other brain regions, which echos existing studies that MTL and HP are early degenerated regions \cite{barnes2009meta,duara2008medial}, Besides, we observe that the frontal lobe (FL), pallidum (PAL), and hippocampus (HP) are mutable regions, which agrees with the heterogeneity found in different age groups \cite{cavedo2014medial,fiford2018patterns}. We can also observe that $Y$ (FAQ) points to $\mathbf{W}$ that is \{MTL\} according to the definition. This means the graphical condition in Thm.~\ref{thm:graph degenerate} does not hold. Thus, we need to search among equivalence classes to find the optimal subset. Applying Alg.~\ref{alg: recover g-equivalence}, we find there are $42$ equivalence classes out of the $2^8$ subsets ($|S|=8$ as shown in Fig.~\ref{fig:simg3_ad_causal_graphs} (b)). 


\noindent\textbf{Results analysis.} Fig.~\ref{fig:adni-intro} (a) shows the max. MSE of our method and baselines. As we can see, our method can outperform the others significantly, which demonstrates the effectiveness of Thm.~\ref{thm:min-max} in optimal subset selection. To explain the improvement over the surgery estimator,  we present a scatter plot in Fig.~\ref{fig:adni-intro} (b) to show the maximal MSE over test environments (\emph{a.k.a}, max. MSE) for all subsets ranked by $\mathcal{L}_{S^\prime}$ of our method (resp. validation's loss of the surgery estimator) marked as red (resp. blue). As shown, the sequence of subsets $\mathcal{L}_{S^\prime}$ appears a positive correlation with the true worst-case risk; in contrast, the correlation is negative for the validation loss in the surgery estimator. Particularly, the top subset selected by our method (\{OL,INS\}) also has the minimal max. MSE; while the surgery estimator fails to identify the optimal subset. This example shows the effectiveness of our method in reflecting the worst-case risk; and besides, is a showcase of the failure of the validation's loss in finding the optimal subset in real-world scenarios. The improvements over ICP, IC, IRM and their extensions can be attributed to the property use of stable information beyond causal features/representations. The advantage over DRO is due to the ability of our method to guarantee robustness beyond bounded distributional shifts; while the advantage over Anchor Regression may be due to the relaxation of the linearity assumption.

 
%\textbf{Analysis of equivalence relation.} Similar to the numerical experiment, we 
%compute the intra-class std versus the inter-class std and can see from  Fig.~\ref{fig: std g-equivalence} (ADNI) that equivalent subsets have comparable max. MSE.  







==> icml23_paras/old_method_mz/method_1.tex <==
\section{Methodology}
\label{sec.methd}

In this section, we introduce our method to select the optimal subset. We firstly establish theoretical results regarding the minimax properties in Sec.~\ref{sec.identify}. Then, guided by the theoretical analysis, we in Sec.~\ref{sec.learn} provide an efficient algorithm for optimal subset selection. Finally, we discuss the complexity of the selection algorithm in Sec.~\ref{sec.complex}.

\subsection{Minimax Analysis} 
\label{sec.identify}

In this section, we establish theoretical results regarding the robustness aspect. Our results answer two key questions: \textbf{i)} In which kind of causal DAG does the whole stable set $S$ reach the minimax optimum? \textbf{ii)} When $S$ may not be optimal, how to \emph{consistently} measure the robustness of each subset on (infinitely many) deployment environments, using only data from a few training environments?

In the following, we first provide the answer to the first question. We find whether the interventional distribution can degenerate is decided by connections between $Y$ and a vertices set $\mathbf{K}$ in the causal DAG. If $Y$ does not point to any member of $\mathbf{K}$, the \emph{do} in $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can be removed and the minimax optimum is reached by the whole stable set $S$. 

\begin{theorem}[Graphical Condition for $S^*\!=\!S$]
\label{thm:graph degenerate}
Suppose Asm~\ref{eq:assum-dag},~\ref{eq:assum-markov-faithfulness} hold. Denote $\mathbf{X}_{M}^{0}\!:=\!\mathbf{X}_{M}\cap \mathrm{Ch}(Y)$ as mutable variables in $Y$'s children, and $\mathbf{K}:=\mathrm{De}(\mathbf{X}_{M}^{0}) \backslash \mathbf{X}_M^0$ as descendants of $\mathbf{X}_{M}^{0}$. Then, $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution if and only if $Y$ does not point to any member of $\mathbf{K}$. Further, under either of the two conditions, $S^*=S$.
\end{theorem}
\vspace{-0.1cm}
\begin{proofsketch}
    If $Y$ does not point to any member of $\mathbf{K}$, we can use the inference rules \cite{pearl2009causality} to remove the ``\emph{do}'' in $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ and degenerate it into $P(Y|\mathbf{X}\backslash (\mathbf{X}_M^0 \cup \mathrm{De}(\mathbf{X}_M^0)))$. For example, in Fig.~\ref{fig: example graphical condition} (a), we have $P(Y|X_1,X_2, do(\boldsymbol{X}_m))=P(Y|X_2, do(\boldsymbol{x}_m))=P(Y|X_2)$. Such a degeneration (to conditional distribution) permits us to construct a probability distribution in $\{P^e| e \in \mathcal{E}\}$ for any predictor $f$, where $f$ has a larger or equal worst-case risk than $f_S$, thus proving the optimality of $S$. On the contrary, when $Y$ points to a member of $\mathbf{K}$, there is a collider ($X_1$ in Fig.~\ref{fig: example graphical condition} (b)) in $\mathbf{X}\backslash \mathbf{X}_M^0$ in some paths between $Y$ and $\mathbf{X}_M^0$. Conditioning on the collider will open the indirect path between $Y$ and $\mathbf{X}_M^0$, making it incapable to remove the ``\emph{do}''.
\end{proofsketch} 
\vspace{-0.1cm}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\columnwidth]{icml23_figs/fig_examples_thm3.1.pdf}
    \caption{Illustration of the graphical condition in Thm.~\ref{thm:graph degenerate}, with $\mathbf{K}$ marked as blue.}
    \label{fig: example graphical condition}
\end{figure}

Thm.~\ref{thm:graph degenerate} for the first time connects a minimax property to a specific graphical structure. Such a connection provides an intuitive explanation for the robustness of the whole stable set. It also saves end-users from running the inference rules to check the degeneration condition and makes the result easily accessible from the causal DAG, as guaranteed by the following proposition.

\begin{proposition}
	\label{prop.thm3.2 justifiability}
	Under Asm.~\ref{eq:assum-dag},~\ref{eq:assum-markov-faithfulness}, the subset $\mathbf{K}$ and whether $Y \to \mathbf{K}$ is identifiable.
\end{proposition}

On the other hand, Thm.~\ref{thm:graph degenerate} reminds us the sufficient condition for $S^*\!=\!S$ may not always hold. When the condition fails, including more stable information may not be always beneficial. Indeed, we provide a counter-example in Fig.~\ref{fig: example graphical condition} (b) that, the whole stable set ${\{X_2\}}$ has a larger generalization error than the empty set ${\varnothing}$, under some conditions\footnote{For details of these conditions, please refer to Sec. in the appendix.}on $P(Y)$ and $P(X_1|Y)$.

To identify the $S^*$ when Thm.~\ref{thm:graph degenerate} fails, we attempt to measure the robustness of each subset $S_{-}$ with data from $\mathcal{E}_{tr}$. Indeed, there are infinitely many deployment environments, each having various behaviors in terms of the probability distribution. A few held-out validation environments from $\mathcal{E}_{tr}$ are hard, if not impossible, to reflect the behavior of the worst-case environment and measure the worst-case risk. 

Our key observation to solve this problem is that all environments in $\mathcal{E}$, no matter how various their behaviors are, are governed by the causal DAG $G$, where the only source of variation is the mutable causal mechanisms of $\mathbf{X}_M$. In this regard, we can parameterize these mutable mechanisms and let them vary arbitrarily, which provides a simulation of the worst-case environment. Each subset's generalization ability on this simulation environment can thus \emph{consistently} reflect its robustness on $\mathcal{E}$. 

What makes the parameterization plausible is that we find $\mathbf{X}_M$ is always a \emph{definite} function of $\mathrm{Pa}(\mathbf{X}_M)$ when the worst-case risk is attained. In this regard, we can parameterize $J\!:\!\mathrm{Pa}(\mathbf{X}_M)\!\to\!\mathbf{X}_M$ with a neural network $J_\theta$ and maximize over $\theta$ to estimate the worst-case risk, due to its ability to approximate any definite function \cite{hornik1989multilayer}. Formally, define an instrumental distribution family $\{P_J\}_{J}$, with $J$ a definite function from $\mathrm{Pa}(\mathbf{X}_M)$ to $\mathbf{X}_M$ and $P_J\! :=\! P(Y,\mathbf{X}_S| do(\mathbf{X}_M\!=\!J(\mathrm{Pa}(\mathbf{X}_M)))$, we have the following minimax property:

\begin{theorem}[Minimax Property]
\label{thm:min-max}
For a subset $S_{-}$, denote $\mathcal{R}(S_{-})\!:=\!\max_{e \in \mathcal{E}} \mathbb{E}_{P^e}[\left(Y \!-\! f_{S_{-}}(\boldsymbol{x})\right)^2]$ as the worst-case risk on $\mathcal{E}$. Denote $\mathcal{L}(S_{-}):=\max_{J}\mathbb{E}_{P_J}[(Y \!-\! f_{S_{-}}(\boldsymbol{x}))^2]$ as the maximal population loss over $P_J$. Then, we have $\mathcal{R}(S_{-})=\mathcal{L}(S_{-})$. Thus, the optimal subset can be obtained via $S^* := \mathop{\mathrm{argmin}}_{S_{-} \subseteq S} \mathcal{L}(S_{-})$.
\end{theorem}

\begin{proofsketch}
Firstly consider the case where $\mathbf{X}_M=\{X_m\}$. The $\mathcal{R}(S_{-})$ expands to:
\begin{equation}
    \mathcal{R}(S_{-}) = \max_{e \in \mathcal{E}} \int_{y,\boldsymbol{x}} [y-f_{S_{-}}(\boldsymbol{x})]^2 p^e(y,x_m,\boldsymbol{x}_{S_{-}}) dy d\boldsymbol{x}.
\label{eq: risk}
\end{equation}
Factorize $p^e(y,x_m,\boldsymbol{x}_S)$ into disentangled causal factors and denote $\tilde{\mathbf{X}}:=\mathbf{X}\backslash (\{X_m\}\cup \mathrm{Pa}(X_m))$, we can split the integral into three parts, respectively over $\mathrm{pa}(x_m)$, $x_m$, and $y, \tilde{\boldsymbol{x}}$. Denote the last one as $g(x_m,\mathrm{pa}(x_m)):=\int_{y, \tilde{\boldsymbol{x}}} [y-f_{S_{-}}(\boldsymbol{x})]^2 p(y|\mathrm{pa}(y)) p(\tilde{\boldsymbol{x}}| \mathrm{pa}(\tilde{\boldsymbol{x}})) dyd\tilde{\boldsymbol{x}}$, Eq.~\ref{eq: risk} becomes:
\begin{align}
    &\mathcal{R}(S_{-}) = \max_{e \in \mathcal{E}} \int_{\mathrm{pa}(x_m)} \prod_{X_i \in \mathrm{Pa}(X_m)} p(x_i|\mathrm{pa}(x_i)) \nonumber \\ 
    &\int_{x_m} g(x_m,\mathrm{pa}(x_m)) p^e(x_m|\mathrm{pa}(x_m)) dx_m d \mathrm{pa}(x_m).
\end{align}
Since $p^e((x_m|\mathrm{pa}(x_m)))$ is the only item varying with $e$, we can move the maximization to the inner integral and have:
\begin{align}
    \mathcal{R}(S_{-})=&\int_{\mathrm{pa}(x_m)} \prod_{X_i \in \mathrm{Pa}(X_m)} p(x_i|\mathrm{pa}(x_i)) \nonumber \\ 
    &g(J^*(\mathrm{pa}(x_m)),\mathrm{pa}(x_m)) d \mathrm{pa}(x_m),
\label{eq: definite function}
\end{align}
with $J^*(\mathrm{pa}(x_m))\!:=\!\arg\max_{x_m}g(x_m,\mathrm{pa}(x_m))$ is a definite function from $\mathrm{pa}(x_m)$ to $x_m$. Eq.~\ref{eq: definite function} indicates the worst-case risk is attained when $x_m$ is a definite function of $\mathrm{pa}(x_m)$ and thus shows $\mathcal{R}(S_{-})=\mathcal{L}(S_{-})$.

In cases where $\mathbf{X}_M$ contains multiple variables, we can consider the maximization sequentially according to the topology order in $\mathbf{X}_M$. For details of the proof, please refer to Sec. in the appendix.
\end{proofsketch}

The tractability of the optimization over $J_\theta$ is assured by the following proposition on structural identifiability.

\begin{proposition}
	\label{prop.thm3.3 justifiability}
	Under Asm.~\ref{eq:assum-dag},~\ref{eq:assum-markov-faithfulness}, the $\mathbf{X}_M, \mathrm{Pa}(\mathbf{X}_M),$ $\mathrm{De}(\mathbf{X}_M), P_J$, and $f_{S_{-}}$ are identifiable. 
\end{proposition}


==> icml23_paras/old_method_mz/method_2.tex <==
\subsection{The Selection Algorithm}
\label{sec.learn}

\begin{algorithm}[tb]
   \caption{Optimal Subset Selection.}
\label{alg:identify-f-star}
\begin{flushleft}
    \textbf{Input:} The training data $\{D_{e}|e\in\mathcal{E}_{\text{Tr}}\}$. \\
    \textbf{Output:} The optimal subset $S^*$ and predictor $f^*$.
\end{flushleft}
\begin{algorithmic}[1]
   \STATE Causal discovery of $G, \mathbf{K}$ and whether $Y \to \mathbf{K}$.
   \IF{$Y \not \to \mathbf{K}$}
        \STATE $S^* \leftarrow S, f^* \leftarrow f_S$. \hfill{\# Thm.~\ref{thm:graph degenerate}} 
   \ELSE
        \STATE $\mathcal{L}_{\min}\leftarrow \infty$.
    \STATE Recover $\mathrm{Pow}(S)\backslash \sim_G$. \hfill{\# Alg.~\ref{alg: recover g-equivalence}}
        \FOR{$[S_{-}]$ in $\mathrm{Pow}(S)\backslash \sim_G$}
            %\STATE Estimate $\mathcal{L}(S_{-})$.
            \IF{$\mathcal{L}(S_{-})<\mathcal{L}_{\min}$}
                \STATE $\mathcal{L}_{\min} \leftarrow \mathcal{L}(S_{-})$.
                \STATE $S^* \leftarrow S_{-}, f^* \leftarrow f_{S_{-}}$. \hfill{\# Thm.~\ref{thm:min-max}} 
            \ENDIF
        \ENDFOR
    \ENDIF
    \STATE \textbf{return} $S^*, f^*$.
\end{algorithmic}
\end{algorithm}
\vspace{-0.2cm}

In this section, we provide an optimal subset selection algorithm under the guidance of Thm.~\ref{thm:graph degenerate} and Thm.~\ref{thm:min-max}. Given data from $\mathcal{E}_{tr}$, this algorithm firstly recovers the causal structures, including the causal graph, the components $\mathbf{X}_M, \mathbf{K}, \mathrm{Pa}(\mathbf{X}_M)$ and $\mathrm{De}(\mathbf{X}_M)$. It then checks whether $Y \to \mathbf{K}$. If $Y$ does not point to any member of $\mathbf{K}$, the algorithm sets $S$ as the optimal subset according to Thm.~\ref{thm:graph degenerate}; Otherwise, it searches over subsets to find the one with minimal $\mathcal{L}(S_{-})$ as the optimal subset, according to Thm.~\ref{thm:min-max}. 

In previous methods \cite{rojas2018invariant,magliacane2018domain,subbaswamy2019preventing,subbaswamy2020spec}, such a search went through the power set of $S$ and was inevitably $\mathrm{NP}$-$\mathrm{hard}$. However, we find searching exhaustively is redundant and the cost can be reduced to $\mathrm{P}$ in some cases. Specifically, there are subsets with the same prediction power and can be grouped together to reduce the cost. For example, in Fig.~\ref{fig: example graphical condition} (a), the subsets $\{X_2\}$ and $\{X_1,X_2\}$ are equivalent, because $X_2$ and $do(x_m)$ block all the paths between $Y$ and $X_1$, and thus $P(Y|X_2,do(x_m))=P(Y|X_1,X_2,do(x_m))$ under Asm.~\ref{eq:assum-markov-faithfulness}. Formally speaking, denote $G^s$ as the stable graph after removing $\mathbf{X}_M$ from $G$, we define the \emph{g}-equivalent relation between subsets as follows.

\begin{definition}[\emph{g}-Equivalence]
    Two subsets $S_i, S_j$ are \emph{g}-equivalent if $\exists S_{ij} \!\subseteq\! S_i \!\cap\! S_j$ s.t. $(Y \!\perp\! \mathbf{X}_{i} \cup \mathbf{X}_{j} \backslash \mathbf{X}_{{ij}} | \mathbf{X}_{{ij}})_{G^s}$\footnote{We omit the subscript $S$ in $\mathbf{X}_{S_i}$ for brevity.}. Denote the \emph{g}-equivalence as $\sim_G$, then elements of the quotient space $\mathrm{Pow}(S)\backslash\!\sim_G$ are called \emph{g}-equivalent classes. We denote the \emph{g}-equivalent class of $S_{-}$ as $[S_{-}]$.
\end{definition}

\begin{remark}
    Under Asm.~\ref{eq:assum-markov-faithfulness}, $S_i \sim_G S_j \Rightarrow f_{S_i}=f_{S_j}$, because $P(Y|\mathbf{X}_{i}, do(\boldsymbol{x}_M))=P(Y|\mathbf{X}_{j}, do(\boldsymbol{x}_M))$.
\end{remark}

In this regard, it suffices to search over $\mathrm{Pow}(S)\backslash\!\sim_G$ to find the optimal subset and the cost can be reduced from $O(2^{d_S})$ to $O(N_G)$, with $d_S:=|S|$ and $N_G:=|\mathrm{Pow}(S)\backslash\!\sim_G|$. To enable the search, we need to recover the quotient space $\mathrm{Pow}(S)\backslash\!\sim_G$. This can be done via checking the conditional independence (CI) in $G$, as shown in Alg.~\ref{alg: recover g-equivalence}. Specifically, the algorithm recursively adds stable variables into the prediction set in the order of their distance to $Y$. During each recursion level, it creates sub-graphs to represent the CI after including/excluding some variables to/from the prediction set. These sub-graphs are constructed as the maximal ancestral graph (MAG) \cite{spirtes2000causation}, due to its ability to preserve the CI when included (\emph{i.e.}, selected) or excluded (\emph{i.e.}, latent) variables exist.

\begin{algorithm}[!h]
   \caption{Quotient Space Recovery.}
   \label{alg: recover g-equivalence}
\begin{flushleft}
    \textbf{Input:} The causal graph $G$.\\
    \textbf{Output:} The quotient space $\mathrm{Pow}(S)\backslash\!\sim_G$.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE Let $G^s$ the stable graph after removing $\mathbf{X}_M$ in $G$.
    \STATE \textbf{return} $\mathrm{Recover}(G^s)$.
    \vspace{+0.05cm}
    \FUNCTION{$\text{Recover}(G)$}
        \STATE Let $S$ the stable set of $G$.
        \IF{$\mathrm{Neig}_G(Y)=\varnothing$}
            \STATE \textbf{return} $\{\mathrm{Pow}(S)\}$. \hfill{\# All subsets are equivalent}
        \ELSE
            \STATE $P_G \leftarrow \varnothing$. \hfill{\# The set that saves equivalent classes}
            \STATE $\tilde{S} \leftarrow S \backslash \mathrm{Neig}_G(Y)$.
            \FOR{$T$ in $\mathrm{Pow}(\mathrm{Neig}_G(Y))$}
                \STATE $\tilde{G} \leftarrow \text{Sub-graph}(G,T,\mathrm{Neig}_G(Y)\backslash T, \tilde{S})$.
                \STATE $P_{\tilde{G}} \leftarrow \text{Recover}(\tilde{G})$.
                % \FOR{$[\tilde{S}_i]$ in $P_{\tilde{G}}$}
                %     \FOR{$\tilde{S}_{i,j}$ in $[\tilde{S}_i]$}
                %         \STATE $\tilde{S}_{i,j} \leftarrow \tilde{S}_{i,j} \cup T$. \hfill{\# Add $T$ to each subset of every equivalent class in $P_{\tilde{G}}$}
                %     \ENDFOR
                % \ENDFOR 
                \STATE Append $T$ to members of every equivalent class in $P_{\tilde{G}}$
                \STATE $P_G \leftarrow P_G \cup P_{\tilde{G}}$.
            \ENDFOR
            \STATE \textbf{return} $P_G$.
        \ENDIF
    \ENDFUNCTION
    \vspace{+0.05cm}
    \FUNCTION{$\text{Sub-graph}(G,T,\mathrm{Neig}_G(Y)\backslash T, \tilde{S})$}
        \STATE \textbf{return} the MAG of $G$, with $T$ as the selection set, $\mathrm{Neig}_G(Y)\backslash T$ as the latent set, and  $\tilde{S}$ as the observation set.
    \ENDFUNCTION
\end{algorithmic}
\end{algorithm}

%\textcolor{red}{The PDAG, PAG problem.}



==> icml23_paras/old_method_mz/method_3.tex <==
\subsection{Complexity Analysis}
\label{sec.complex}

In this section, we discuss the time complexity of Alg.~\ref{alg:identify-f-star}, which is composed of two parts: \textbf{i)} the causal discovery; \textbf{ii)} the identification of the optimal subset.

Complexity of causal discovery algorithms such as the PC \cite{spirtes2000causation} and its extension \cite{huang2020causal} to heterogeneous data can be bounded by $O(d^\Delta)$, with $\Delta$ the maximal degree of $G$. Benefit from the graphical condition in Thm.~\ref{thm:graph degenerate}, our method can identify the optimal subset in constant time when $Y \not \to \mathbf{K}$. When $Y \to \mathbf{K}$, the complexity includes the recovery and search over \emph{g}-equivalent classes. Specifically, complexity of Alg.~\ref{alg: recover g-equivalence} is decided by the size of the recursion tree. Since each vertex in the recursion tree has at least two children, the size of the tree is at most twice the number of leaf vertices in the tree. The latter of which is exactly $N_G$, \emph{i.e.}, the number of \emph{g}-equivalent classes. So, the complexity of Alg.~\ref{alg: recover g-equivalence} is $O(N_G)$ and the overall cost of recovering and searching over \emph{g}-equivalent classes can be bounded by $O(N_G)$.

To illustrate the rank of $N_G$ relative to $d_S$, we first define the following structures. We omit the subscript $S$ and denote the stable graph as $G$ for brevity.

\begin{definition}
    In $G$, a \emph{branch} vertex is a vertex with at least three neighbors. A \emph{chain} is a path where every vertex on the path has at most two neighbors. The length of a chain is the number of vertices in it. A \emph{maximal chain} is a chain that can not be extended longer. A maximal chain $c$ is \emph{isolated} if there is no path through $c$ connects $Y$ and another maximal chain. Denote the set of isolated maximal chains as $\mathrm{Iso}_{G}$. In a maximal chain, call the vertices closet to $Y$ as the \emph{head} vertices. A maximal chain $c$ is the \emph{adjacent} of $Y$ if there is no other maximal chain in the shortest path between $Y$ and the heads of $c$. For a maximal chain $c$ that is adjacent to $Y$, define a set of operators $\mathrm{opt}_c$: if $c$ is isolated, $\mathrm{opt}_c(G):=\{\text{remove} \ c\}$; Otherwise, $\mathrm{opt}_c(G):=\{\text{remove} \ \mathbf{X}^{1:i}_c| i=1,2,...,\mathrm{len}(c)\} \cup \{\text{replace} \ c \ \text{with an edge}\}$, where $X^i_c$ is the $i$-th vertex (in the order of the distance to $Y$) in $c$. Define $\mathrm{cost}(c):=\mathrm{len}(c)+1$ if $c$ has one head, $\frac{\mathrm{len}(c)^2+\mathrm{len}(c)+2}{2}$ if $c$ has two heads. 
\end{definition}

%The rank of $N_G$ w.r.t. $d_S$ is decided by structure of the stable graph $G^s$. When $G^s$ is sparse, vertices close to $Y$ can block all the paths between $Y$ and vertices away from $Y$, making many subsets be equivalent and $N_G$ be small. Formally, define the following structures. 

Intuitively, $N_G$ is associated with the sparsity of $G$. When $G$ is sparse, vertices close to $Y$ can block the paths between $Y$ and the other vertices, which means many subsets are equivalent and $N_G$ is small. We find such a sparsity can be described by the density of branch vertices and maximal chains in $G$. Formally speaking,

\begin{proposition} 
    In $G$, denote $d_{\geq 3}$ as the number of branch vertices. Let $F_G$ be the product of summation of the costs of maximal chains:
    \begin{equation*}
        F_G:=\prod_{c\in \mathrm{Neig}_G(Y) \cap \mathrm{Iso_{G}}} \mathrm{cost}(c) \sum_{\mathrm{opt}\in \prod_{c\in \mathrm{Neig}_G(Y)}\mathrm{opt}_{c}} F_{\mathrm{opt}(G)}.
    \end{equation*}
    Then, $N_G=\mathrm{P}(d_S)$ iff $d_{\geq 3}=O(\mathrm{log}(d_S)), F_{G}=\mathrm{P}(d_S)$.
\end{proposition}


==> icml23_paras/old_method_mz/method_xw-1.tex <==
\section{Methodology}
\label{sec.methd}


\subsection{Minimax Analysis}
\label{sec.identify}


redraw figure 2


\textbf{Learning to attain the Worst-case Risk.}



In this section, we introduce our method to select the optimal subset. We firstly establish theoretical results regarding the minimax properties in Sec.~\ref{sec.identify}. Then, guided by the theoretical analysis, we in Sec.~\ref{sec.learn} provide an efficient algorithm for optimal subset selection. Finally, we discuss the complexity of the selection algorithm in Sec.~\ref{sec.complex}.



In this section, we establish theoretical results regarding the robustness aspect. Our results answer two key questions: \textbf{i)} In which kind of causal DAG does the whole stable set $S$ reach the minimax optimum? \textbf{ii)} When $S$ may not be optimal, how to \emph{consistently} measure the robustness of each subset on (infinitely many) deployment environments, using only data from a few training environments?

In the following, we first provide the answer to the first question. We find whether the interventional distribution can degenerate is decided by connections between $Y$ and a vertices set $\mathbf{K}$ in the causal DAG. If $Y$ does not point to any member of $\mathbf{K}$, the \emph{do} in $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can be removed and the minimax optimum is reached by the whole stable set $S$. 

\begin{theorem}[Graphical Condition for $S^*\!=\!S$]
\label{thm:graph degenerate}
Suppose Asm~\ref{eq:assum-dag},~\ref{eq:assum-markov-faithfulness} hold. Denote $\mathbf{X}_{M}^{0}\!:=\!\mathbf{X}_{M}\cap \mathrm{Ch}(Y)$ as mutable variables in $Y$'s children, and $\mathbf{K}:=\mathrm{De}(\mathbf{X}_{M}^{0}) \backslash \mathbf{X}_M^0$ as descendants of $\mathbf{X}_{M}^{0}$. Then, $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution if and only if $Y$ does not point to any member of $\mathbf{K}$. Further, under either of the two conditions, $S^*=S$.
\end{theorem}
\vspace{-0.1cm}
\begin{proofsketch}
    If $Y$ does not point to any member of $\mathbf{K}$, we can use the inference rules \cite{pearl2009causality} to remove the ``\emph{do}'' in $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ and degenerate it into $P(Y|\mathbf{X}\backslash (\mathbf{X}_M^0 \cup \mathrm{De}(\mathbf{X}_M^0)))$. For example, in Fig.~\ref{fig: example graphical condition} (a), we have $P(Y|X_1,X_2, do(\boldsymbol{X}_m))=P(Y|X_2, do(\boldsymbol{x}_m))=P(Y|X_2)$. Such a degeneration (to conditional distribution) permits us to construct a probability distribution in $\{P^e| e \in \mathcal{E}\}$ for any predictor $f$, where $f$ has a larger or equal worst-case risk than $f_S$, thus proving the optimality of $S$. On the contrary, when $Y$ points to a member of $\mathbf{K}$, there is a collider ($X_1$ in Fig.~\ref{fig: example graphical condition} (b)) in $\mathbf{X}\backslash \mathbf{X}_M^0$ in some paths between $Y$ and $\mathbf{X}_M^0$. Conditioning on the collider will open the indirect path between $Y$ and $\mathbf{X}_M^0$, making it incapable to remove the ``\emph{do}''.
\end{proofsketch} 
\vspace{-0.1cm}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\columnwidth]{icml23_figs/fig_examples_thm3.1.pdf}
    \caption{Illustration of the graphical condition in Thm.~\ref{thm:graph degenerate}, with $\mathbf{K}$ marked as blue.}
    \label{fig: example graphical condition}
\end{figure}

Thm.~\ref{thm:graph degenerate} for the first time connects a minimax property to a specific graphical structure. Such a connection provides an intuitive explanation for the robustness of the whole stable set. It also saves end-users from running the inference rules to check the degeneration condition and makes the result easily accessible from the causal DAG, as guaranteed by the following proposition.

\begin{proposition}
	\label{prop.thm3.2 justifiability}
	Under Asm.~\ref{eq:assum-dag},~\ref{eq:assum-markov-faithfulness}, the subset $\mathbf{K}$ and whether $Y \to \mathbf{K}$ is identifiable.
\end{proposition}

On the other hand, Thm.~\ref{thm:graph degenerate} reminds us the sufficient condition for $S^*\!=\!S$ may not always hold. When the condition fails, including more stable information may not be always beneficial. Indeed, we provide a counter-example in Fig.~\ref{fig: example graphical condition} (b) that, the whole stable set ${\{X_2\}}$ has a larger generalization error than the empty set ${\varnothing}$, under some conditions\footnote{For details of these conditions, please refer to Sec. in the appendix.}on $P(Y)$ and $P(X_1|Y)$.

To identify the $S^*$ when Thm.~\ref{thm:graph degenerate} fails, we attempt to measure the robustness of each subset $S_{-}$ with data from $\mathcal{E}_{tr}$. Indeed, there are infinitely many deployment environments, each having various behaviors in terms of the probability distribution. A few held-out validation environments from $\mathcal{E}_{tr}$ are hard, if not impossible, to reflect the behavior of the worst-case environment and measure the worst-case risk. 

Our key observation to solve this problem is that all environments in $\mathcal{E}$, no matter how various their behaviors are, are governed by the causal DAG $G$, where the only source of variation is the mutable causal mechanisms of $\mathbf{X}_M$. In this regard, we can parameterize these mutable mechanisms and let them vary arbitrarily, which provides a simulation of the worst-case environment. Each subset's generalization ability on this simulation environment can thus \emph{consistently} reflect its robustness on $\mathcal{E}$. 

What makes the parameterization plausible is that we find $\mathbf{X}_M$ is always a \emph{definite} function of $\mathrm{Pa}(\mathbf{X}_M)$ when the worst-case risk is attained. In this regard, we can parameterize $J\!:\!\mathrm{Pa}(\mathbf{X}_M)\!\to\!\mathbf{X}_M$ with a neural network $J_\theta$ and maximize over $\theta$ to estimate the worst-case risk, due to its ability to approximate any definite function \cite{hornik1989multilayer}. Formally, define an instrumental distribution family $\{P_J\}_{J}$, with $J$ a definite function from $\mathrm{Pa}(\mathbf{X}_M)$ to $\mathbf{X}_M$ and $P_J\! :=\! P(Y,\mathbf{X}_S| do(\mathbf{X}_M\!=\!J(\mathrm{Pa}(\mathbf{X}_M)))$, we have the following minimax property:

\begin{theorem}[Minimax Property]
\label{thm:min-max}
For a subset $S_{-}$, denote $\mathcal{R}(S_{-})\!:=\!\max_{e \in \mathcal{E}} \mathbb{E}_{P^e}[\left(Y \!-\! f_{S_{-}}(\boldsymbol{x})\right)^2]$ as the worst-case risk on $\mathcal{E}$. Denote $\mathcal{L}(S_{-}):=\max_{J}\mathbb{E}_{P_J}[(Y \!-\! f_{S_{-}}(\boldsymbol{x}))^2]$ as the maximal population loss over $P_J$. Then, we have $\mathcal{R}(S_{-})=\mathcal{L}(S_{-})$. Thus, the optimal subset can be obtained via $S^* := \mathop{\mathrm{argmin}}_{S_{-} \subseteq S} \mathcal{L}(S_{-})$.
\end{theorem}

\begin{proofsketch}
Firstly consider the case where $\mathbf{X}_M=\{X_m\}$. The $\mathcal{R}(S_{-})$ expands to:
\begin{equation}
    \mathcal{R}(S_{-}) = \max_{e \in \mathcal{E}} \int_{y,\boldsymbol{x}} [y-f_{S_{-}}(\boldsymbol{x})]^2 p^e(y,x_m,\boldsymbol{x}_{S_{-}}) dy d\boldsymbol{x}.
\label{eq: risk}
\end{equation}
Factorize $p^e(y,x_m,\boldsymbol{x}_S)$ into disentangled causal factors and denote $\tilde{\mathbf{X}}:=\mathbf{X}\backslash (\{X_m\}\cup \mathrm{Pa}(X_m))$, we can split the integral into three parts, respectively over $\mathrm{pa}(x_m)$, $x_m$, and $y, \tilde{\boldsymbol{x}}$. Denote the last one as $g(x_m,\mathrm{pa}(x_m)):=\int_{y, \tilde{\boldsymbol{x}}} [y-f_{S_{-}}(\boldsymbol{x})]^2 p(y|\mathrm{pa}(y)) p(\tilde{\boldsymbol{x}}| \mathrm{pa}(\tilde{\boldsymbol{x}})) dyd\tilde{\boldsymbol{x}}$, Eq.~\ref{eq: risk} becomes:
\begin{align}
    &\mathcal{R}(S_{-}) = \max_{e \in \mathcal{E}} \int_{\mathrm{pa}(x_m)} \prod_{X_i \in \mathrm{Pa}(X_m)} p(x_i|\mathrm{pa}(x_i)) \nonumber \\ 
    &\int_{x_m} g(x_m,\mathrm{pa}(x_m)) p^e(x_m|\mathrm{pa}(x_m)) dx_m d \mathrm{pa}(x_m).
\end{align}
Since $p^e((x_m|\mathrm{pa}(x_m)))$ is the only item varying with $e$, we can move the maximization to the inner integral and have:
\begin{align}
    \mathcal{R}(S_{-})=&\int_{\mathrm{pa}(x_m)} \prod_{X_i \in \mathrm{Pa}(X_m)} p(x_i|\mathrm{pa}(x_i)) \nonumber \\ 
    &g(J^*(\mathrm{pa}(x_m)),\mathrm{pa}(x_m)) d \mathrm{pa}(x_m),
\label{eq: definite function}
\end{align}
with $J^*(\mathrm{pa}(x_m))\!:=\!\arg\max_{x_m}g(x_m,\mathrm{pa}(x_m))$ is a definite function from $\mathrm{pa}(x_m)$ to $x_m$. Eq.~\ref{eq: definite function} indicates the worst-case risk is attained when $x_m$ is a definite function of $\mathrm{pa}(x_m)$ and thus shows $\mathcal{R}(S_{-})=\mathcal{L}(S_{-})$.

In cases where $\mathbf{X}_M$ contains multiple variables, we can consider the maximization sequentially according to the topology order in $\mathbf{X}_M$. For details of the proof, please refer to Sec. in the appendix.
\end{proofsketch}

The tractability of the optimization over $J_\theta$ is assured by the following proposition on structural identifiability.

\begin{proposition}
	\label{prop.thm3.3 justifiability}
	Under Asm.~\ref{eq:assum-dag},~\ref{eq:assum-markov-faithfulness}, the $\mathbf{X}_M, \mathrm{Pa}(\mathbf{X}_M),$ $\mathrm{De}(\mathbf{X}_M), P_J$, and $f_{S_{-}}$ are identifiable. 
\end{proposition}

==> icml23_paras/old_method_mz/method_xw-2.tex <==
\subsection{Searching the Optimal subset from $g$-Equivalence}

Mention algorithm 1: composed of two parts: Y \to K and Y \not\to K

for Y \to K, g-equivalence. 

simplify algorithm 2. 



==> icml23_paras/old_method_mz/method_xw-3.tex <==
\subsection{Complexity Analysis}

composed of two parts: 

g-equivalence: exponential with < log(n); polynomial with > log(n); NP or P with = log(n). 

Others are left to appendix (include the necessary and the sufficient condition)

==> icml23_paras/old_method_xw/background.tex <==
\section{Preliminaries and Background} 
\label{sec.background}

\textbf{Problem Setup \& Notations.} We consider the supervised regression scenario, where the system includes a target variable $Y\!\in\!\mathcal{Y}$, a multivariate predictive variable $\mathbf{X} := [X_1,...,X_d] \!\in\! \mathbb{R}^d$, and data collected from heterogeneous environments. In practice, different ``environments" can refer to different groups of subjects or different experimental settings. We denote the set of training environments as $\mathcal{E}_{tr}$, and the broader set of environments for deployment as $\mathcal{E}$. We use $\{D_{e}|e\in\mathcal{E}_{\text{tr}}\}$ to denote our training data, with ${D_{e}\!:=\!\{(\boldsymbol{x}_{k}^e, {y}_{k}^e)\}_{k=1}^{n_e} \sim_{i.i.d} P^e(\mathbf{X},Y)}$ being the data sampled from environment $e$. In a directed acyclic graph (DAG) $G$, denote the parents, children, neighbors, and descendants of the vertices set $\mathbf{V}$ as $\mathrm{Pa}({\mathbf{V}})$, $\mathrm{Ch}({\mathbf{V}})$, $\mathrm{Neig}(\mathbf{V})$ and $\mathrm{De}({\mathbf{V}})$, respectively. Define the degree of a vertex as the number of its neighbors and denote the maximum degree as $\Delta$. We use $\perp$ to denote conditional independence, and $(\perp)_G$ to denote \emph{d}-separation in $G$. We denote $G_{\overline{\mathbf{V}}}$ as the graph in removing arrows pointing into vertices in $\mathbf{V}$. 
%Denote the manipulated graph \cite{spirtes2000causation} obtained by removing all arrows pointing into vertices in $\mathbf{V}$ as $G_{\overline{\mathbf{V}}}$.

% Our goal is to find the most robust predictor $f^*$ in the stable predictor set $\mathcal{F}^s$ using data from $\mathcal{E}_{\mathrm{tr}}$. 

Our goal is to find the most robust predictor $f^*$ among stable predictors using data from $\mathcal{E}_{\mathrm{tr}}$. Here, we say a predictor $f: \mathbb{R}^d \to \mathcal{Y}$ is stable if it is independent of $E$. We denote the set of stable predictors as $\mathcal{F}^s$. For robustness, a commonly adopted measurement \cite{peters2016causal,ahuja2021invariance} for a predictor is to investigate its worst-case risk, which provides a safeguard for deployment in unseen environments. That is, we want $f^*$ to be min-max optimal among the set of stable predictors $\mathcal{F}^s$:
\begin{align}
    f^{*}(\boldsymbol{x})=\mathop{\mathrm{argmin}}\limits_{f \in \mathcal{F}^s}        \max_{e\in\mathcal{E}}
    \mathbb{E}_{P^e}[(Y-f(\boldsymbol{x}))^2].
\label{eq.robust}
\end{align}
In the following, we first introduce some basic assumptions that our methods are based on. These assumptions are commonly made in the literature of causal inference and learning \cite{pearl2009causality,spirtes2000causation,arjovsky2019invariant}.
\begin{assumption}[Structural Causal Model]
\label{eq:assum-dag}
We assume that $P^e(\mathbf{X},Y)$ is entailed by an \emph{unknown} DAG $G$ over $\mathbf{V}$ for all $e \in \mathcal{E}$, where $\mathbf{V}:= \mathbf{X} \cup Y$. Each variable $V_i \in \mathbf{V}$ is generated via a structural equation $V_i=g^e_{i}(\mathrm{Pa}({V_i}), U_i)$, where $U_i$ denotes a exogenous variable. We assume  
each $g^e_{i}$ is continuous and bounded. Each edge $V_i \to V_j$ in $G$ represents a direct causal relationship from $V_i$ to $V_j$. %\citep{pearl1995causal}. 
\end{assumption}
%The causal DAG model is commonly assumed in the literature of causal inference \citep{pearl2009causality, spirtes2000causation}. 
Equipped with the autonomous property of structural equations, we define the intervention $\text{do}(V_i\!=\!v_i)$ as lifting $V_i$ from its original generating mechanism $V_i\!=\!\!g_{i}(\mathrm{PA}({V_i}), U_i)$ and setting it to a constant value $v_i$ \citep{pearl2009causality}. Under the following Markovian assumption, the intervention distribution $p(\boldsymbol{v}| do(\boldsymbol{v}_i))\!:=\!p(\boldsymbol{v})/\prod_{\tilde{v} \in \boldsymbol{v}_i}p(\tilde{v}|pa({\tilde{v}}))$.

\begin{assumption}[Markovian and Faithfulness]
\label{eq:assum-markov-faithfulness}
The Markovian assumes $\{U_i\}$ are mutually independent. This means {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Rightarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}, $\forall$ disjoint sets {\small $\mathbf{V}_i, \mathbf{V}_j, \mathbf{V}_k$}. The faithfulness assumes {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Leftarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}. In combination, we assume {\small $\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k \Leftrightarrow (\mathbf{V}_i \!\perp\! \mathbf{V}_j | \mathbf{V}_k)_G$}.
\end{assumption}

According to the Causal Markov Condition \citep{pearl2009causality}, we have the causal factorization of the joint probability $p(v) = \prod_i p(v_i|pa(v_i)))$, where each term $p(v_i|pa(v_i))$ represents the generating of $V_i$ given its parents $\mathrm{PA}(V_i)$. 
%This factorization allows us to find the reason behind distributional shifts as the variation of some generating factors. According to the Causal Markov Condition theorem, the joint distribution over $\mathbf{V}$ has the following causal factorization: $P(\mathbf{V}) = \Pi_i P(V_i|\mathrm{Pa}(V_i))$. Based on this, the interventional distribution is defined as $P(\mathbf{V}|do(V_i=v_i))$ as $P(\mathbf{V}|do(V_i=v_i)) = \Pi_{j \neq i}P(V_j|\mathrm{Pa}(V_j))\mathbbm{1}(V_i = v_i)$. 
In our scenario, we have the following form of $P^e(\mathbf{X},Y)$:
\begin{align}
\label{eq: causal factorization}
    & P^e(\boldsymbol{X}, Y) = P(Y|\mathrm{Pa}(Y)) \prod_{i \in S} P\left(X_i|\mathrm{Pa}(X_i)\right) \nonumber \\
    & \prod_{i \in M} P^e(X_i|\mathrm{Pa}(X_i)), d_S:=|S|, d_M:=|M|,
\end{align}
%the joint distribution $P^e(\mathbf{X},Y)$ for each $e$ can factorize into disentangled causal factors \cite{scholkopf2021toward}:
%\begin{equation}
%    P^e(\mathbf{X},Y)=P^e(Y|\mathrm{Pa}(Y)) \prod_{i=1}^d P^e(X_i|\mathrm{Pa}(X_i)).
%\label{eq: causal factorization}
%\end{equation}
where $S, M$ respectively denote stable and mutable sets such that each $X_i \in \mathbf{X}_S$ has invariant conditional factor $P(X_i|\mathrm{Pa}(X_i))$; while the factor varies across $\mathcal{E}$ for each $X_i \in \mathbf{X}_M$. Correspondingly, we call $\mathbf{X}_S$ as stable variables and $\mathbf{X}_M$ as mutable variables. In addition to $\mathbf{X}_S$, we also assume the causal factor of $Y$ keeps invariant across $\mathcal{E}$, which has been widely adopted in the existing literature \cite{arjovsky2019invariant,sun2021recovering,mitrovic2021representation}. Besides, we assume that $\mathcal{E}_{tr}$ can consistently reflect the heterogeneity in $\mathcal{E}$, which is formally stated as follows: 
\begin{assumption}[Consistent Heterogeneity]
\label{assum:e-train}
For each $X_i \in \mathbf{X}_M$, we assume that there exists $e_1, e_2 \in \mathcal{E}_{tr}$ with $e_1 \neq e_2$ such that $P^{e_1}(X_i|\mathrm{Pa}(X_i)) \neq P^{e_1}(X_i|\mathrm{Pa}(X_i))$.
\end{assumption}

This assumption requires $\mathcal{E}_{tr}$ to be large and diverse enough to reflect the variation of $\mathbf{X}_M$ across $\mathcal{E}$, which is necessary to recover $\mathbf{X}_M$ from training data. 


% To detect the mutable sets from the training environments, we assume that $\mathcal{E}_{tr}$ can consistently reflect the heterogeneity in $\mathcal{E}$, \emph{i.e.}, any mutable variable in $\mathcal{E}$ is a mutable variable in $\mathcal{E}_{tr}$. 

\textbf{Surgery Estimator.} The surgery estimator \citep{subbaswamy2019preventing} proposed to remove the mutation in $P^e(\mathbf{X},Y)$ by intervening on $\mathbf{X}_M$ and obtained a set of stable predictors $\mathcal{F}^s:=\{f_{S_{-}}(\boldsymbol{x})\!:=\!\mathbb{E}[Y|\boldsymbol{x}_{S_{-}}, do(\boldsymbol{x}_M)]|{S_{-}} \!\subseteq \!{S}\}$ over the interventional distribution. In this regard, identifying the optimal min-max optimal predictor in Eq.~\ref{eq.robust} is equivalent to selecting the optimal subset $S^* \!\subseteq\! S$. 

For this purpose, the \cite{subbaswamy2019preventing} first proved that the whole stable set $S$ is optimal under \emph{degeneration condition}: the intervened distribution $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution, \emph{i.e.}, $P(Y|\mathbf{X}_{-})$ for some $\mathbf{X}_{-} \subseteq \mathbf{X}$. However, the authors did not provide an approach to \textbf{test this condition}, limiting the utility of the theory. In practice, they compared each subset $S_{-} \subseteq S$ and selected the optimal subset as the one with minimal loss on a held-out validation set. This method \textbf{lacks} a theoretical guarantee. Indeed, we observe from Fig. \ref{fig:adni-intro} that the selected subset is not optimal, because the validation loss does not necessarily reflect the worst-case risk among deployed environments. In the subsequent section, we propose to remedy the above problems of the graph surgery estimator, by considering the following questions: \textbf{i)} \emph{can we test the degeneration condition, or some of its equivalent conditions, in order to determine whether $S = S^*$?} \textbf{ii)} \emph{can we provide an approach to identify the optimal subset with theoretical guarantees under general scenarios?}

% This method does not theoretical guarantee for the selected subset to be optimal


% In more general cases when this condition does not hold, they compared each subset $S_{-} \subseteq S$ in terms of the loss on a held-out validation set in $\mathcal{E}_{tr}$ and selected the optimal subset as the one with minimal validation loss. Although their method tackles the stability issue well, their analysis of robustness suffers from the following problems: \textbf{i)} for the degeneration condition for $S^*=S$, they did not provide an approach to test the condition, violating this condition into practical use; \textbf{ii)} there is no theoretical guarantee for the optimality of the selected subset  because the validation loss may not reflect a subset's worst-case risk (as shown in Fig. \ref{fig:adni-intro}). 

% In the next section, we will provide a comprehensive minimax analysis to remedy these issues.

% selected the optimal subset as the one with minimal held-out validation loss.  for each subset $S_{-} \subseteq S$ and selected the optimal subset with minimal .

==> icml23_paras/old_method_xw/complexity.tex <==
\section{Complexity Analysis}
\label{sec.complex}

In this section, we discuss the time complexity of Alg.~\ref{alg:identify-f-star}, which is composed of two parts: \textbf{i)} the causal discovery; \textbf{ii)} the selection of optimal subset.

Complexity of constraint-based causal discovery algorithms such as the PC \cite{spirtes2000causation} and its extension to heterogeneous data \cite{huang2020causal} can be bounded by $O(d^\Delta)$. As for the cost of subset selection, when $Y \not \to \mathbf{W}$, Alg.~\ref{alg:identify-f-star} uses the graphical condition in Thm.~\ref{thm:graph degenerate} and has $S^*=S$ in constant time. When $Y \to \mathbf{W}$, the complexity consists of the recovery and search over \emph{g}-equivalent classes. Specifically, recovering \emph{g}-equivalent classes with  Alg.~\ref{alg: recover g-equivalence} involves a recursive construction of MAGs, the complexity of which is then decided by size of the recursion tree. Since each vertex in the recursion tree has at least two children, the size of the tree is at most twice the number of leaf vertices in the tree. The latter one is exactly $N_G$, \emph{i.e.}, the number of \emph{g}-equivalent classes. As a result, the complexity of \emph{g}-equivalence recovery is $O(N_G)$ and the overall cost of recovering and searching over \emph{g}-equivalent classes can also be bounded by $O(N_G)$.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{icml23_figs/simg3_ad_causal_graphs.pdf}
    \caption{(a) The causal graph for synthetic data generation. The dashed line $M_1 \to S_1$ does not exist (resp. exist) in setting-1 (resp. setting-2). (b) The learned causal graph on ADNI. $\leftrightarrow$ denotes undirected edges.}
    \label{fig:simg3_ad_causal_graphs}
\end{figure*}

To illustrate the relation between $N_G$ and the number of stable variables $d_S$, we first define the following structures. 

\begin{definition}
    A branch vertex is a vertex of degree at least three. A chain is a sequence of adjacent and distinct vertices where every vertex is non-branch vertex. A maximal chain is a chain that can not be extended longer. 
\end{definition}

\begin{claim}[\emph{g}-Equivalence in Chains]
    Suppose the skeleton of $G_S$ is a chain with $Y$ at the beginning side, \emph{i.e.}, $Y*-*X_1*-*...*-*X_{d_S}$. Then, we have $N_G = d_S+1$ is decided by the length of the chain.
\end{claim}

The rank of $N_G$ with respect to $d_S$ is decided by the stable graph's structural sparsity. Specifically, when $G_S$ is sparse and most vertices are non-branch vertices, the graph will be mostly composed of disjoint maximal chains. Since the number of \emph{g}-equivalent classes in a chain is decided by its length, $N_G$ will be decided by the product of maximal chains' lengths. In contrast, when $G_S$ is dense and most vertices are branch vertices, the maximum leaf spanning tree of $G_S$ will have many leaf vertices. Subsets consisting these leaf vertices are not equivalent, resulting the recovery and search of the $N_G$ equivalent classes $\mathrm{NP}$-hard. 



% We can write an informal version of iff condition, then explain it in details in the appendix
\begin{proposition}[Informal]
In $G_S$, let $d_{\geq 3}$ be the number of branch vertices, let $\pi$ be the product of maximal chains' lengths. Then, $N_G=\mathrm{P}(d_S)$ iff $d_{\geq 3}=O(\mathrm{log}(d_S))$ and $\pi=\mathrm{P}(d_S)$.
\label{prop: complexity}
\end{proposition}

\begin{remark}
    The formal definition of $\pi$, as well as the proof of Prop. \ref{prop: complexity} are available in Sect. in the appendix. 
\end{remark}



%To illustrate the rank of $N_G$ relative to $d_S$, we first define the following structures. We omit the subscript $S$ and denote the stable graph as $G$ for brevity.

%\begin{definition}
%     In $G$, a \emph{branch} vertex is a vertex with at least three neighbors. A \emph{chain} is a path where every vertex on the path has at most two neighbors. The length of a chain is the number of vertices in it. A \emph{maximal chain} is a chain that can not be extended longer. A maximal chain $c$ is \emph{isolated} if there is no path through $c$ connects $Y$ and another maximal chain. Denote the set of isolated maximal chains as $\mathrm{Iso}_{G}$. In a maximal chain, call the vertices closet to $Y$ as the \emph{head} vertices. A maximal chain $c$ is the \emph{adjacent} of $Y$ if there is no other maximal chain in the shortest path between $Y$ and the heads of $c$. For a maximal chain $c$ that is adjacent to $Y$, define a set of operators $\mathrm{opt}_c$: if $c$ is isolated, $\mathrm{opt}_c(G):=\{\text{remove} \ c\}$; Otherwise, $\mathrm{opt}_c(G):=\{\text{remove} \ \mathbf{X}^{1:i}_c| i=1,2,...,\mathrm{len}(c)\} \cup \{\text{replace} \ c \ \text{with an edge}\}$, where $X^i_c$ is the $i$-th vertex (in the order of the distance to $Y$) in $c$. Define $\mathrm{cost}(c):=\mathrm{len}(c)+1$ if $c$ has one head, $\frac{\mathrm{len}(c)^2+\mathrm{len}(c)+2}{2}$ if $c$ has two heads. 
% \end{definition}

%The rank of $N_G$ w.r.t. $d_S$ is decided by structure of the stable graph $G^s$. When $G^s$ is sparse, vertices close to $Y$ can block all the paths between $Y$ and vertices away from $Y$, making many subsets be equivalent and $N_G$ be small. Formally, define the following structures. 

% Intuitively, $N_G$ is associated with the sparsity of $G$. When $G$ is sparse, vertices close to $Y$ can block the paths between $Y$ and the other vertices, which means many subsets are equivalent and $N_G$ is small. We find such a sparsity can be described by the density of branch vertices and maximal chains in $G$. Formally speaking,

% \begin{proposition} 
%     In $G$, denote $d_{\geq 3}$ as the number of branch vertices. Let $F_G$ be the product of summation of the costs of maximal chains:
%     \begin{equation*}
%         F_G:=\prod_{c\in \mathrm{Neig}_G(Y) \cap \mathrm{Iso_{G}}} \mathrm{cost}(c) \sum_{\mathrm{opt}\in \prod_{c\in \mathrm{Neig}_G(Y)}\mathrm{opt}_{c}} F_{\mathrm{opt}(G)}.
%     \end{equation*}
%     Then, $N_G=\mathrm{P}(d_S)$ iff $d_{\geq 3}=O(\mathrm{log}(d_S)), F_{G}=\mathrm{P}(d_S)$.
% \label{prop: complexity}
% \end{proposition}

==> icml23_paras/old_method_xw/complexity_v2.tex <==
\section{Complexity Analysis}
\label{sec.complex}

In this section, we discuss the time complexity of Alg.~\ref{alg:identify-f-star}, which is composed of two parts: \textbf{i)} causal discovery; \textbf{ii)} identify $S^*$ when $Y \to \mathbf{W}$.

For causal discovery, the constraint-based algorithms such as PC algorithm \cite{spirtes2000causation} and its extension to heterogeneous data \cite{huang2020causal} have the complexity of $O(d^\Delta)$. For \textbf{ii)}, the complexity is accounted by recovery and search over \emph{g}-equivalent classes. Obviously, the complexity of searching is $\Theta(N_G)$ with $N_G := |\mathrm{Pow}(S)\backslash\!\sim_G\!|$. For recovery of $\mathrm{Pow}(S)\backslash \sim_G$, it involves a recursive construction of MAGs. By applying the recursion tree method, we can show that this complexity is also $\Theta(N_G)$. Therefore, the complexity of part \textbf{ii)} is $\Theta(N_G)$. Next, we will discuss the order of $N_G$. Particularly, we are interested to know: \emph{can the $g$-equivalence reduce the exponential cost in searching over all subsets, to the polynomial cost?}


Intuitively, $N_G$ is related to the sparsity of the graph $G_S$: the smaller of the sparsity level means more conditional independence, hence making it easier for subsets to be equivalent, according to the definition of $g$-equivalence. Formally speaking, we denote $d_{\geq 3}$ as the number of vertices (in $\mathbf{X}_S$) of degree at least three; and $\Delta_S$ as the maximum degree among $Y \cup \mathbf{X}_S$. We then have the following result: 

\begin{proposition}[Complexity]
\label{prop: complexity}
Denote $\mathrm{P}(\cdot)$ and $\mathrm{NP}(\cdot)$ as polynomial and non-polynomial time complexity. Then we have \textbf{i)} $N_G=\mathrm{P}(d_S)$ if $d_{\geq 3} = O(1)$ and $\Delta_{S} = O(1)$; \textbf{ii)} $N_G=\mathrm{NP}(d_S)$ if either $d_{\geq 3} > \Omega(\log(d_S))$ or $\Delta_{S} = \Omega(\log(d_S))$; \textbf{iii)} if both $d_{\geq 3}$ and $\Delta_S$ are $=O(\log(d))$ but $=\Omega(1)$, $N_G$ can be $\mathrm{P}(d_S)$ or $\mathrm{NP}(d_S)$. 
\end{proposition}
\begin{remark}
    In the case \textbf{iii)} when both $d_{\geq 3}$ and $\Delta_S$ are $=O(\log(d))$ but $=\Omega(1)$, we have a sufficient and necessary condition to determine $\mathrm{P}$ or $\mathrm{NP}$. Such a condition is related to the graph structure. Roughly speaking, it considers the product of the lengths of each maximal chain in the graph. Here, a chain is a sequence of adjacent and distinct vertices where every vertex is of degree at most two; and a maximal chain is a chain that can not be extended longer. To illustrate, we consider the $G_S$ with $Y$ connecting to $K$ disjoint chains $C_1,...,C_K$, then we have $N_G = \Pi_{k}^K (|C_K|+1)$. Due to space limits, we leave formal definitions, results, and detailed analysis in Sec. \textcolor{blue}{??} in the appendix. 
\end{remark}

This result means that if the graph is sufficiently sparse, \emph{i.e.}, most vertices are with degrees less than three as well as a constant level of maximal degree, we can reduce the complexity to the polynomial cost. However, the complexity is still $\mathrm{NP}$ if $G_S$ is dense. We will empirically show that the complexity can be reduced to a larger extent, if the graph gets more sparse. 
%let $d_{\geq 3}$ be the number of branch vertices, let $\pi$ be the product of maximal chains' lengths. for some $\alpha > 1$ iff $d_{\geq 3}=O(\mathrm{log}(d_S))$ and $\pi=\mathrm{P}(d_S)$.

%To illustrate the relation between $N_G$ and the number of stable variables $d_S$, we first define the following structures. 

%\begin{definition}
%    A branch vertex is a vertex of degree at least three. A chain is a sequence of adjacent and distinct vertices where every vertex is non-branch vertex. A maximal chain is a chain that can not be extended longer. 
%\end{definition}

%\begin{claim}[\emph{g}-Equivalence in Chains]
%    Suppose the skeleton of $G_S$ is a chain with $Y$ at the beginning side, \emph{i.e.}, $Y*-*X_1*-*...*-*X_{d_S}$. Then, we have $N_G = d_S+1$ is decided by the length of the chain.
%\end{claim}

%The rank of $N_G$ with respect to $d_S$ is decided by the stable graph's structural sparsity. Specifically, when $G_S$ is sparse and most vertices are non-branch vertices, the graph will be mostly composed of disjoint maximal chains. Since the number of \emph{g}-equivalent classes in a chain is decided by its length, $N_G$ will be decided by the product of maximal chains' lengths. In contrast, when $G_S$ is dense and most vertices are branch vertices, the maximum leaf spanning tree of $G_S$ will have many leaf vertices. Subsets consisting these leaf vertices are not equivalent, resulting the recovery and search of the $N_G$ equivalent classes $\mathrm{NP}$-hard. 



% We can write an informal version of iff condition, then explain it in details in the appendix


%\begin{remark}
%    The formal definition of $\pi$, as well as the proof of Prop. \ref{prop: complexity} are available in Sect. in the appendix. 
%\end{remark}



==> icml23_paras/old_method_xw/complexity_v3.tex <==
\section{Searching Complexity Analysis}
\label{sec.complex}

In this section, we discuss the searching complexity of Alg.~\ref{alg:identify-f-star}. We show that our proposed $\sim_G$-equivalence can reduce the exponential cost $O(2^{d_S})$ of exhaustive search to a polynomial one $\mathrm{P}(d_S)$.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\textwidth]{icml23_figs/simg3_ad_causal_graphs.pdf}
    \caption{(a) The causal graph for synthetic data generation. The dashed line $M_1 \to S_1$ does not exist (resp. exist) in setting-1 (resp. setting-2). (b) The learned causal graph on ADNI. $\leftrightarrow$ denotes undirected edges.}
    \label{fig:simg3_ad_causal_graphs}
\end{figure*}

To begin, we first look at a special graph structure: the chain (Fig.~\ref{fig:complexity_chain_tree} (a)), which is important in reducing the complexity. To see the reason, note that each vertex in the chain can $d$-separate the other far-ends vertices from $Y$, making each subset equivalent to ones that append other far-end nodes. For example, in Fig.~\ref{fig:complexity_chain_tree} (a), we have $S_i \sim_G S_i \cup S_{-}$ for each $S_- \subseteq \{S_i,...,S_6\}$ since $S_i$ d-separates $S_i,...,S_6$ from $Y$. As a result, we have $\mathrm{Pow}(S)\backslash \! \sim_G = \{[S_1],...,[S_6],\{\varnothing\}\}$. Formally, we have: 

\begin{claim}[Chain]
For a chain with $d_S$ vertices, there are $d_S+1$ equivalent classes.
\end{claim}

This means, in the chain structure, the $\sim_G$-equivalence can reduce the complexity from $2^{d_S}$ to $d_S+1$. Therefore, intuitively the overall searching cost will be reduced more significantly, if more vertices are distributed in chains. Formally, we split the node set of $\mathbf{X}_S$ into $\mathbf{V}_{\leq 2}:=\{V_i \in \mathbf{X}_S: \mathrm{degree}(V_i)\leq 2\}$ and $\mathbf{V}_{\geq 3}:=\{V_i \in \mathbf{X}_S: \mathrm{degree}(V_i)\geq 3\}$, where $\mathbf{V}_{\leq 2}$ contains nodes in some chain. We then use $d_{\leq 2}:=|\mathbf{V}_{\leq 2}|$ and $d_{\geq 3}:=|\mathbf{V}_{\geq 2}|$ to respectively denote the number of chain nodes and non-chain nodes. We show that when $d_{\geq 3} = O(\log{d_S})$ with $d_S:=|\mathbf{X}_S|$, which means the chain nodes take a major proportion, the $N_G$ can be reflected by $F_G$ that is roughly speaking, the products of chain's' lengths. 

To ease the understanding, we first define $F_G$ over the tree structure in Fig.~\ref{fig:complexity_chain_tree} (c), which does not have any cycles. Similar to $\mathrm{Neig}$ and $\mathrm{Ch}$ over nodes, we say a chain $\tilde{c} \in \mathrm{Ch}^{\circ}(c)$ (resp. $\mathrm{Neig}^{\circ}(c)$) if the start node of $\tilde{c}$ is the child of the end node of $c$ (resp. some end node of $\tilde{c}$ and $c$ are adjacent), in terms of the distance to $Y$. 
% To conclude, we find that the more vertices distributed in chains, and the more intensive the chains are, the smaller $N_G$ will be. Since vertices in chains have $\mathrm{deg} \leq 2$, we can use the $d_{\leq 2}:=\sum_i {1}(\mathrm{deg}(X_i) \leq 2)$ to measure their proportion. To measure the intensity of chains, we introduce a new metric $F_G$, which is an extension of the products of chains' lengths. We first illustrate $F_G$ in trees, as follows:

\begin{claim}[Tree]
For a $Y$-rooted tree, let
\begin{align*}
    F_G:=\prod_{c \in \mathrm{Ch}^{\circ}(Y)} f(c), \,\, f(c):=\mathrm{len}(c)+\prod_{\tilde{c} \in \mathrm{Ch}^{\circ}(c)} f(\tilde{c}),
\end{align*}
We have {\small $N_G=\mathrm{P}(d_S)$} iff {\small $d_{\geq 3}=O(\mathrm{log}(d_S))$ and $F_G=\mathrm{P}(d_S)$}. 
\end{claim}
\begin{remark}
In Fig.~\ref{fig:complexity_chain_tree} (c) where $c_3, c_4 \in \mathrm{Ch}^{\circ}(c_1)$ and $c_5, c_6 \in \mathrm{Ch}^{\circ}(c_2)$, we have $d_{\geq 3}=2$ and $F_G=(l_1+l_3 l_4)(l_2+l_5 l_6)$ with $l_i:=\mathrm{len}(c_i)$. 
\end{remark}
% In this regard, we can compare $F_G$ with $d_S$ to decide the complexity.

Now we consider general graphs that have cycle chains, \emph{e.g.}, $Y \leftrightarrow C_1 \leftrightarrow S_1 \leftrightarrow Y$ in Fig.~\ref{fig:complexity_chain_tree} (d). To extend $F_G$, we break each cycle via deleting edges at each node to convert it into a series of sub-trees, as shown in Fig.~\ref{fig:complexity_chain_tree} (d). Formally, for each chain $c$ that is adjacent to $Y$, we define a set of edge-deletion operators $\mathrm{opt}_c:=\{\text{delete each between adjacent nodes}\}$. Then we have the following $F_G$ and the conclusion in general cases: 

\begin{proposition}[Informal] For a graph $G_S$, let
\begin{align*}
    F_{G_S}:=\prod_{\substack{c\in \mathrm{Neig}^{\circ}(Y) \\ \mathrm{Neig}^{\circ}(c) = \varnothing}} \mathrm{len}(c) \sum_{\mathrm{opt}\in \prod_{c\in \mathrm{Neig}^{\circ}(Y)}\mathrm{opt}_{c}} F_{\mathrm{opt}(G_S)},
\end{align*}
We have {\small $N_G=\mathrm{P}(d_S)$} iff {\small $d_{\geq 3}=O(\mathrm{log}(d_S))$} and {\small $F_G=\mathrm{P}(d_S)$}. 
\end{proposition}

This result means as long as $d_{\geq 3}=O(\mathrm{log}(d_S))$, the $\sim_G$-equivalence can reduce the searching cost from exponential cost to a polynomial cost. 

==> icml23_paras/old_method_xw/complexity_xw_v2.tex <==
\section{Complexity Analysis}
\label{sec.complex}

In this section, we discuss the time complexity of Alg.~\ref{alg:identify-f-star}, which is composed of two parts: \textbf{i)} causal discovery; \textbf{ii)} identify $S^*$ when $Y \to \mathbf{W}$.

For causal discovery, the constraint-based algorithms such as PC algorithm \cite{spirtes2000causation} and its extension to heterogeneous data \cite{huang2020causal} have the complexity of $O(d^\Delta)$. For \textbf{ii)}, the complexity is accounted by recovery and search over \emph{g}-equivalent classes. Obviously, the complexity of searching is $\Theta(N_G)$ with $N_G := |\mathrm{Pow}(S)\backslash\!\sim_G\!|$. For recovery of $\mathrm{Pow}(S)\backslash \sim_G$, it involves a recursive construction of MAGs. By applying the recursion tree method, we can show that this complexity is also $\Theta(N_G)$. Therefore, the complexity of part \textbf{ii)} is $\Theta(N_G)$. Next, we will discuss the order of $N_G$. Particularly, we are interested to know: \emph{can the $g$-equivalence reduce the exponential cost in searching over all subsets, to the polynomial cost?}


Intuitively, $N_G$ is related to the sparsity of the graph $G_S$: the smaller of the sparsity level means more conditional independence, hence making it easier for subsets to be equivalent, according to the definition of $g$-equivalence. Formally speaking, we denote $d_{\geq 3}$ as the number of vertices (in $\mathbf{X}_S$) of degree at least three; and $\Delta_S$ as the maximum degree among $Y \cup \mathbf{X}_S$. We then have the following result: 

\begin{proposition}[Complexity]
\label{prop: complexity}
Denote $\mathrm{P}(\cdot)$ and $\mathrm{NP}(\cdot)$ as polynomial and non-polynomial time complexity. Then we have \textbf{i)} $N_G=\mathrm{P}(d_S)$ if $d_{\geq 3} = O(1)$ and $\Delta_{S} = O(1)$; \textbf{ii)} $N_G=\mathrm{NP}(d_S)$ if either $d_{\geq 3} > \Omega(\log(d_S))$ or $\Delta_{S} = \Omega(\log(d_S))$; \textbf{iii)} if both $d_{\geq 3}$ and $\Delta_S$ are $=O(\log(d))$ but $=\Omega(1)$, $N_G$ can be $\mathrm{P}(d_S)$ or $\mathrm{NP}(d_S)$. 
\end{proposition}
\begin{remark}
    In the case \textbf{iii)} when both $d_{\geq 3}$ and $\Delta_S$ are $=O(\log(d))$ but $=\Omega(1)$, we have a sufficient and necessary condition to determine $\mathrm{P}$ or $\mathrm{NP}$. Such a condition is related to the graph structure. Roughly speaking, it considers the product of the lengths of each maximal chain in the graph. Here, a chain is a sequence of adjacent and distinct vertices where every vertex is of degree at most two; and a maximal chain is a chain that can not be extended longer. To illustrate, we consider the $G_S$ with $Y$ connecting to $K$ disjoint chains $C_1,...,C_K$, then we have $N_G = \Pi_{k}^K (|C_K|+1)$. Due to space limits, we leave formal definitions, results, and detailed analysis in Sec. \textcolor{blue}{??} in the appendix. 
\end{remark}

This result means that if the graph is sufficiently sparse, \emph{i.e.}, most vertices are with degrees less than three as well as a constant level of maximal degree, we can reduce the complexity to the polynomial cost. However, the complexity is still $\mathrm{NP}$ if $G_S$ is dense. We will empirically show that the complexity can be reduced to a larger extent, if the graph gets more sparse. 
%let $d_{\geq 3}$ be the number of branch vertices, let $\pi$ be the product of maximal chains' lengths. for some $\alpha > 1$ iff $d_{\geq 3}=O(\mathrm{log}(d_S))$ and $\pi=\mathrm{P}(d_S)$.

%To illustrate the relation between $N_G$ and the number of stable variables $d_S$, we first define the following structures. 

%\begin{definition}
%    A branch vertex is a vertex of degree at least three. A chain is a sequence of adjacent and distinct vertices where every vertex is non-branch vertex. A maximal chain is a chain that can not be extended longer. 
%\end{definition}

%\begin{claim}[\emph{g}-Equivalence in Chains]
%    Suppose the skeleton of $G_S$ is a chain with $Y$ at the beginning side, \emph{i.e.}, $Y*-*X_1*-*...*-*X_{d_S}$. Then, we have $N_G = d_S+1$ is decided by the length of the chain.
%\end{claim}

%The rank of $N_G$ with respect to $d_S$ is decided by the stable graph's structural sparsity. Specifically, when $G_S$ is sparse and most vertices are non-branch vertices, the graph will be mostly composed of disjoint maximal chains. Since the number of \emph{g}-equivalent classes in a chain is decided by its length, $N_G$ will be decided by the product of maximal chains' lengths. In contrast, when $G_S$ is dense and most vertices are branch vertices, the maximum leaf spanning tree of $G_S$ will have many leaf vertices. Subsets consisting these leaf vertices are not equivalent, resulting the recovery and search of the $N_G$ equivalent classes $\mathrm{NP}$-hard. 



% We can write an informal version of iff condition, then explain it in details in the appendix


%\begin{remark}
%    The formal definition of $\pi$, as well as the proof of Prop. \ref{prop: complexity} are available in Sect. in the appendix. 
%\end{remark}



==> icml23_paras/old_method_xw/complexity_xw_v3.tex <==
\section{Searching Complexity Analysis}
\label{sec.complex}

In this section, we show that the equivalent relation can reduce the searching complexity of Alg.~\ref{alg:identify-f-star} from exponential $O(2^{d_S})$ to polynomial $\mathrm{P}(d_S)$.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\textwidth]{icml23_figs/simg3_ad_causal_graphs.pdf}
    \caption{(a) The causal graph for synthetic data generation. The dashed line $M_1 \to S_1$ does not exist (resp. exist) in setting-1 (resp. setting-2). (b) The learned causal graph on ADNI. $\leftrightarrow$ denotes undirected edges.}
    \label{fig:simg3_ad_causal_graphs}
\end{figure*}

To begin, we first look at a special graph structure called \emph{chain} as shown in Fig.~\ref{fig:complexity_chain_tree} (a), which is important in reducing the complexity. In a chain, each vertex can block the other far-ends vertices from $Y$, making each subset equivalent to ones that append any other far-end vertices. For example, in Fig.~\ref{fig:complexity_chain_tree} (a), we have $\{S_i\} \sim_G \{S_i\} \cup S^\prime$ for each $S^\prime \subseteq \{S_i,S_{i+1},...,S_6\}$ since $\{S_i\}$ blocks the far-ends vertices $\{S_i,S_{i+1},...,S_6\}$ from $Y$. As a result, we have $\mathrm{Pow}(S)/ \! \sim_G = \{[S_1],...,[S_6],\{\varnothing\}\}$. Formally, we have: 

\begin{claim}[Chain]
A chain with $d_S$ vertices has $d_S+1$ equivalent classes.
%For a chain with $d_S$ vertices, there are $d_S+1$ equivalent classes.
\end{claim}

This means the complexity is reduced from $O(2^{d_S})$ to $O(d_S)$ for each chain. Intuitively for the whole graph, more chain vertices will reduce more of the complexity. Formally, we split the vertices in $G_S$ into chain vertices and non-chain vertices, with chain vertices (resp. non-chain vertices) referring to those vertices with $\mathrm{deg} \leq 2$ (resp. $\mathrm{deg} > 2$). We use $d_{\leq 2}$ and $d_{>2}$ to respectively denote the number of chain vertices and non-chain vertices. We show that when $d_{>2} = O(\log({d_S}))$, which means the chain vertices take a major proportion in $G_S$, the complexity of $N_G$ is reflected by a graphical metric called $F_G$. 

Roughly speaking, $F_G$ measures the product of chains' lengths in the graph. To ease the understanding, we first introduce $F_G$ for the tree structure (Fig.~\ref{fig:complexity_chain_tree} (c)), which does not contain cycles. In a $Y$-rooted tree and a chain $c$ in the tree, we denote $V^{\mathrm{end}}_c$ (resp. $V^{\mathrm{sta}}_c$) as the node of $c$ that has the largest (resp. smallest) distance to $Y$. We say $c' \in \mathrm{Ch}^\prime(c)$ for two chains $c$ and $c'$, if $V^{\mathrm{sta}}_{c'} \in \mathrm{Ch}(V^{\mathrm{end}}_c)$. We introduce $F_G$ and its relation to the complexity as follows: 
%define the parent of a chain $c$ as the chain adjacent to $c$ on the path to the root $Y$. Denote $\mathrm{Pa}^\prime(c), \mathrm{Ch}^\prime(c)$ as the set of $c$'s parent and children, respectively. Then, we have:
\begin{claim}[Tree]
\label{prop:tree-complexity}
For a $Y$-rooted tree, let
\begin{align*}
    F_G:=\prod_{c \in \mathrm{Ch}^{\prime}(Y)} f(c), \,\, f(c):=\mathrm{len}(c)+\prod_{\tilde{c} \in \mathrm{Ch}^{\prime}(c)} f(\tilde{c}).
\end{align*}
Then, {\small $N_G=\mathrm{P}(d_S)$} iff {\small $d_{>2}=O(\mathrm{log}(d_S))$} and {\small $F_G=\mathrm{P}(d_S)$}. 
\end{claim}

For example, in Fig.~\ref{fig:complexity_chain_tree} (c), we have 
$d_{>2}=2$, $\mathrm{Ch}^\prime(Y):=\{c_1, c_2\}$, $\mathrm{Ch}^{\prime}(c_1):=\{c_3, c_4\}$, $\mathrm{Ch}^{\prime}(c_2):=\{c_5, c_6\}$, and the $F_G:=(l_1+l_3 l_4)(l_2+l_5 l_6)$ with $l_i:=\mathrm{len}(c_i)$.


Now, we consider the general cases where $G_S$ has cycles (Fig.~\ref{fig:complexity_chain_tree} (d)). To extend the $F_G$, we can break the cycles via deleting edges and convert $G_S$ into a series of subtrees. Formally, we say $c\in \mathrm{Neig}^\prime(Y)$ for a chain $c$, if there is no other chain node that does not belong to $c$ such that it has a smaller distance than $V^{\mathrm{sta}}_c$ from $Y$. Let $\mathrm{Neig}^\prime(c)=\varnothing$ if $c$ is disjoint with the other chains. For each $k$-length chain $\{c(1),...,c(k)\}:=c\in \mathrm{Neig}^\prime(Y)$, define a set of edge-deletion operators $\mathrm{opt}_c:=\{\text{delete } e_c(1) \text{ to } e_c(i)| i=1,...,\mathrm{len}(c)\}$, where $e_c(i)$ denotes the edge between $c(i-1)$ to $c(i)$ for $i > 1$ or the edge between $Y$ and $c(1)$ for $i=1$. 

\begin{proposition}[Informal] For a stable graph, let
\label{prop:general-complexity}
\begin{align*}
    F_{G}:=\prod_{\substack{c\in \mathrm{Neig}^{\prime}(Y) \\ \mathrm{Neig}^{\prime}(c) = \varnothing}} \mathrm{len}(c) \sum_{\mathrm{opt}\in \prod_{c\in \mathrm{Neig}^{\prime}(Y)}\mathrm{opt}_{c}} F_{\mathrm{opt}(G)},
\end{align*}
Then, {\small $N_G=\mathrm{P}(d_S)$} iff {\small $d_{>2}=O(\mathrm{log}(d_S))$} and {\small $F_G=\mathrm{P}(d_S)$}. 
\end{proposition}

\begin{remark}
    When the general graph degenerates to the tree, the $F_G$ defined in Prop.~\ref{prop:general-complexity} is the same as the one defined in Prop.~\ref{prop:tree-complexity}.
\end{remark}

==> icml23_paras/old_method_xw/complexity_xw_v5.tex <==


\textbf{Searching complexity.} We show that compared to the exponential cost $O(2^{d_S})$ of exhaustive search, our search strategy enjoys a polynomial cost $\mathrm{P}(d_S)$ when $G_S$ mainly consists of chains. To be specific, denote chain vertices as those of degree $\leq 2$, and a chain as a sequence of adjacent chain vertices. We have the following result: 
\begin{proposition}[Complexity (informal)]
    \label{prop:complexity(informal)}
    Let $d_{\leq 2}$ and $d_{>2}\!:=\!d_S\!-\!d_{\leq 2}$ respectively denote the number of chain vertices and non-chain vertices. When the chain vertices are ``distributed intensively", $N_G=\mathrm{P}(d_S)$ if and only if $d_{>2}=O(\log(d_S))$.
\end{proposition}

Here, ``distributed intensively" means the chains in the graph have very different lengths. Roughly speaking, this is because when the graph is composed of multiple chains that do not intersect each other, $N_G$ can be determined by the product of multiple chains' lengths. As a result, the $N_G$ tends to be smaller when these lengths are very different. More formal and general results are left to Appx.~\ref{sec: appendix complexity}. 



==> icml23_paras/old_method_xw/equivalence.tex <==
\section{Searching $S^*$ among $g$-Equivalence}
\label{sec.learn}

\begin{algorithm}[tb]
   \caption{Optimal Subset Selection.}
\label{alg:identify-f-star}
\begin{flushleft}
    \textbf{Input:} The training data $\{D_{e}|e\in\mathcal{E}_{\text{Tr}}\}$. \\
    \textbf{Output:} The optimal subset $S^*$ and predictor $f^*$.
\end{flushleft}
\begin{algorithmic}[1]
   \STATE Causal discovery of $G, \mathbf{W}$ and whether $Y \to \mathbf{W}$.
   \IF{$Y \not \to \mathbf{W}$}
        \STATE $S^* \leftarrow S, f^* \leftarrow f_S$. \hfill{\# Thm.~\ref{thm:graph degenerate}} 
   \ELSE
        \STATE $\mathcal{L}_{\min}\leftarrow \infty$.
    \STATE Recover $\mathrm{Pow}(S)\backslash \sim_G$. \hfill{\# Alg.~\ref{alg: recover g-equivalence}}
        \FOR{$[S_{-}]$ in $\mathrm{Pow}(S)\backslash \sim_G$}  
        \IF{$\mathcal{L}(S_{-})<\mathcal{L}_{\min}$}
            \STATE $\mathcal{L}_{\min} \leftarrow \mathcal{L}(S_{-})$.
            \STATE $S^* \leftarrow S_{-}, f^* \leftarrow f_{S_{-}}$. \hfill{\# Thm.~\ref{thm:min-max}} 
            \ENDIF
        \ENDFOR
    \ENDIF
    \STATE \textbf{return} $S^*, f^*$.
\end{algorithmic}
\end{algorithm}
\vspace{-0.2cm}

In this section, we provide an optimal subset selection algorithm from data in $\mathcal{E}_{tr}$, which combines the results in Thm.~\ref{thm:graph degenerate} and Thm.~\ref{thm:min-max}, as summarized in Alg.~\ref{alg:identify-f-star}. As claimed in line 3, the algorithm returns the whole stable set $S^*=S$, if the graphical criterion $Y \not\to K$ holds. If this condition fails, a natural strategy is searching over all subsets of $S$, to find the one with minimal worst-case risk, \emph{i.e.}, $\mathcal{R}(S_{-})$, which is commonly adopted in the literature \cite{rojas2018invariant,magliacane2018domain,subbaswamy2019preventing,subbaswamy2020spec}. 

However, this search strategy can be redundant for subsets that are equivalent in terms of the worst-case risk. As this risk is determined by $P(Y,\mathbf{X}_S|do(\mathbf{X}_M))$, two subsets $\hat{S}$ and $\tilde{S}$ are equivalent if $P(Y,\mathbf{X}_{\hat{S}}|do(\mathbf{X}_M)) = P(Y,\mathbf{X}_{\tilde{S}}|do(\mathbf{X}_M))$. Once the equivalent class is identified, we only need to randomly pick up one subset for estimation. For this consideration, we define the $g$-equivalence via $d$-separation in the following: 

\begin{definition}[\emph{g}-Equivalence]
\label{def:g-equi}
    Denote $G_{S}:=G_{\mathbf{V}=\mathbf{X}_S \cup Y}$ as the sub-graph restricted on $\mathbf{X}_S \cup Y$. We say two subsets $\hat{S}, \tilde{S}$ are \emph{g}-equivalent, if $\exists S_{\cap} \subseteq \hat{S} \cap \tilde{S}$ s.t. $(Y \!\perp\! (\mathbf{X}_{\hat{S}} \cup \mathbf{X}_{\tilde{S}}) \backslash \mathbf{X}_{S_{\cap}} | \mathbf{X}_{S_{\cap}})_{G_S}$. Denote the \emph{g}-equivalence as $\sim_G$. Then, we call the elements of the quotient space $\mathrm{Pow}(S)\backslash\!\sim_G$ as the set of \emph{g}-equivalent classes. We denote the \emph{g}-equivalent class of $S_{-}$ as $[S_{-}]$.
\end{definition}

\begin{remark}
    \label{remark: gequivalence indicates}
     To see the $g$-equivalent subsets have the same worst-case risk, note that for each $\hat{S} \sim_G \tilde{S}$, since $(Y \!\perp\! \mathbf{X}_{\hat{S}} \backslash \mathbf{X}_{S_{\cap}} | \mathbf{X}_{S_{\cap}})_{G_S}$ and $(Y \!\perp\!  \mathbf{X}_{\tilde{S}} \backslash \mathbf{X}_{S_{\cap}} | \mathbf{X}_{S_{\cap}})_{G_S}$, we have 
     \begin{align*}
         P(Y|\mathbf{X}_{\hat{S}}, do(\boldsymbol{x}_M)) 
         %& = 
         %P(Y|\mathbf{X}_{\hat{S}} \backslash \mathbf{X}_{S_{\cap}}, \mathbf{X}_{S_{\cap}}, do(\boldsymbol{x}_M)) \nonumber \\
         & = P(Y| \mathbf{X}_{S_{\cap}}, do(\boldsymbol{x}_M)) \nonumber \\
         %& = P(Y|\mathbf{X}_{\tilde{S}} \backslash \mathbf{X}_{S_{\cap}}, % \mathbf{X}_{S_{\cap}}, do(\boldsymbol{x}_M)) \nonumber \\
         & = P(Y|\mathbf{X}_{\tilde{S}}, do(\boldsymbol{x}_M))，
     \end{align*}
     %{\small $P(Y|\mathbf{X}_{\hat{S}}, do(\boldsymbol{x}_M)) = P(Y|\mathbf{X}_{S_{\cap}}, do(\boldsymbol{x}_M))$} and {\small $P(Y|\mathbf{X}_{\tilde{S}}, do(\boldsymbol{x}_M)) = P(Y|\mathbf{X}_{S_{\cap}}, do(\boldsymbol{x}_M))$}, 
     according to the Markovian assumption~\ref{eq:assum-markov-faithfulness}. We thus have {\small $\mathcal{R}_{\hat{S}} = \mathcal{R}_{\tilde{S}}$}. To illustrate, in Fig.~\ref{fig: example graphical condition} (a) we have {\small $\{X_{S_2}\} \sim_G \{X_{S_1},X_{S_2}\}$} because {\small $(Y \!\perp\! X_{S_1} |X_{S_2})_{G_S}$}. Correspondingly, we have {\small $P(Y|X_{S_1},X_{S_2},do(X_M))$ $=P(Y|X_{S_2},do(X_M))$}.
     %t is sufficient to search over $\mathrm{Pow}(S) \backslash \!\sim_G:=\{\{X_2\},\{\{X_1\},\{X_1,X_2\}\}$. 
\end{remark}
%Generally speaking, we go over only equivalent classes $\mathrm{Pow}(S) \backslash \!\sim_G$ and randomly pick up an element in each class to estimate the worst-case risk, as summarized in lines 7-9 in Alg.~\ref{alg:identify-f-star}. 

\begin{algorithm}[!h]
   \caption{[Informal] $\mathrm{Pow}(S) \backslash \!\sim_G:=\text{Recover}(G)$\protect\footnote{We only need the input graph to be Markov equivalent to $G$.}}
   \label{alg: recover g-equivalence}
\begin{algorithmic}[1]
       \STATE \textbf{Return} $\{\mathrm{Pow}(S)\}$ if $\mathrm{Neig}_G(Y)=\varnothing$.
       \STATE \textbf{Else}, set $P_G \leftarrow \emptyset$, $\tilde{S} \leftarrow S \backslash \mathrm{Neig}_G(Y)$.
       \STATE \quad \textbf{for} $T$ in $\mathrm{Pow}(\mathrm{Neig}_G(Y))$
       \STATE \quad \quad $\tilde{G} \leftarrow \text{MAG}(G,T,\mathrm{Neig}_G(Y)\backslash T, \tilde{S})$.
       \STATE \quad \quad $P_{\tilde{G}} \leftarrow \text{Recover}(\tilde{G})$.
       \STATE \quad \quad Append $T$ to members of every class in $P_{\tilde{G}}$. 
       \STATE \quad \quad $P_G \leftarrow P_G \cup P_{\tilde{G}}$.
       \STATE \quad \textbf{return} $P_G$.
\end{algorithmic}
%.}
\end{algorithm}

Finally, we introduce Alg.~\ref{alg: recover g-equivalence} to recover $\mathrm{Pow}(S) \backslash \!\sim_G$. Given any graph (which can be obtained by the causal discovery in line 1 of Alg.~\ref{alg:identify-f-star}) that is Markov equivalent to the ground-truth graph $G$, the Alg.~\ref{alg: recover g-equivalence} first goes over each subset of $Y$'s neighborhood set $\mathrm{Neig}_G(Y)$, since any two subsets are not equivalent. If $\mathrm{Neig}_G(Y) = \emptyset$, $\mathrm{Pow}(S) \backslash \!\sim_G$ only has one element: $\{\mathrm{POW}(S)\}$, since all subsets are equivalent according to Def.~\ref{def:g-equi}. Otherwise, for each subset $T \in \mathrm{Pow}(\mathrm{Neig}_G(Y))$, we take $T$ as selection variables and $\mathrm{Neig}_G(Y)\backslash T$ as latent variables to obtain the \emph{Maximal Ancestral Graph} (MAG) over other variables $S \backslash \mathrm{Neig}_G(Y)$, via $\text{MAG}(G,\mathbf{V}_{S},\mathbf{V}_L,\tilde{\mathbf{V}})$ \cite{zhang2008completeness} that obtains the MAG over $\tilde{\mathbf{V}}$ from $G$ over $\mathbf{V}:=\mathbf{V}_{S} \cup \mathbf{V}_L \cup \tilde{\mathbf{V}}$ (here $\mathbf{V}_{S}$ denotes the selection variable set, and $\mathbf{V}_L$ denotes the latent variable set). We then apply Alg.~\ref{alg: recover g-equivalence} on the MAG and repeat this procedure until the neighborhood set of $Y$ is empty. The following result shows that our algorithm can correctly recover $\mathrm{Pow}(S) \backslash \!\sim_G$. 


\begin{proposition}
\label{prop:recover}
    Under Asm~\ref{eq:assum-dag},~\ref{eq: causal factorization} and for each input graph that is Markov equivalent to the ground-truth graph $G$, Alg.~\ref{alg: recover g-equivalence} can correctly recover $\mathrm{Pow}(S) \backslash \!\sim_G$.
\end{proposition}

%\begin{remark}
%    We leave the formal version of Alg.~\ref{alg: recover g-equivalence} and the proof of Prop.~\ref{prop:recover}. Note that Alg.~\ref{alg: recover g-equivalence} almost does not bring about additional computational costs to the searching procedure in Alg.~\ref{alg:identify-f-star}. Specifically, denote $N_G:=|\mathrm{POW}(S)\backslash \sim_G|$, we show in the appendix that the complexity of Alg.2 is $O(N_G \times |\mathbf{V}|^2)$ because the operator $\text{MAG}(\cdot,\cdot,\cdot,\cdot)$ is $O(|\mathbf{V}|^2)$ \cite{zhang2008completeness}. In contrast, the complexity of the searching procedure in Alg.1 is $\mathcal{O}(N_G \times n|\mathbf{V}||\theta_f||\theta_J|k_fk_{\mathcal{L}})$, where $\theta_f$, $\theta_J$ respectively denote the parameter in the predictor $f_{S_{-}}$ and the function $J$; the $k_f, k_{\mathcal{L}}$ respectively denotes the number of iteration in learning $f_{S_{-}}$ and optimizing $\mathcal{L}_{S_{-}}(J)$; $n$ denotes the number of samples. When $n > |\mathbf{V}|$, the 
%\end{remark}





% the guidance of Thm.~\ref{thm:graph degenerate} and Thm.~\ref{thm:min-max}. Given data from $\mathcal{E}_{tr}$, this algorithm firstly recovers the causal structures, including the causal graph, the components $\mathbf{X}_M, \mathbf{W}, \mathrm{Pa}(\mathbf{X}_M)$ and $\mathrm{De}(\mathbf{X}_M)$. It then checks whether $Y \to \mathbf{W}$. If $Y$ does not point to any member of $\mathbf{W}$, the algorithm sets $S$ as the optimal subset according to Thm.~\ref{thm:graph degenerate}; Otherwise, it searches over subsets to find the one with minimal $\mathcal{L}(S_{-})$ as the optimal subset, according to Thm.~\ref{thm:min-max}. 

%In previous methods \cite{rojas2018invariant,magliacane2018domain,subbaswamy2019preventing,subbaswamy2020spec}, such a search went through the power set of $S$ and was inevitably $\mathrm{NP}$-$\mathrm{hard}$. However, we find searching exhaustively is redundant and the cost can be reduced to $\mathrm{P}$ in some cases. Specifically, there are subsets with the same prediction power and can be grouped together to reduce the cost. For example, in Fig.~\ref{fig: example graphical condition} (a), the subsets $\{X_2\}$ and $\{X_1,X_2\}$ are equivalent, because $X_2$ and $do(x_m)$ block all the paths between $Y$ and $X_1$, and thus $P(Y|X_2,do(x_m))=P(Y|X_1,X_2,do(x_m))$ under Asm.~\ref{eq:assum-markov-faithfulness}. Formally speaking, denote $G^s$ as the stable graph after removing $\mathbf{X}_M$ from $G$, we define the \emph{g}-equivalent relation between subsets as follows.

% In this regard, it suffices to search over $\mathrm{Pow}(S)\backslash\!\sim_G$ to find the optimal subset and the cost can be reduced from $O(2^{d_S})$ to $O(N_G)$, with $d_S:=|S|$ and $N_G:=|\mathrm{Pow}(S)\backslash\!\sim_G|$. To enable the search, we need to recover the quotient space $\mathrm{Pow}(S)\backslash\!\sim_G$. This can be done via checking the conditional independence (CI) in $G$, as shown in Alg.~\ref{alg: recover g-equivalence}. Specifically, the algorithm recursively adds stable variables into the prediction set in the order of their distance to $Y$. During each recursion level, it creates sub-graphs to represent the CI after including/excluding some variables to/from the prediction set. These sub-graphs are constructed as the maximal ancestral graph (MAG) \cite{spirtes2000causation}, due to its ability to preserve the CI when included (\emph{i.e.}, selected) or excluded (\emph{i.e.}, latent) variables exist.

%\begin{algorithm}[!h]
%   \caption{Quotient Space Recovery.}
%   \label{alg: recover g-equivalence}
%\begin{flushleft}
%    \textbf{Input:} The causal graph $G$.\\
%    \textbf{Output:} The quotient space $\mathrm{Pow}(S)\backslash\!\sim_G$.
%\end{flushleft}
%\begin{algorithmic}[1]
%    \STATE Let $G^s$ the stable graph after removing $\mathbf{X}_M$ in $G$.
%    \STATE \textbf{return} $\mathrm{Recover}(G^s)$.
%    \vspace{+0.05cm}
%    \FUNCTION{$\text{Recover}(G)$}
%        \STATE Let $S$ the stable set of $G$.
%        \IF{$\mathrm{Neig}_G(Y)=\varnothing$}
%            \STATE \textbf{return} $\{\mathrm{Pow}(S)\}$. \hfill{\# All subsets are equivalent}
%        \ELSE
%            \STATE $P_G \leftarrow \varnothing$. \hfill{\# The set that saves equivalent classes}
%            \STATE $\tilde{S} \leftarrow S \backslash \mathrm{Neig}_G(Y)$.
%            \FOR{$T$ in $\mathrm{Pow}(\mathrm{Neig}_G(Y))$}
%                \STATE $\tilde{G} \leftarrow \text{Sub-graph}(G,T,\mathrm{Neig}_G(Y)\backslash T, \tilde{S})$.
 %               \STATE $P_{\tilde{G}} \leftarrow \text{Recover}(\tilde{G})$.
                % \FOR{$[\tilde{S}_i]$ in $P_{\tilde{G}}$}
                %     \FOR{$\tilde{S}_{i,j}$ in $[\tilde{S}_i]$}
                %         \STATE $\tilde{S}_{i,j} \leftarrow \tilde{S}_{i,j} \cup T$. \hfill{\# Add $T$ to each subset of every equivalent class in $P_{\tilde{G}}$}
                %     \ENDFOR
                % \ENDFOR 
 %               \STATE Append $T$ to members of every equivalent class in $P_{\tilde{G}}$
 %               \STATE $P_G \leftarrow P_G \cup P_{\tilde{G}}$.
 %           \ENDFOR
 %           \STATE \textbf{return} $P_G$.
 %       \ENDIF
 %   \ENDFUNCTION
 %   \vspace{+0.05cm}
 %   \FUNCTION{$\text{Sub-graph}(G,T,\mathrm{Neig}_G(Y)\backslash T, \tilde{S})$}
 %       \STATE \textbf{return} the MAG of $G$, with $T$ as the selection set, $\mathrm{Neig}_G(Y)\backslash T$ as the latent set, and  $\tilde{S}$ as the observation set.
 %   \ENDFUNCTION
%\end{algorithmic}
%\end{algorithm}

==> icml23_paras/old_method_xw/equivalence_v2.tex <==
\section{Searching $S^*$ among equivalence Classes}
\label{sec.learn}


In this section, we provide an optimal subset selection algorithm in Alg.~\ref{alg:identify-f-star} that combines Thm.~\ref{thm:graph degenerate} and Thm.~\ref{thm:min-max}. Specifically, Alg.~\ref{alg:identify-f-star} (line 3) selects the whole stable set as $S^*$, if the graphical condition $Y \not\to \mathbf{W}$ is tested true. If this condition fails, a simple strategy is to \emph{exhaustively} compare the worst-case risk of all subsets, which is commonly adopted in the literature \cite{rojas2018invariant,magliacane2018domain,subbaswamy2019preventing,subbaswamy2020spec}. 


In the following, we provide a new search strategy with better efficiency, by noticing that the exhaustive search can be redundant for subsets that have the same worst-case risk. Formally, we consider stable graph $G_S$ as the sub-graph of $G$ over $\mathbf{X}_S \cup Y$ as $G_S$, and introduce the following equivalence relation: 

\begin{definition}[Equivalence Relation]
\label{def:equi}
    Let $\sim_G$ be an equivalence relation on all subsets of $S$. Two subsets $S^{\prime}, S^{\prime \prime}$ are equivalent if $\exists \, S_{\cap} \subseteq S^\prime \cap S^{\prime \prime}$ s.t.
    \begin{align*}
    (Y \perp \mathbf{X}_{S_\cap^c} | \mathbf{X}_{S_\cap})_{G_S},
    \end{align*}
    with $S_\cap^c:=(S^\prime\cup S^{\prime \prime}) \backslash S_\cap$ the complementary set of $S_\cap$. We call elements of the quotient space $\mathrm{Pow}(S)/\!\sim_G$ as equivalence classes. We denote $[S^\prime] :=\{S^{\prime \prime}|S^{\prime \prime} \sim_G S^\prime\}$ as the equivalence class of $S^\prime$ and $N_G:=|\mathrm{Pow}(S)/\!\sim_G\!|$ as the number of equivalence classes. 
\end{definition}

\begin{algorithm}[tb]
   \caption{Optimal Subset Selection.}
\label{alg:identify-f-star}
\vspace{-0.1cm}
\begin{flushleft}
    \textbf{Input:} The training data $\{D_{e}|e\in\mathcal{E}_{\text{tr}}\}$. \\
    \textbf{Output:} The optimal subset $S^*$.
\end{flushleft}
\vspace{-0.2cm}
\begin{algorithmic}[1]
   \STATE Causal discovery of $G, \mathbf{W}$, and whether $Y \to \mathbf{W}$.
   \STATE \textbf{if} {$Y \not \to \mathbf{W}$} \textbf{then}
        \STATE \quad $S^* \leftarrow S$. \hfill{\# Thm.~\ref{thm:graph degenerate}} 
   \STATE \textbf{else}
    \STATE \quad  Recover $\mathrm{Pow}(S)/\!\sim_G$ via Alg.~\ref{alg: recover g-equivalence}.
    \STATE \quad  $\mathcal{L}_{\min}\leftarrow \infty$.
        \STATE \quad \textbf{for} {$[S^\prime]$ \textbf{in} $\mathrm{Pow}(S)/ \!\sim_G$} \textbf{do}
        \STATE \quad \quad \textbf{if} {$\mathcal{L}_{S^\prime} <\mathcal{L}_{\min}$} \textbf{then}
            \STATE \quad \quad \quad $\mathcal{L}_{\min} \leftarrow \mathcal{L}_{S^\prime}$, $S^* \leftarrow S^\prime$. \hfill{\# Thm.~\ref{thm:min-max}} 
            \STATE \quad \quad \textbf{end if}
        \STATE \quad \textbf{end for}
    \STATE \textbf{end if} 
    \STATE \textbf{return} $S^*$.
\end{algorithmic}
\end{algorithm} 

Intuitively, $S^\prime$ and $S^{\prime \prime}$ are equivalent if they share an intersection set $S_\cap$ that can \emph{d}-separate vertices in $S_\cap^c$ from $Y$. As a result, we have { $P(Y|\mathbf{X}_{S^\prime},do(\boldsymbol{x}_M)) \!=\! P(Y|\mathbf{X}_{S_\cap},do(\boldsymbol{x}_M)) = P(Y|\mathbf{X}_{S^{\prime \prime}},do(\boldsymbol{x}_M))$} and hence $\mathcal{R}_{S^\prime}\!=\!\mathcal{R}_{S_\cap}\!=\!\mathcal{R}_{S^{\prime \prime}}$. For example, in Fig.~\ref{fig: example graphical condition} (a), we have {$\{S_2\} \sim_G \{S_1,S_2\}$} because {$S_\cap=\{S_2\}$} can d-separate {$S_2^c=\{S_1,S_2\}\backslash \{S_2\}=\{S_1\}$ from $Y$}.

\begin{algorithm}[b!]
   \caption{(Informal) Equivalence Classes Recovery}
   \label{alg: recover g-equivalence}
\vspace{-0.1cm}
\begin{flushleft}
    \textbf{Input:} The stable graph $G_S$. \\
    \textbf{Output:} The equivalence classes $\mathrm{Pow}(S)/\!\sim_G$.
\end{flushleft}
\vspace{-0.2cm}
\begin{algorithmic}[1]
       \FUNCTION{$\text{Recover}(G_S)$}
        \IF{$\mathrm{Neig}(Y)=\varnothing$}
        \STATE \textbf{return} $\{\mathrm{Pow}(S)\}$.
        \ELSE
        \STATE $\mathrm{Pow}(S)/\!\sim_G \leftarrow \varnothing$.
        \FOR{$S^\prime$ \textbf{in} $\mathrm{Pow}(\mathrm{Neig}(Y))$}
        \STATE Construct a $\mathrm{MAG}$ from $G_S$ over $S \backslash \mathrm{Neig}(Y)$, with $S^\prime$ as the selection set, $\mathrm{Neig}(Y)\backslash S^\prime$ as the latent set.
        \vspace{+0.1cm}
        \STATE $\mathrm{Pow}(S)/\!\sim_G\text{.add}(\{S^\prime\} \cup \text{Recover}(\mathrm{MAG}))$.
        \ENDFOR
        \STATE\textbf{return} $\mathrm{Pow}(S)/\!\sim_G$.
        \ENDIF
       \ENDFUNCTION
\end{algorithmic}
\end{algorithm}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{icml23_figs/complexity_chain_tree.pdf}
    \caption{Illustration of the searching complexity. (a) A chain, where $N_G=6+1=7$. (b) A graph with disjoint chains, where $N_G=(2+1)^3=27$. (c) A tree consisting six chains, where $F_G=(l_1+l_3 l_4)(l_2+l_5 l_6), l_i:=\mathrm{len}(c_i)$. (d) A graph with cycles can be converted to subtrees via deleting edges to break the cycle, $c_1^i$ is attained by deleting the $1:i$ edges in $c_1$.}
    \label{fig:complexity_chain_tree}
    \vspace{-0.4cm}
\end{figure} 

With the equivalence relation, we can reduce the exhaustive search over $\mathrm{Pow}(S)$ to a search over $\mathrm{Pow}(S)/\!\sim_G$. To enable the search, we provide a $\mathrm{Pow}(S)/\!\sim_G$ recovery method in Alg.~\ref{alg: recover g-equivalence}. Given the input stable graph, Alg.~\ref{alg: recover g-equivalence} first finds $Y$'s neighbors. When $\mathrm{Neig}(Y)=\varnothing$, all subsets of $S$ are blocked from $Y$ and become equivalent. Thus, the algorithm returns a single equivalence class $\mathrm{Pow}(S)$. When $\mathrm{Neig}(Y)\neq \varnothing$, Alg.~\ref{alg: recover g-equivalence} goes over $S^\prime \subseteq \mathrm{Neig}(Y)$ to include them into the selection set. Here, the selection set contains variables used to predict $Y$; while the latent set contains those excluded from prediction. To explore vertices beyond $\mathrm{Neig}(Y)$, Alg.~\ref{alg: recover g-equivalence} constructs Maximal Ancestral Graphs (MAGs) \cite{spirtes2000causation} over $S\backslash\mathrm{Neig}(Y)$, where we can define the equivalence relation via \emph{m}-separation\footnote{Replace the \emph{d}-separation with \emph{m}-separation in Def.~\ref{def:equi}.}. This procedure is repeated recursively until $\mathrm{Neig}(Y)$ is empty.

\begin{proposition}
\label{prop:recover}
    Under Asm.~\ref{eq:assum-markov-faithfulness}, for each input graph that is Markov equivalent to the ground-truth $G_S$, Alg.~\ref{alg: recover g-equivalence} can correctly recover the $\mathrm{Pow}(S)/\! \sim_G$ in $O(N_G)$ time.
\end{proposition}


==> icml23_paras/old_method_xw/gequi_v2.tex <==
\vspace{-0.2cm}
\section{Searching $S^*$ among $g$-Equivalence}
\label{sec.learn}
\vspace{-0.1cm}

In this section, we provide an optimal subset selection algorithm in Alg.~\ref{alg:identify-f-star} that combines Thm.~\ref{thm:graph degenerate} and Thm.~\ref{thm:min-max}. Specifically, Alg.~\ref{alg:identify-f-star} (line 3) selects the whole stable set as $S^*$, if the graphical condition $Y \not\to \mathbf{W}$ is tested true. If this condition fails, a simple strategy is to \emph{exhaustively} compare $\mathcal{R}_{S_{-}}$ for all subsets, which is commonly adopted in the literature \cite{rojas2018invariant,magliacane2018domain,subbaswamy2019preventing,subbaswamy2020spec}. 


In this section, we provide a new searching strategy with better efficiency, by noticing that the exhaustive search can be redundant for subsets that have the same worst-case risk. Formally, we consider the stable graph $G_S$ of $G$ over $\mathbf{X}_S \cup Y$ and introduce the following equivalence via $d$-separation: 

\begin{algorithm}[tb]
   \caption{Optimal Subset Selection.}
\label{alg:identify-f-star}
\vspace{-0.2cm}
\begin{flushleft}
    \textbf{Input:} The training data $\{D_{e}|e\in\mathcal{E}_{\text{tr}}\}$. \\
    \textbf{Output:} The optimal subset $S^*$.
\end{flushleft}
\vspace{-0.2cm}
\begin{algorithmic}[1]
   \STATE Causal discovery of $G, \mathbf{W}$, and whether $Y \to \mathbf{W}$.
   \STATE \textbf{if} {$Y \not \to \mathbf{W}$} \textbf{then}
        \STATE \quad $S^* \leftarrow S$. \hfill{\# Thm.~\ref{thm:graph degenerate}} 
   \STATE \textbf{else}
    \STATE \quad  Recover $\mathrm{Pow}(S)\backslash\!\sim_G$ by Alg.~\ref{alg: recover g-equivalence}.
    \STATE \quad  $\mathcal{L}_{\min}\leftarrow \infty$.
        \STATE \quad \textbf{for} {$[S_{-}]$ \textbf{in} $\mathrm{Pow}(S)\backslash \!\sim_G$} \textbf{do}
        \STATE \quad \quad \textbf{if} {$\mathcal{L}_{S_{-}} <\mathcal{L}_{\min}$} \textbf{then}
            \STATE \quad \quad \quad $\mathcal{L}_{\min} \leftarrow \mathcal{L}_{S_{-}}$, $S^* \leftarrow S_{-}$. \hfill{\# Thm.~\ref{thm:min-max}} 
            \STATE \quad \quad \textbf{end if}
        \STATE \quad \textbf{end for}
    \STATE \textbf{end if} \textbf{return} $S^*$.
\end{algorithmic}
\end{algorithm}

\begin{definition}[$\sim_G$-equivalence]
\label{def:equi}
    Let $\sim_G$ be an equivalence relation on all subsets in $S$. We say two subsets $S_A$, $S_B$ are $\sim_G$-equivalence if $\exists \, S_{\cap} \subseteq S_A \cap S_B$ s.t.
    \begin{align*}
    (Y \perp \mathbf{X}_{S_\cap^c} | \mathbf{X}_{S_\cap})_{G_S}, \ \text{where } S_\cap^c:=(S_A\cup S_B) \backslash S_\cap. 
    \end{align*}
    We call elements of the quotient space $\mathrm{Pow}(S)\backslash\!\sim_G$ as $\sim_G$-equivalent classes, and $[S_-] \in \mathrm{Pow}(S)\backslash\!\sim_G$ as the $\sim_G$-equivalent class of $S_{-}$. We denote $N_G:=|\mathrm{Pow}(S)\backslash\!\sim_G\!|$ as the number of equivalent classes. 
\end{definition}

Graphically, $S_A$ and $S_B$ are $\sim_G$-equivalent if they share an intersection set $S_\cap$ that can \emph{d}-separate $S_\cap^c$ from $Y$. As a result, we have {\small $P(Y|\mathbf{X}_{S_A},do(\boldsymbol{x}_M)) \!=\! P(Y|\mathbf{X}_{S_\cap},do(\boldsymbol{x}_M)) = P(Y|\mathbf{X}_{S_B},do(\boldsymbol{x}_M))$}. Therefore, we have $\mathcal{R}_{S_A}\!=\!\mathcal{R}_{S_B}$. To illustrate, we have {\small $S_2 \sim_G \{S_1,S_2\}$} in Fig.~\ref{fig: example graphical condition} (a) since {\small $S_\cap=S_2$} can d-separate {\small $S_2^c:=\{S_1,S_2\}\backslash S_2=S_1$ from $Y$}. 



\begin{algorithm}[h]
   \caption{(Informal) \emph{g}-Equivalence Recovery}
   \label{alg: recover g-equivalence}
\vspace{-0.2cm}
\begin{flushleft}
    \textbf{Input:} The stable graph $G$ \protect \footnote{We omit the subscript $S$ for brevity. We only require the input to be Markovian equivalent to $G$. The formal version is at Alg.~\ref{alg: recover g-equivalence detail}.}. \\
    \textbf{Output:} The \emph{g}-equivalent classes $\mathrm{Pow}(S)\backslash\!\sim_G$.
\end{flushleft}
\vspace{-0.2cm}
\begin{algorithmic}[1]
       \FUNCTION{$\text{Recover}(G)$}
        \IF{$\mathrm{Neig}(Y)=\varnothing$}
        \STATE \textbf{return} $\{\mathrm{Pow}(S)\}$.
        \ELSE
        \STATE $\mathrm{Pow}(S)\backslash\!\sim_G \leftarrow \varnothing$.
        \FOR{$S_-$ \textbf{in} $\mathrm{Pow}(\mathrm{Neig}(Y))$}
        \STATE Construct a MAG $\tilde{G}$ from $G$ over $S \backslash \mathrm{Neig}(Y)$, with $S_-$ as the selection set, $\mathrm{Neig}(Y)\backslash S_-$ as the latent set.
        \vspace{+0.1cm}
        \STATE $\mathrm{Pow}(S)\backslash\!\sim_G\text{.add}(\{S_-\} \cup \text{Recover}(\tilde{G}))$.
        \ENDFOR
        \STATE\textbf{return} $\mathrm{Pow}(S)\backslash\!\sim_G$.
        \ENDIF
       \ENDFUNCTION
\end{algorithmic}
\end{algorithm}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{icml23_figs/complexity_chain_tree.pdf}
    \caption{Illustration of the searching complexity. (a) A chain, where $N_G=6+1=7$. (b) A graph consisting disjoint chains, where $N_G=(2+1)^3=27$. (c) A tree consisting six chains, where $F_G=(l_1+l_3 l_4)(l_2+l_5 l_6)$. (d) A graph with cycle can be converted to subtrees by deleting edges to break the cycle, where $c_1^i$ is attained by deleting the $1:i$ edges in $c_1$.}
    \label{fig:complexity_chain_tree}
    \vspace{-0.4cm}
\end{figure}

With $\sim_G$-equivalence, we can reduce the exhaustive search over $\mathrm{Pow}(S)$ to a search over $\mathrm{Pow}(S)\backslash\!\sim_G$. To enable the search, we provide a $\mathrm{Pow}(S)\backslash\!\sim_G$ recovery method in Alg.~\ref{alg: recover g-equivalence}. Given the input stable graph $G_S$, Alg.~\ref{alg: recover g-equivalence} first finds $Y$'s neighbors. When $\mathrm{Neig}(Y)=\varnothing$, all subsets of $S$ are blocked from $Y$ and $\sim_G$-equivalent. Thus, the algorithm returns a single $\sim_G$-equivalent class $\mathrm{Pow}(S)$. When $\mathrm{Neig}(Y)\neq \varnothing$, Alg.~\ref{alg: recover g-equivalence} goes over $S_-\subseteq \mathrm{Neig}(Y)$ to include them into the prediction set. By taking $S_-$ as selection set and $\mathrm{Neig}(Y)\backslash S_-$ as the latent set, it then constructs Maximal Ancestral Graphs (MAGs) over $S\backslash\mathrm{Neig}(Y)$, in which we can define equivalent subsets via $m$-separation\footnote{Def.~\ref{def:equi} is the same except that $d$-separation is replaced with $m$-separation.} \cite{zhang2008completeness} beyond $\mathrm{Neig}(Y)$. This procedure is repeated until $\mathrm{Neig}(Y)$ is empty. 

%We use the MAGs because they can represent \emph{d}-separations when selection (\emph{i.e.}, variables included into the prediction set) and latent (\emph{i.e.}, variables excluded from the prediction set) variables exist.

\begin{proposition}
\label{prop:recover}
    Under Asm.~\ref{eq:assum-markov-faithfulness}, for each input graph that is Markov equivalent to the input stable graph, Alg.~\ref{alg: recover g-equivalence} can correctly recover the $\mathrm{Pow}(S)\backslash\! \sim_G$ in $O(N_G)$ time.
\end{proposition}


==> icml23_paras/old_method_xw/minimax.tex <==
\section{Minimax Analysis for the Optimal Subset}
\label{sec.identify}

%In this section, we establish theoretical results regarding the robustness aspect. Our results answer two key questions: \textbf{i)} In which kind of causal DAG does the whole stable set $S$ reach the minimax optimum? \textbf{ii)} When $S$ may not be optimal, how to \emph{consistently} measure the robustness of each subset on (infinitely many) deployment environments, using only data from a few training environments?

In this section, we provide a comprehensive analysis regarding the min-max optimal subset, to resolve the problems of the surgery estimator. Specifically, we first provide a graphical condition that is equivalent to the \emph{degeneration condition}, for the whole stable set to be optimal, \emph{i.e.}, $S = S^*$. Not only does this condition provide a more intuitive perspective from the graph structure, compared to the degeneration condition; but more importantly, it can be easily tested via causal discovery. When this condition is not met, we propose an optimization scheme that is provable to identify the worst-case risk for each subset, equipped with which we can pick up the $S^*$ as the one with minimal worst-case risk. 

In the following, we first introduce the graphical condition for $S=S^*$, which is equivalent to the degeneration condition, as summarized in Thm.~\ref{thm:graph degenerate}. 


% show that for each subset, the worst-case risk can be attained when the conditional causal factor of $\mathbf{X}_M$, \emph{i.e.}, $P(\mathbf{X}_M|Pa(\mathbf{X}_M))$ degenerates to the delta function of $h(Pa(\mathbf{X}_M))$ for some $h$. This result inspires us to optimize the function of $Pa(\mathbf{X}_M)$ to estimate the worst-case risk 
% translate the \emph{degeneration condition}into an equivalent graphical criterion for the whole stable set to be optimal, \emph{i.e.}, $S = S^*$. Not only this 
%In the following, we first provide the answer to the first question. We find whether the interventional distribution can degenerate is decided by connections between $Y$ and a vertices set $\mathbf{W}$ in the causal DAG. If $Y$ does not point to any member of $\mathbf{W}$, the \emph{do} in $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can be removed and the minimax optimum is reached by the whole stable set $S$. 
\begin{theorem}[Graphical Condition for $S^*\!=\!S$]
\label{thm:graph degenerate}
Suppose asmp.~\ref{eq:assum-dag} holds. Denote $\mathbf{X}_{M}^{0}\!:=\!\mathbf{X}_{M}\cap \mathrm{Ch}(Y)$ as mutable variables in $Y$'s children, and $\mathbf{W}:=\mathrm{De}(\mathbf{X}_{M}^{0}) \backslash \mathbf{X}_M^0$ as descendants of $\mathbf{X}_{M}^{0}$. Then, $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution if and only if $Y$ does not point to any vertex in $\mathbf{W}$. Further, under either of the two conditions, $S^*=S$.
\end{theorem}
% \vspace{-0.1cm}
% since $X_i$ is not allowed to belong to $\mathbf{X}_M = \mathbf{X}_M^0 \cup \mathbf{X}_M \backslash \mathbf{X}_M^0$ :=\mathbf{X} \backslash \mathbf{X}_M
%The proof is left in the appendix. To understand this equivalence, note that the $v$-structure (\emph{e.g.}, $i \to j \gets k$) violates the ``do"-operator in $P(i|j,do(k))$ to be removed. In our scenario, this $v$-structure corresponds to $Y \to X_i \gets \mathbf{X}^0_M$ if we let $Y \to X_i \in \mathbf{W}$, where we have $X_i \in \mathbf{X}_S$ since it can neighther belong to $\mathbf{X}_M^0$ nor $\mathbf{X}_M \backslash \mathbf{X}_M^0$ according to the definition of $\mathbf{X}_M^0$. As a result, $P(Y|\mathbf{X}_S, do(\mathbf{x}_m))$ cannot degenerate to the conditional distribution. To illustrate, we consider examples shown in Fig.~\ref{fig: example graphical condition}, in which $Y \not\to \mathbf{W}$ (\emph{i.e.}, degeneration condition holds) and $Y \to \mathbf{W}$ (\emph{i.e.}, degeneration condition does not hold) in Fig.~\ref{fig: example graphical condition} (a) and Fig.~\ref{fig: example graphical condition} (b), respectively. In Fig.~\ref{fig: example graphical condition} (b), the $v$-structure in $Y \to X_1 \gets X_m$ can make it fail to remove ``do" in $P(Y|X_1,do(x_m))$. In Fig.~\ref{fig: example graphical condition} (a), since $Y \not\to X_1$ and $(Y \perp X_1,X_m|X_2)_{G_{\overline{X}_m}}$, we have $P(Y|X_1,X_2,do(x_m)) = P(Y|X_2)$ according to inferential rules in \cite{pearl2009causality}. 


The proof is left in the appendix. To understand this equivalence, note that if $Y$ does not point to any member of $\mathbf{W}$, we can use the rules \citep{pearl2009causality} of \textit{\emph{do}-calculus} to remove the ``do" in $p(y|\boldsymbol{x}_S, do(\boldsymbol{x}_M))$ and degenerate it into $p(y|\boldsymbol{x}\backslash(\boldsymbol{x}_M^0 \cup de(\boldsymbol{x}_M^0)))$. For example, in Fig.~\ref{fig: example graphical condition} (a), since $Y \not\to X_{S_1}$ and $(Y \perp X_{S_1},X_M|X_{S_2})_{G_{\overline{X}_M}}$, we have $p(y|{x_{S_1}},x_{S_2},do(x_M))=p(y|x_{S_2},do(x_M))=p(y|x_{S_2})$ according to inferential rules in \cite{pearl2009causality}. On the contrary, if $Y$ points to $\mathbf{W}$, then there exists a collider in $\mathbf{W}$ in some paths between $Y$ and $\mathbf{X}_M^0$, making it incapable to remove the ``do''. For example, in Fig.~\ref{fig: example graphical condition} (b), such a collider between $Y$ and $X_M$ refers to $X_{S_1}$, hence making it fail to remove ``do" in $p(y|x_{S_1},do(x_M))$.


% Such a degeneration (to conditional distribution) permits us to construct a probability distribution in $\mathcal{P}$ for any predictor $f$, that has larger or equal quadratic loss than $f_S$, thus proving the optimality of $f_S$. 
% (in our case, $Y \to X_i \gets \mathbf{X}_M$, with $X_i \in \mathbf{X}_S$) can violate $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ to degenerate to the conditional distribution. Concretely, this $v$-structure corresponds to $Y \to X_i \gets \mathbf{X}^0_M$ if we let $Y \to X_i \in \mathbf{W}$, where we have $X_i \in \mathbf{X}_S:=\mathbf{X} \backslash \mathbf{X}_M$ since $X_i$ is not allowed to belong to $\mathbf{X}_M = \mathbf{X}_M^0 \cup \mathbf{X}_M \backslash \mathbf{X}_M^0$ according to the definition of $\mathbf{X}_M^0$. To illustrate, we consider examples shown in Fig.~\ref{fig: example graphical condition}, in which $Y \not\to \mathbf{W}$ and $Y \to \mathbf{W}$ (therefore correspondingly we have the degeneration condition holds and not hold) respectively in Fig.~\ref{fig: example graphical condition} (a) and Fig.~\ref{fig: example graphical condition} (b). Fig.~\ref{fig: example graphical condition} (b), the $v$-structure in $Y \to X_1 \gets X_m$ can make it fail to remove ``do" in $P(Y|X_1,do(x_m))$. In contrast in Fig.~\ref{fig: example graphical condition} (a), since $Y \not\to X_1$ and $(Y \perp X_1,X_m|X_2)_{G_{\overline{X}_m}}$, we have $P(Y|X_1,X_2,do(x_m)) = P(Y|X_2)$ according to inferential rules in \cite{pearl2009causality}. 


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{icml23_figs/examples_thm3.1.pdf}
    \caption{Illustration of the graphical condition in Thm.~\ref{thm:graph degenerate}. The sets $\mathbf{X}_M=\mathbf{X}_M^0$ and $\mathbf{W}$ are marked as red and blue, respectively.}
    \label{fig: example graphical condition}
\end{figure}







%\begin{proofsketch}
%    If $Y$ does not point to any member of $\mathbf{W}$, we can use the inference rules \cite{pearl2009causality} to remove the ``\emph{do}'' in $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ and degenerate it into $P(Y|\mathbf{X}\backslash (\mathbf{X}_M^0 \cup \mathrm{De}(\mathbf{X}_M^0)))$. For example, in Fig.~\ref{fig: example graphical condition} (a), we have $P(Y|X_1,X_2, do(\boldsymbol{X}_m))=P(Y|X_2, do(\boldsymbol{x}_m))=P(Y|X_2)$. Such a degeneration (to conditional distribution) permits us to construct a probability distribution in $\{P^e| e \in \mathcal{E}\}$ for any predictor $f$, where $f$ has a larger or equal worst-case risk than $f_S$, thus proving the optimality of $S$. On the contrary, when $Y$ points to a member of $\mathbf{W}$, there is a collider ($X_1$ in Fig.~\ref{fig: example graphical condition} (b)) in $\mathbf{X}\backslash \mathbf{X}_M^0$ in some paths between $Y$ and $\mathbf{X}_M^0$. Conditioning on the collider will open the indirect path between $Y$ and $\mathbf{X}_M^0$, making it incapable to remove the ``\emph{do}''.
%\end{proofsketch} 
%\vspace{-0.1cm}


The following proposition states that this graphical condition can be tested. 


%facilitates an easier way to test the criterion via causal discovery. 
%Such a connection provides an intuitive explanation for the robustness of the whole stable set. It also saves end-users from running the inference rules to check the degeneration condition and makes the result easily accessible from the causal DAG, as guaranteed by the following proposition.

\begin{proposition}[Testability of the graphical condition]
	\label{prop.thm3.2 justifiability}
	Under asmp.~\ref{eq:assum-dag}-\ref{assum:e-train}, we have that \textbf{i)} the $\mathbf{W}$ is identifiable; and \textbf{ii)} the condition $Y \to \mathbf{W}$ is testable from $\{P^e(\mathbf{X},Y)\}_{\mathcal{E}_{\mathrm{Tr}}}$.
\end{proposition}

% \begin{remark}
% \label{remark:test}
%     To identify $\mathbf{W}:=\mathrm{De}(\mathbf{X}_M^0)\backslash \mathbf{X}_M^0$, we employ causal discovery from multiple domains (obtained by the environmental variable $E$) in \cite{huang2020causal}. Specifically, we first identify $\mathbf{X}_M$ as those variables $X_i \not\perp E | \mathbf{X}'$ for any $\mathbf{X}' \subset \mathbf{X}$. Then we can identify $\mathrm{Ch}(X_i)$ and $\mathrm{Pa}(X_i)$ for each $X_i \in \mathbf{X}_M$, by employing the hypothesis testing via Hilbert Schmidt Independence Criterion (HSIC) norm \cite{huang2020causal, gretton2007kernel}. In this regard, we can identify $\mathbf{X}_M^0:=\mathbf{X}_M \cap \mathrm{Ch}(Y)$. Following this procedure iteratively, we can identify $\mathrm{Ch}(X_i)$ and $\mathrm{Pa}(X_i)$ for each $X_i \in \mathrm{De}(\mathbf{X}_M^0)$. Therefore, we can identify $\mathbf{W}:=\mathrm{De}(\mathbf{X}_M^0)\backslash \mathbf{X}_M^0$ and whether $Y \to \mathbf{W}$. Details are left in Sec. \textcolor{blue}{??} in the appendix. 
% \end{remark}

Compared to the degeneration condition, the graphical condition in Thm.~\ref{thm:graph degenerate} connects the minimax property to the graphical structure. Rather than exhaustively running the inference rules to check the degeneration condition adopted in \cite{subbaswamy2019preventing}, this connection inspires us to simply test the condition via causal discovery. Specifically, we first learn the skeleton of the graph $G$ and leverage the heterogeneity among multiple training environments to detect $\mathbf{X}_M^0$ and $\mathbf{W}$ \cite{huang2020causal}. Then we determine whether there is a directed edge from $Y$ to $\mathbf{W}$, in order to test the graphical condition.

Thm.~\ref{thm:graph degenerate} only provides a sufficient condition of the optimality. When this condition fails, the $S$ may not necessarily be optimal. To illustrate, we construct an example with Fig.~\ref{fig: example graphical condition} (b) as the causal graph, in which $Y, X_M, X_{S_1}$ are binary variables. We then have the following result: 
\begin{proposition}
\label{prop:counter}
There exists $P(Y)$ and $P(X_{S_1}|X_M, Y)$, such that $f_{S}:=\mathbb{E}[Y|X_{S_1},do(X_M)]$ has larger maximal loss than $f_{\emptyset} = \mathbb{E}[Y|do(X_M)]$: 
\begin{align*}
    \max_{P^e} \mathbb{E}_{P^e}[Y-f_S]^2 > \max_{P^e} \mathbb{E}_{P^e}[Y-f_\emptyset]^2.
\end{align*}
\end{proposition}
This example implies the possibility of the whole stable set not being optimal when the graphical condition does not hold. Under these cases, it still remains unknown that \emph{which subset of stable information is the optimal one to transfer?} To answer this question, we note that the optimal subset has minimal worst-case risk. Therefore, it is sufficient to estimate the worst-case risk denoted as $\mathcal{R}(S_{-})\!:=\!\max_{e \in \mathcal{E}} \mathbb{E}_{P^e}[\left(Y \!-\! f_{S_{-}}(\boldsymbol{x})\right)^2]$ for each $S_{-}$. 

% Under some conditions on $P(Y)$ and $P(X_{S_1}|X_M, Y)$, we show that $f_S$ with the whole stable set $S:=\{S_1\}$ has larger maximal loss than $f_\emptyset$. 

To estimate the worst case risk, we consider a distribution family  $\{P_h\}_{h}$, where $h$ is a Borel function from $\mathrm{PA}(\mathbf{X}_M)$ to $\mathbf{X}_M$ and $P_h\! :=\! p(y,\boldsymbol{x}_S| do(\mathbf{X}_M\!=\!h(pa(\boldsymbol{x}_M)))$. This distribution keeps the invariant mechanisms on $Y$ and $\mathbf{X}_S$ unchanged while allowing the $\mathbf{X}_M$ given their parents to vary arbitrarily, in order to mimic the behavior of the worst-case quadratic loss. Therefore, we can obtain the worst-case loss for each subset $S_-$ by considering its maximal expected loss over $h \in \mathcal{B}$, where $\mathcal{B}$ denotes the set of Borel functions from $\mathbb{R}^{|\mathrm{Pa}(\mathbf{X}_M)|}$ to $\mathbb{R}^{|\mathbf{X}_M|}$. This is formalized in the following theorem. 

%To answer this question, we note that the optimal subset has minimal worst-case risk. Therefore, it is sufficient to estimate the worst-case risk for each subset. 

%By implementing causal discovery, we have $S^* = S$ if the graphical criterion holds, \emph{i.e.}, $Y \not\to \mathbf{W}$. If this condition fails, we provide an example in Sec. \textcolor{blue}{??} in the appendix to show that the whole stable set is not necessarily optimal. In these cases, it remains unknown that \emph{which subset of stable information is the optimal one to transfer?} From the min-max perspective, the optimal subset is the one with the minimal worst-case risk. Therefore, to answer this question, it is sufficient to identify the worst-case risk for each subset. 

%To accurately estimate the worst-case risk, it is key to notice from our causal factorization in Eq.~\eqref{eq: causal factorization} that the heterogeneity of $\mathcal{E}$ is governed by the mutable mechanisms of $\mathbf{X}_M$ condition on its parents, because it is the only source of variation across $\mathcal{E}$. This motivates us to parameterize these mechanisms and optimize them to explore the worst-case environment. Formally, we consider the family $\{P_h:=P(Y,\mathbf{X}_S| do(\mathbf{X}_M\!=\!h(\mathrm{Pa}(\mathbf{X}_M)))\}_{h}$, where $h$ is a Borel measurable function that maps from $\mathrm{Pa}(\mathbf{X}_M)$ to $\mathbf{X}_M$. Correspondingly, we denote $\mathcal{B}$ as the set of Borel functions from $\mathbb{R}^{|\mathrm{Pa}(\mathbf{X}_M)|}$ to $\mathbb{R}^{|\mathbf{X}_M|}$. The following theorem shows that the worst-case risk for each subset can be attained at some $P_{h^*}$ for some $h^* \in \mathcal{B}$. 

% mutable mechanisms of $\mathbf{X}_M 

%Our key observation to solve this problem is that all environments in $\mathcal{E}$, no matter how various their behaviors are, are governed by the causal DAG $G$, where the only source of variation is the mutable causal mechanisms of $\mathbf{X}_M$. In this regard, we can parameterize these mutable mechanisms and let them vary arbitrarily, which provides a simulation of the worst-case environment. Each subset's generalization ability on this simulation environment can thus \emph{consistently} reflect its robustness on $\mathcal{E}$. 

% What makes the parameterization plausible is that we find $\mathbf{X}_M$ is always a \emph{definite} function of $\mathrm{Pa}(\mathbf{X}_M)$ when the worst-case risk is attained. In this regard, we can parameterize $h\!:\!\mathrm{Pa}(\mathbf{X}_M)\!\to\!\mathbf{X}_M$ with a neural network $h_\theta$ and maximize over $\theta$ to estimate the worst-case risk, due to its ability to approximate any definite function \cite{hornik1989multilayer}. Formally, define an instrumental distribution family $\{P_h\}_{h}$, with $h$ a definite function from $\mathrm{Pa}(\mathbf{X}_M)$ to $\mathbf{X}_M$ and $P_h\! :=\! P(Y,\mathbf{X}_S| do(\mathbf{X}_M\!=\!h(\mathrm{Pa}(\mathbf{X}_M)))$, we have the following minimax property:

\begin{theorem}[Minimax Property]
\label{thm:min-max}
For each subset $S_{-} \subset S$, 
%denote $\mathcal{R}(S_{-})\!:=\!\max_{e \in \mathcal{E}} \mathbb{E}_{P^e}[\left(Y \!-\! f_{S_{-}}(\boldsymbol{x})\right)^2]$ as the worst-case risk on $\mathcal{E}$. 
denote $\mathcal{L}(S_{-}):=\max_{h \in  \mathcal{B}}\mathbb{E}_{P_h}[(Y \!-\! f_{S_{-}}(\boldsymbol{x}))^2]$ as the maximal population loss over $P_h$. Then, we have $\mathcal{R}(S_{-})=\mathcal{L}(S_{-})$. Further, this means we can select the optimal subset as $S^* := \mathop{\mathrm{argmin}}_{S_{-} \subseteq S} \mathcal{L}(S_{-})$.
\end{theorem}



%To achieve this identification, we first show that the worst-case risk can be attained when the conditional factor of $\mathbf{X}_M$, \emph{i.e.}, $P^e(\mathbf{X}_M|\mathrm{Pa}(\mathbf{X}_M)$ that governs the distributional shifts across $\mathcal{E}$, degenerates to the delta function of $h^*(\mathrm{Pa}(\mathbf{X}_M))$ for some function $h^*$, as summarized in the following Thm.~\ref{thm:min-max}. This theorem turns the worst risk estimation problem into an optimization problem over the function $h$ that maps from $\mathrm{Pa}(\mathbf{X}_M)$ to $\mathbf{X}_M$. 

%\begin{theorem}[Minimax Property]
%\label{thm:min-max}
%Denote $\mathcal{R}(S_{-})\!:=\!\max_{e \in \mathcal{E}} \mathbb{E}_{P^e}[\left(Y \!-\! f_{S_{-}}(\boldsymbol{x})\right)^2]$ as the worst-case risk for each subset $S_{-} \subset S$. We have that $\mathcal{R}(S_{-})$ can be attained, if the $P^e(\mathbf{X}_M|\mathrm{Pa}(\mathbf{X}_M))$ of $P^e$ in Eq.~\eqref{eq: causal factorization} degenerates to $\mathbbm{1}(\mathbf{X}_M=h^*(\mathrm{Pa}(\mathbf{X}_M))$ for some $h^*: \mathrm{Pa}(\mathbf{X}_M) \to \mathbf{X}_M$. 
%\end{theorem}

%\begin{remark}
   %This result means for each $\mathrm{Pa}(\mathbf{x}_M)$, there exists $\mathbf{x}_M$ such that the predictor $f_{S_-}(\mathbf{x})$ has the largest prediction error on $P(Y,\mathbf{X}_S|do(\mathbf{X}_M=\mathbf{x}_M))$ among $\mathcal{P}$. The $h^*$ is the function that maps from $\mathrm{Pa}(\mathbf{x}_M)$ to $\mathbf{x}_M$.
   %condition on each $\mathrm{Pa}(\mathbf{x}_m)$, the intervention on $\mathbf{X}_M$ via $h$ define a generating mechanism to generate data for $\mathbf{X}_M$; and $h^*$ generates the data on which the predictor $f_{S{-}}(\mathbf{x})$ has largest prediction error. 
    %no matter how various their behaviors are, are governed by the causal DAG $G$, where the only source of variation is the mutable causal mechanisms of $\mathbf{X}_M$. In this regard, we can parameterize these mutable mechanisms and let them vary arbitrarily, which provides a simulation of the worst-case environment. Each subset's generalization ability on this simulation environment can thus \emph{consistently} reflect its robustness on $\mathcal{E}$. 
%\end{remark}


Inspired by this result, we consider the following optimization problem over the function $h \in  \mathcal{B}$: 
\begin{align*}
    \max_{h \in  \mathcal{B}} \mathcal{L}_{S_{-}}(h) := \mathbb{E}_{P_h}[(Y \!-\! f_{S_{-}}(\boldsymbol{x}))^2].
\end{align*}
According to Thm.~\ref{thm:min-max}, this optimization approach is guaranteed to attain the worst-case risk $\mathcal{R}(S_-)$. To implement, we parameterize $h\!:\!\mathrm{Pa}(\mathbf{X}_M)\!\to\!\mathbf{X}_M$ with a neural network $h_\theta$ and optimize over $\theta$, inspired by the ability of the neural network to approximate any Borel measurable function \cite{hornik1989multilayer}. The following result shows that $\mathcal{L}_{S_{-}}(h)$ is identifiable, which ensures the tractability of this optimization. 

% Since $P_h \in \{P^e\}_{e \in \mathcal{E}}$, we have $\max_h \mathcal{L}_{S_{-}}(h) = \mathcal{R}(S_{-})$ according to Thm.~\ref{thm:min-max}. Therefore, the maximum value can attain the worst-case risk for $S_-$, \emph{i.e.}, $\mathcal{R}(S_{-})$. Intuitively speaking, since the variation of $P^e$ comes from the mutable causal mechanism of $\mathbf{X}_M$, we keep the stable mechanism $P(\mathbf{X}_S|\mathrm{Pa}(\mathbf{X}_S))$ unchanged and take the intervened function of $\mathbf{X}_M$ as parameters; and optimize to find the intervened function that corresponds to the worst-case environment among $\{P^e\}_{\mathcal{E}}$. 

% condition on each $\mathrm{Pa}(\mathbf{x}_m)$, this optimization is exploring thethis optimization is is letting the generating mechanism of $\mathbf{X}_M$  

\begin{proposition}
	\label{prop.thm3.3 justifiability}
	Under asmp.~\ref{eq:assum-dag}-\ref{assum:e-train}, the  $P_h$, $f_{S_-}$ and hence $\mathcal{L}_{S_{-}}(h)$ are identifiable. 
\end{proposition}

%\begin{remark}
%    According to remark~\ref{remark:test}, we can identify $\mathrm{P}(X_i)$ and $\mathrm{Ch}(X_i)$ for each $X_i \in \mathrm{De}(\mathbf{X}_M^0)$. Therefore, the $\mathrm{Pa}(\mathbf{X}_M)\backslash \mathbf{X}_M$ satisfies the back-door criterion and thus can be taken as admissible set \cite{pearl2009causality} to make the $P(Y,\mathbf{X}_S|\mathbf{X}_M)$ identifiable. 
%\end{remark}

%For practical estimation, we propose a permutation-regeneration method, the core of which is based on the identification of $\mathbf{X}_M$, $\mathbf{X}_M$


% For practical estimation of $f_{S_{-}}$ (the estimation of $\mathcal{L}_{S_{-}}(h)$ is similar), we propose a permutation-regeneration method. Specifically, we first notice that the predictor $f_{S_-}:=\mathbb{E}_{P}[Y|\mathbf{x}_S,do(\mathbf{x}_M)]=\mathbb{E}_{\tilde{P}}[Y|\mathbf{x}_S,\mathbf{x}_M]$, where $\tilde{P}$ changes the mutable factors from $P(\mathbf{X}_M|\mathrm{Pa}(\mathbf{X}_M))$ to $P(\mathbf{X}_M)$. To generate data from $\tilde{P}$ for empirical estimation, we first generate data from $P(\mathbf{X}_M)$ via sample-wise permutation. Then, we generate data for $\mathrm{De}(\mathbf{X}_M)$, by estimating $P(X_i|\mathrm{Pa}(X_i))$ for each $X_i \in \mathrm{De}(\mathbf{X}_M)$. This estimation is possible since we can identify $\mathrm{Ch}(X_i)$ and $\mathrm{Pa}(X_i)$ for each $X_i \in \mathrm{De}(\mathbf{X}_M^0)$ according to remark~\ref{remark:test}.

\textbf{Discussions.} Our results Thm.~\ref{thm:graph degenerate},~\ref{thm:min-max} answer the two questions raised in Sec.~\ref{sec.background}. Specifically, Thm.~\ref{thm:graph degenerate} provides an equivalent but more intuitive graphical condition to determine whether $S^*=S$; while Thm.~\ref{thm:min-max} motivates an optimization-based approach to identify the optimal subset $S^*$ under general scenarios. 

% via sample wise permutation for each $X_i \in \mathbf{X}_M$. In this regard, we have $f_{S_-}:=\mathbb{E}_{P}[Y|\mathbf{x}_S,do(\mathbf{x}_M)]=\mathbb{E}_{\tilde{P}}[Y|\mathbf{x}_S,\mathbf{x}_M]$ where $\tilde{P}$ 



%The maximizer can 

%Denote $\mathcal{L}(S_{-}):=\max_{h}\mathbb{E}_{P_h}[(Y \!-\! f_{S_{-}}(\boldsymbol{x}))^2]$ as the maximal population loss over $P_h$. Then, we have $\mathcal{R}(S_{-})=\mathcal{L}(S_{-})$. Thus, the optimal subset can be obtained via $S^* := \mathop{\mathrm{argmin}}_{S_{-} \subseteq S} \mathcal{L}(S_{-})$.







% Our key observation to solve this problem is that all environments in $\mathcal{E}$, no matter how various their behaviors are, are governed by the causal DAG $G$, where the only source of variation is the mutable causal mechanisms of $\mathbf{X}_M$. In this regard, we can parameterize these mutable mechanisms and let them vary arbitrarily, which provides a simulation of the worst-case environment. Each subset's generalization ability on this simulation environment can thus \emph{consistently} reflect its robustness on $\mathcal{E}$. 




%a new method dubbed as \emph{optimize to learn the min-max optimality}.  


%can examine whether $Y \to \mathbf{W}$. If $Y \not\to \mathbf{W}$, we can take $S^*$ as the whole stable set. When this condition fails, it is natural to ask: 


%On the other hand, Thm.~\ref{thm:graph degenerate} reminds us the sufficient condition for $S^*\!=\!S$ may not always hold. When the condition fails, including more stable information may not be always beneficial. Indeed, we provide a counter-example in Fig.~\ref{fig: example graphical condition} (b) that, the whole stable set ${\{X_2\}}$ has a larger generalization error than the empty set ${\varnothing}$, under some conditions\footnote{For details of these conditions, please refer to Sec. in the appendix.}on $P(Y)$ and $P(X_1|Y)$.

%To identify the $S^*$ when Thm.~\ref{thm:graph degenerate} fails, we attempt to measure the robustness of each subset $S_{-}$ with data from $\mathcal{E}_{tr}$. Indeed, there are infinitely many deployment environments, each having various behaviors in terms of the probability distribution. A few held-out validation environments from $\mathcal{E}_{tr}$ are hard, if not impossible, to reflect the behavior of the worst-case environment and measure the worst-case risk. 



%What makes the parameterization plausible is that we find $\mathbf{X}_M$ is always a \emph{definite} function of $\mathrm{Pa}(\mathbf{X}_M)$ when the worst-case risk is attained. In this regard, we can parameterize $h\!:\!\mathrm{Pa}(\mathbf{X}_M)\!\to\!\mathbf{X}_M$ with a neural network $h_\theta$ and maximize over $\theta$ to estimate the worst-case risk, due to its ability to approximate any definite function \cite{hornik1989multilayer}. Formally, define an instrumental distribution family $\{P_h\}_{h}$, with $h$ a definite function from $\mathrm{Pa}(\mathbf{X}_M)$ to $\mathbf{X}_M$ and $P_h\! :=\! P(Y,\mathbf{X}_S| do(\mathbf{X}_M\!=\!h(\mathrm{Pa}(\mathbf{X}_M)))$, we have the following minimax property:



%\begin{proofsketch}
%Firstly consider the case where $\mathbf{X}_M=\{X_m\}$. The $\mathcal{R}(S_{-})$ expands to:
%\begin{equation}
%    \mathcal{R}(S_{-}) = \max_{e \in \mathcal{E}} \int_{y,\boldsymbol{x}} [y-f_{S_{-}}(\boldsymbol{x})]^2 p^e(y,x_m,\boldsymbol{x}_{S_{-}}) dy d\boldsymbol{x}.
%\label{eq: risk}
%\end{equation}
%Factorize $p^e(y,x_m,\boldsymbol{x}_S)$ into disentangled causal factors and denote $\tilde{\mathbf{X}}:=\mathbf{X}\backslash (\{X_m\}\cup \mathrm{Pa}(X_m))$, we can split the integral into three parts, respectively over $\mathrm{pa}(x_m)$, $x_m$, and $y, \tilde{\boldsymbol{x}}$. Denote the last one as $g(x_m,\mathrm{pa}(x_m)):=\int_{y, \tilde{\boldsymbol{x}}} [y-f_{S_{-}}(\boldsymbol{x})]^2 p(y|\mathrm{pa}(y)) p(\tilde{\boldsymbol{x}}| \mathrm{pa}(\tilde{\boldsymbol{x}})) dyd\tilde{\boldsymbol{x}}$, Eq.~\ref{eq: risk} becomes:
%\begin{align}
%    &\mathcal{R}(S_{-}) = \max_{e \in \mathcal{E}} \int_{\mathrm{pa}(x_m)} \prod_{X_i \in \mathrm{Pa}(X_m)} p(x_i|\mathrm{pa}(x_i)) \nonumber \\ 
%    &\int_{x_m} g(x_m,\mathrm{pa}(x_m)) p^e(x_m|\mathrm{pa}(x_m)) dx_m d \mathrm{pa}(x_m).
%\end{align}
%Since $p^e((x_m|\mathrm{pa}(x_m)))$ is the only item varying with $e$, we can move the maximization to the inner integral and have:
%\begin{align}
%    \mathcal{R}(S_{-})=&\int_{\mathrm{pa}(x_m)} \prod_{X_i \in \mathrm{Pa}(X_m)} p(x_i|\mathrm{pa}(x_i)) \nonumber \\ 
%    &g(h^*(\mathrm{pa}(x_m)),\mathrm{pa}(x_m)) d \mathrm{pa}(x_m),
%\label{eq: definite function}
%\end{align}
%with $h^*(\mathrm{pa}(x_m))\!:=\!\arg\max_{x_m}g(x_m,\mathrm{pa}(x_m))$ is a definite function from $\mathrm{pa}(x_m)$ to $x_m$. Eq.~\ref{eq: definite function} indicates the worst-case risk is attained when $x_m$ is a definite function of $\mathrm{pa}(x_m)$ and thus shows $\mathcal{R}(S_{-})=\mathcal{L}(S_{-})$.

%In cases where $\mathbf{X}_M$ contains multiple variables, we can consider the maximization sequentially according to the topology order in $\mathbf{X}_M$. For details of the proof, please refer to Sec. in the appendix.
%\end{proofsketch}







==> icml23_paras/wang_advice/introduction_wang_mz_v1.tex <==
\vspace{-0.7cm}
\section{Introduction}
\vspace{-0.1cm}

Current machine learning systems, which are commonly deployed based on their in-distribution performance, often encounter \emph{dataset shifts} \cite{quinonero2008dataset} such as covariate shift, due to changes in the data generating process. When such a shift exists in deployment environments, the model may give unreliable prediction results, which can cause severe consequences in safe-critical tasks such as healthcare \citep{hendrycks2021many}. At the heart of this unreliability issue are \emph{stability} and \emph{robustness} aspects, which respectively denote the insensitivity of prediction behavior and generalization errors to dataset shifts. 

For example, consider the system deployed to predict the Functional Activities Questionnaire (FAQ) score that is commonly adopted \cite{mayo2016use} to measure the severity of Alzheimer's disease (AD). During the prediction, the system can only access biomarkers or volumes of brain regions as covariates, with demographic information anonymous for privacy consideration. However, the changes in such demographics can cause shifts in covariates. To achieve reliability for the deployed model, its prediction is desired to be stable against demographic changes, and meanwhile to be constantly accurate across all populations. For this purpose, this paper aims to find the most robust (\emph{i.e.}, minimax optimal) predictor, among the set of stable predictors across all deployed environments. 

To achieve this goal, many studies attempted to learn invariance to transfer to unseen data. Examples include ICP \cite{peters2016causal} and \citep{arjovsky2019invariant, liu2021heterogeneous, ahuja2021invariance,zhou2022sparse} that assumed and utilized the invariant prediction mechanism given causal features or representations; and  \citep{subbaswamy2019preventing,rothenhausler2021anchor} that explicitly attributed the variation to a prior selection diagram or an exogenous variable, then identified invariance by removing the varied features. However, an important question regarding robustness remains: \emph{which part of the invariance should the model transfer, in order to achieve optimal generalization ability?}

\begin{figure*}
\centering
\includegraphics[width=0.76\textwidth]{icml23_figs2/ad_results.png}
\caption{FAQ prediction in Alzheimer's disease. (a) Comparison of maximal mean square error (max. MSE) over deployed environments. (b) Max. MSE of subsets that are ranked in the ascending order from left to right, respectively according to the estimated worst-case risk of our method (marked by red) and the validation's loss adopted in \citep{subbaswamy2019preventing} (marked by blue). }
\vspace{-0.2cm}
\label{fig:adni-intro}
\end{figure*}

In this paper, we provide a comprehensive answer from the perspective of causality. We first identify a set of invariant features based on the \emph{sparse mechanism shift hypothesis} \cite{scholkopf2021toward}. Specifically, we posit the dataset shifts as the result of changes in a subset of the causal model's mechanisms, and correspondingly call the set of variables with changed (resp. unchanged) causal mechanisms the mutable $M$ (resp. stable $S$) set. Equipped with causal discovery and the ``do'' operator, we detect the mutable set and remove its mutation, resulting a set of invariant features, each of which corresponds to a stable subset in $S$. 

To further select the most robust feature for transfer, we study the minimax property of these stable features via the lens of Causal Graphical Model (CGM). Specifically, we first provide a graphical condition that is sufficient for the whole stable set to be optimal. This condition can be easily tested via causal discovery. When this condition fails, we construct an example that counter-intuitively shows that this whole stable set, although keeps all stable information, is \textbf{NOT} the optimal one to transfer. Under these cases,
we investigate the mutable mechanisms and propose to optimize the intervention on the mutable set, in order to mimic the worst-case deployed environment. We show that such an optimization-based approach can attain the worst-case risk for each stable subset, which is crucial to selecting the optimal subset in an accurate way. Back to the FAQ prediction example, Fig.~\ref{fig:adni-intro} (b) shows that our method can consistently estimate the maximal mean squared error (max. MSE) for each subset, while the validation's loss adopted by \cite{subbaswamy2019preventing} fails. This result explains our advantage in predicting FAQ across patient groups shown in Fig.~\ref{fig:adni-intro} (a). 

To efficiently search for the optimal subset, we define an equivalence relation between stable subsets via $d$-separation such that two equivalent subsets share the same worst-case risk. We theoretically show that compared to exhaustive searching over all subsets, searching over only equivalence classes can reduce the exponential complexity to the polynomial complexity. The effectiveness and efficiency of our methods are demonstrated by improved robustness, stability, and computation efficiency achieved on a synthetic dataset and the diagnosis of Alzheimer's disease. 

\textbf{Contributions.} We summarize our contributions as follows: 
\begin{enumerate}[noitemsep,topsep=0.1pt]
    \item We propose to identify the optimal subset of invariance to transfer, guided by a comprehensive minimax analysis from a causal perspective. To the best of our knowledge, this is the \emph{first} work to comprehensively study the problem of \emph{which invariance should we transfer}, in the literature of robust learning. 
    \item We define an equivalence relation between stable subsets, and accordingly propose to search over only equivalence classes. This new search algorithm can be efficiently solved in polynomial time. 
    \item We achieve better robustness and stability than others on synthetic data and Alzheimer's disease diagnosis. 
\end{enumerate}




==> icml23_paras/wang_advice/introduction_wang_xw_v2.tex <==
\vspace{-0.7cm}
\section{Introduction}
\vspace{-0.1cm}

Current machine learning systems, which are commonly deployed based on their in-distribution performance, often encounter \emph{dataset shifts} \cite{subbaswamy2019preventing} such as covariate shift, due to changes in the data generating process. When such a shift exists in deployment environments, the model may give unreliable prediction results, which can cause severe consequences in safe-critical tasks such as healthcare \citep{hendrycks2021many}. At the heart of this unreliability issue are \emph{stability} and \emph{robustness} aspects, which respectively denote the insensitivity of prediction behavior and generalization errors to dataset shifts. 

For example, consider the system deployed to predict the Functional Activities Questionnaire (FAQ) score that is commonly adopted \cite{mayo2016use} to measure the severity of Alzheimer's disease (AD). During the prediction, the system can only access biomarkers or volumes of brain regions as covariates, with demographic information anonymous for privacy consideration. However, the changes in such demographics can cause shifts in covariates. To achieve reliability for the deployed model, its prediction is desired to be stable against demographic changes, and meanwhile to be constantly accurate across all populations. For this purpose, this paper aims to find the most robust (\emph{i.e.}, minimax optimal) predictor, among the set of stable predictors across all deployed environments. 

To achieve this goal, many studies attempted to learn invariance to transfer to unseen data. Examples include ICP \cite{peters2016causal} and \citep{arjovsky2019invariant, liu2021heterogeneous, ahuja2021invariance} that assumed the prediction mechanism given causal features or representations to be invariant; or \citep{subbaswamy2019preventing, rothenhausler2021anchor} that explicitly attributed the variation to a prior selection diagram or an exogenous variable. These methods either suffer from restricted application scenarios in which only causal features are allowed to be invariant, or lack theoretical guarantee in terms of robustness. 

\begin{figure*}
\centering
\includegraphics[width=0.76\textwidth]{icml23_figs2/ad_results.png}
\caption{FAQ prediction in Alzheimer's disease. (a) Comparison of maximal mean square error (max. MSE) over deployed environments. (b) Max. MSE of subsets that are ranked in ascending order from left to right, respectively according to the estimated worst-case risk of our method (marked by red) and the validation loss of the surgery estimator \cite{subbaswamy2019preventing} (marked by blue). }
\vspace{-0.2cm}
\label{fig:adni-intro}
\end{figure*}

To resolve the first problem, we adopt the \emph{sparse mechanism shift hypothesis} \cite{scholkopf2021toward} that posits the dataset shifts as the result of changes in a subset of the causal model's mechanisms, and correspondingly call the set of variables with changed (resp. unchanged) causal mechanisms the mutable $M$ (resp. stable $S$) set. Equipped with causal discovery via heterogeneous data, we can detect the mutable set and intervene on them to obtain a set of stable predictors \cite{subbaswamy2019preventing}, each of which corresponds to a stable subset in $S$. Compared to ICP-related methods \cite{peters2016causal, buhlmann2020invariance}, such stable predictors can additionally exploit invariance from the output's effect, thus can be potentially applied to more general scenarios. However, an important question regarding robustness remains: \emph{which part of the invariance should the model transfer, in order to achieve optimal generalization ability?}




% Particularly, \cite{subbaswamy2019preventing,subbaswamy2020spec} causally decomposed the joint distribution into the mutable ($M$) set and the stable ($S$) set, which contains variables with changed and unchanged causal mechanisms, respectively. By intervening on $M$, they can obtain a set of stable predictors, each of which is based on a stable subset in $S$. To further find the most robust predictor, the following question remains: \emph{which subset of $S$ should the model transfer, in order to be most robust against dataset shifts?} 

%In \cite{subbaswamy2019preventing}, this optimal subset is simply taken as the one with the minimal validation loss, which lacks theoretical guarantees as the validation environment may not reflect the worst-case risk over deployed environments, as shown by Fig.~\ref{fig:adni-intro} (b). 





To answer this question, we give a comprehensive analysis from the perspective of causality. Specifically, we first provide a graphical condition that is sufficient for the whole stable set to be optimal. This condition can be easily tested via causal discovery. When this condition fails, we construct an example that counter-intuitively shows that this whole stable set, although keeps all stable information, is \textbf{NOT} the optimal one to transfer. Under these cases,
we investigate the mutable mechanisms and propose to optimize the intervention on the mutable set, in order to mimic the worst-case deployed environment. We show that such an optimization-based approach can attain the worst-case risk for each stable subset, which is crucial to select the optimal subset in a more accurate way. Back to the FAQ prediction example, Fig.~\ref{fig:adni-intro} (b) shows that our method can well reflect the maximal mean squared error (max. MSE) over deployed environments; as a contrast, the validation's loss adopted by \cite{subbaswamy2019preventing} fails to do so. This can explain our advantage in predicting FAQ across patient groups shown in Fig.~\ref{fig:adni-intro} (a). 

To efficiently search for the optimal subset, we define an equivalence relation between stable subsets via $d$-separation such that two equivalent subsets share the same worst-case risk. We theoretically show that compared to exhaustive searching over all subsets, searching over only equivalence classes can reduce the exponential complexity to the polynomial complexity. The effectiveness and efficiency of our methods are demonstrated by improved robustness, stability, and computation efficiency achieved on a synthetic dataset and the diagnosis of Alzheimer's disease. 

\textbf{Contributions.} To summarize, our contributions are:
\begin{enumerate}[noitemsep,topsep=0.1pt]
    \item We propose to identify the optimal subset of invariance to transfer, guided by a comprehensive minimax analysis from a causal perspective. To the best of our knowledge, this is the \emph{first} work to comprehensively study the problem of \emph{which invariance should we transfer}, in the literature of robust learning. 
    \item We define an equivalence relation between stable subsets, and accordingly propose to search over only equivalence classes. This new search algorithm can be efficiently solved in polynomial time. 
    \item We achieve better robustness and stability than others on synthetic data and Alzheimer's disease diagnosis. 
\end{enumerate}

==> icml23_paras/wang_advice/introduction_wang_xw_v3.tex <==
\vspace{-0.7cm}
\section{Introduction}
\vspace{-0.1cm}

Current machine learning systems, which are commonly deployed based on their in-distribution performance, often encounter \emph{dataset shifts} \cite{subbaswamy2019preventing} such as covariate shift, due to changes in the data generating process. When such a shift exists in deployment environments, the model may give unreliable prediction results, which can cause severe consequences in safe-critical tasks such as healthcare \citep{hendrycks2021many}. At the heart of this unreliability issue are \emph{stability} and \emph{robustness} aspects, which respectively denote the insensitivity of prediction behavior and generalization errors to dataset shifts. 

For example, consider the system deployed to predict the Functional Activities Questionnaire (FAQ) score that is commonly adopted \cite{mayo2016use} to measure the severity of Alzheimer's disease (AD). During the prediction, the system can only access biomarkers or volumes of brain regions as covariates, with demographic information anonymous for privacy consideration. However, the changes in such demographics can cause shifts in covariates. To achieve reliability for the deployed model, its prediction is desired to be stable against demographic changes, and meanwhile to be constantly accurate across all populations. For this purpose, this paper aims to find the most robust (\emph{i.e.}, minimax optimal) predictor, among the set of stable predictors across all deployed environments. 

To achieve this goal, many studies attempted to learn invariance to transfer to unseen data. Examples include ICP \cite{peters2016causal} and \citep{arjovsky2019invariant, liu2021heterogeneous, ahuja2021invariance} that assumed the prediction mechanism given causal features or representations to be invariant; or \citep{subbaswamy2019preventing, rothenhausler2021anchor} that explicitly attributed the variation to a prior selection diagram or an exogenous variable. Particularly, on the basis of \emph{sparse mechanism shift hypothesis} \cite{scholkopf2021toward} that posits the dataset shifts as the result of changes in mechanisms on a subset of covariates (called mutable set $M$) and assumes mechanisms unchanged on other variables (called stable set $S$), we can follow \cite{subbaswamy2019preventing} and references therein to intervene on variables in $M$ and obtain a set of stable predictors \cite{subbaswamy2019preventing}, each of which corresponds to a stable subset in $S$. Compared to ICP-related methods \cite{peters2016causal, buhlmann2020invariance}, such stable predictors can additionally exploit invariance from the output's effect, thus can be potentially applied to more general scenarios. However, an important question regarding robustness remains: \emph{which part of the invariance should the model transfer, in order to achieve optimal generalization ability?}

% and correspondingly call the set of variables with changed (resp. unchanged) causal mechanisms the mutable $M$ (resp. stable $S$) set

\begin{figure*}
\centering
\includegraphics[width=0.76\textwidth]{icml23_figs2/ad_results.png}
\caption{FAQ prediction in Alzheimer's disease. (a) Comparison of maximal mean square error (max. MSE) over deployed environments. (b) Max. MSE of subsets that are ranked in ascending order from left to right, respectively according to the estimated worst-case risk of our method (marked by red) and the validation loss of the surgery estimator \cite{subbaswamy2019preventing} (marked by blue). }
\vspace{-0.2cm}
\label{fig:adni-intro}
\end{figure*}

% To resolve the first problem, we adopt the \emph{sparse mechanism shift hypothesis} \cite{scholkopf2021toward} that posits the dataset shifts as the result of changes in a subset of the causal model's mechanisms, and correspondingly call the set of variables with changed (resp. unchanged) causal mechanisms the mutable $M$ (resp. stable $S$) set. Equipped with causal discovery via heterogeneous data, we can detect the mutable set and intervene on them to obtain a set of stable predictors \cite{subbaswamy2019preventing}, each of which corresponds to a stable subset in $S$. 
% Compared to ICP-related methods \cite{peters2016causal, buhlmann2020invariance}, such stable predictors can additionally exploit invariance from the output's effect, thus can be potentially applied to more general scenarios. However, an important question regarding robustness remains: \emph{which part of the invariance should the model transfer, in order to achieve optimal generalization ability?}




% Particularly, \cite{subbaswamy2019preventing,subbaswamy2020spec} causally decomposed the joint distribution into the mutable ($M$) set and the stable ($S$) set, which contains variables with changed and unchanged causal mechanisms, respectively. By intervening on $M$, they can obtain a set of stable predictors, each of which is based on a stable subset in $S$. To further find the most robust predictor, the following question remains: \emph{which subset of $S$ should the model transfer, in order to be most robust against dataset shifts?} 

%In \cite{subbaswamy2019preventing}, this optimal subset is simply taken as the one with the minimal validation loss, which lacks theoretical guarantees as the validation environment may not reflect the worst-case risk over deployed environments, as shown by Fig.~\ref{fig:adni-intro} (b). 





To answer this question, we give a comprehensive analysis from the perspective of causality. Specifically, we first provide a graphical condition that is sufficient for the whole stable set to be optimal. This condition can be easily tested via causal discovery. When this condition fails, we construct an example that counter-intuitively shows that this whole stable set, although keeps all stable information, is \textbf{NOT} the optimal one to transfer. Under these cases,
we investigate the mutable mechanisms and propose to optimize the intervention on the mutable set, in order to mimic the worst-case deployed environment. We show that such an optimization-based approach can attain the worst-case risk for each stable subset, which is crucial to select the optimal subset in a more accurate way. Back to the FAQ prediction example, Fig.~\ref{fig:adni-intro} (b) shows that our method can well reflect the maximal mean squared error (max. MSE) over deployed environments; as a contrast, the validation's loss adopted by \cite{subbaswamy2019preventing} fails to do so. This can explain our advantage in predicting FAQ across patient groups shown in Fig.~\ref{fig:adni-intro} (a). 

To efficiently search for the optimal subset, we define an equivalence relation between stable subsets via $d$-separation such that two equivalent subsets share the same worst-case risk. We theoretically show that compared to exhaustive searching over all subsets, searching over only equivalence classes can reduce the exponential complexity to the polynomial complexity. The effectiveness and efficiency of our methods are demonstrated by improved robustness, stability, and computation efficiency achieved on a synthetic dataset and the diagnosis of Alzheimer's disease. 

\textbf{Contributions.} To summarize, our contributions are:
\begin{enumerate}[noitemsep,topsep=0.1pt]
    \item We propose to identify the optimal subset of invariance to transfer, guided by a comprehensive minimax analysis from a causal perspective. To the best of our knowledge, this is the \emph{first} work to comprehensively study the problem of \emph{which invariance should we transfer}, in the literature of robust learning. 
    \item We define an equivalence relation between stable subsets, and accordingly propose to search over only equivalence classes. This new search algorithm can be efficiently solved in polynomial time. 
    \item We achieve better robustness and stability than others on synthetic data and Alzheimer's disease diagnosis. 
\end{enumerate}

==> icml23_paras/wang_advice/minimax_wang_mz_v1.tex <==
\section{Causal analysis for the optimal predictor}
\label{sec.identify}
In this section, we introduce our causal analysis to identify the minimax optimal predictor in Eq.~\ref{eq.robust}. First, in Sec.~\ref{sec.invariant}, we identify a set of stable predictors and convert the robust predictor identification into a subset selection problem. Then, in Sec.~\ref{sec.selection}, we provide minimax theories to select the optimal subset.

\subsection{Stable predictors identification}
\label{sec.invariant}

Equipped with the causal assumptions in Sec.~\ref{sec.background} especially the sparse mechanism shift hypothesis, we can identify a set of stable predictors via causal discovery and the ``do'' operator. Specifically, we first use the environmental indicator variable $E_{\text{tr}}$ with support $\mathcal{E}_{\text{tr}}$ to detect the mutable variables $\mathbf{X}_M$, with $X_i \in \mathbf{X}_M$ iff $E_{\text{tr}} \to X_i$ in the augmented graph $G_{\text{aug}}$ over $\mathbf{V}\cup E_{\text{tr}}$ \cite{huang2020causal}. Then, we consider a set of predictors by implementing the ``do'' on the detected $\mathbf{X}_M$, \emph{i.e.}, $\mathcal{F}_S:=\{f_{S^\prime}(\boldsymbol{x})|S^\prime\!\subseteq \!{S}\}, f_{S^\prime}(\boldsymbol{x})\!:=\!\mathbb{E}[Y|\boldsymbol{x}_{S^\prime}, do(\boldsymbol{x}_M)]$. Since this ``do'' operation removes the mutable causal mechanisms that generate $\mathbf{X}_M$, we have the following invariance property, which is firstly established by Prop.~$1$ in \citep{subbaswamy2019preventing}:
\begin{proposition}[Invariance property]
    For each $S^\prime \subseteq S$, the $f_{S^\prime}$ is a stable predictor.
\end{proposition}

In this regard, identifying the optimal predictor in Eq.~\ref{eq.robust} is equivalent to selecting the optimal subset $S^*$ s.t. $f^*=f_{S^*}$.


\subsection{Minimax theories for $S^*$ selection}
\label{sec.selection}

In this section, we provide minimax theories to select the optimal subset. Specifically, we first provide a graphical condition for the whole stable set to be optimal, \emph{i.e.}, $S^* = S$. When this condition is not met, we show that this whole stable set may not be optimal. To select the $S^*$ in these cases, we propose an optimization scheme that is provable to identify the worst-case risk for each subset, equipped with which we can pick up the $S^*$ as the one with minimal worst-case risk. 

In the following, we first introduce the graphical condition for $S^*=S$.
\begin{theorem}[Graphical condition for $S^*\!=\!S$]
\label{thm:graph degenerate}
Suppose Asm.~\ref{eq:assum-dag} holds. Denote $\mathbf{X}_{M}^{0}\!:=\!\mathbf{X}_{M}\cap \mathbf{Ch}(Y)$ as mutable variables in $Y$'s children, and $\mathbf{W}:=\mathbf{De}(\mathbf{X}_{M}^{0}) \backslash \mathbf{X}_M^0$ as descendants of $\mathbf{X}_{M}^{0}$. Then, we have $S^*=S$ if $Y$ does not point to any vertex in $\mathbf{W}$.
\end{theorem}

Indeed, a similar result has been established in \cite{subbaswamy2019preventing}, \emph{i.e.}, the degeneration condition for $S^*=S$, which states that the $S$ is optimal when the interventional distribution $P(Y|\mathbf{X}_S,do(\boldsymbol{x}_M))$ can degenerate to a conditional distribution $P(Y|\mathbf{X}^\prime)$ for some $\mathbf{X}^\prime \subseteq \mathbf{X}$. However, as we will show later, our graphical condition not only has the same power as the degeneration condition; but also enjoys a better intuition from the perspective of graph structure, thus facilitating an easy testing approach via causal discovery.

\begin{proposition}
    The interventional distribution can degenerate if and only if the graphical condition in Thm.~\ref{thm:graph degenerate} holds.
\end{proposition}

To understand this equivalence, note that if $Y \not \to \mathbf{W}$, we can use the inference rules \citep{pearl2009causality} to remove the ``do" in $P(Y|\mathbf{X}_S, do(\boldsymbol{x}_M))$ and degenerate it into $P(Y|\mathbf{X}\backslash(\mathbf{X}_M^0 \cup \mathbf{De}(\mathbf{X}_M^0)))$. On the contrary, if $Y \to \mathbf{W}$, there will a collider in $\mathbf{W}$ in some paths between $Y$ and $\mathbf{X}_M^0$, making it incapable to remove the ``do''. For illustration, consider the causal graph that is shown in Fig.~\ref{fig: example graphical condition} (a), where $Y \not\to \mathbf{W}$. We thus have {\small $Y\ind_{G_{\overline{X_M}}}\! X_1,X_M|X_2$} and hence  {\small $P(Y|X_1,X_2,do(x_M))=P(Y|X_2)$}.  In contrast, for the causal graph shown in Fig.~\ref{fig: example graphical condition} (b), the collider $X_1$ causes {\small $Y \not \ind_{G_{\overline{X_M}}} X_M | X_1$} and prevents the removing of the ``do'' in {\small $P(Y|X_1,do(x_M))$}.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{icml23_figs2/thm3.1_example.pdf}
    \caption{Illustration of the graphical condition in Thm.~\ref{thm:graph degenerate}. Stable and mutable variables are respectively marked blue and red. In both (a) and (b), we have $\mathbf{X}_M^0=\{X_M\}, \mathbf{W}=\{X_1\}$.}
    \label{fig: example graphical condition}
\end{figure}


Compared to exhaustively running the inference rules to check the degeneration condition, our graphical condition can be effectively tested via causal discovery. Specifically, we first learn the skeleton of $G$, followed by detecting $\mathbf{X}_M^0$ and $\mathbf{W}$ by leveraging the heterogeneity in $\mathcal{E}_{\mathrm{tr}}$ \cite{huang2020causal}. Finally, we have $Y \to \mathbf{W}$ if and only if $Y$ is adjacent to a vertex in $\mathbf{W}$ since $\mathbf{W} \subseteq \mathbf{De}(Y)$ by the definition of $\mathbf{W}$. The involved causal structures, \emph{i.e.}, the skeleton of $G$, $\mathbf{X}_M^0$, and $\mathbf{W}$ are identifiable according to the following proposition:

\begin{proposition}
    \label{prop.thm3.2 justifiability}
    Under Asm.~\ref{eq:assum-dag}-\ref{assum:e-train}, we have that the skeleton of $G$, $\mathbf{X}_M^0$, and $\mathbf{W}$ are identifiable.
\end{proposition}

On the other hand, when this condition is not met, we show that the whole stable set may not be optimal. To be specific, we construct an example with the DAG of Fig.~\ref{fig: example graphical condition} (b), in which $Y, X_M, X_{1}$ are binary variables. We then have the following result:
\begin{claim}
\label{prop:counter}
There exists $P(Y)$ and $P(X_{1}|X_M, Y)$, such that $f_{S}(\boldsymbol{x}):=\mathbb{E}[Y|x_{1},do(x_M)]$ has larger worst-case risk than $f_{\emptyset}(\boldsymbol{x}) := \mathbb{E}[Y|do(x_M)]$: 
\begin{align*}
    \max_{P^e} \mathbb{E}_{P^e}[(Y-f_S(\boldsymbol{x}))^2] > \max_{P^e} \mathbb{E}_{P^e}[(Y-f_\emptyset(\boldsymbol{x}))^2].
\end{align*}
\end{claim}

\begin{remark}
This result seems surprising as intuitively the whole stable set should be optimal since it fully exploits the stable information, according to existing minimax results in \cite{peters2016causal, rojas2018invariant}. To explain, we should note that these results are built on \emph{conditional} distributions, where one can construct a $P^e$ to make any other predictor having a larger quadratic loss than $f_S$. However, when the \emph{interventional} distribution can not degenerate, such a construction is generally not feasible. Please refer to Appx.~\ref{sec: counter example appendix new} for a more detailed analysis. 
\end{remark}

Under the general cases where the whole stable set may not be optimal, it remains unknown that \emph{which subset of stable information is the optimal one to transfer?} To answer this question, we propose to estimate the worst-case risk $\mathcal{R}_{S^\prime}\!:=\!\max_{e \in \mathcal{E}} \mathbb{E}_{P^e}[\left(Y \!-\! f_{S^\prime}(\boldsymbol{x})\right)^2]$ for each subset $S^\prime$; then the $S^*$ corresponds to the subset with minimal $\mathcal{R}$. To estimate $\mathcal{R}_{S^\prime}$ for each $S^\prime \subseteq S$, we consider a distribution family $\{P_h\}_{h}$, where $h$ maps from $\mathcal{P}a(\mathcal{X}_M)$ to $\mathcal{X}_M$ and $P_h\! :=\! P(Y,\mathbf{X}_S| do(\boldsymbol{x}_M\!=\!h(\boldsymbol{pa}(\boldsymbol{x}_M)))$. This distribution set keeps the invariant mechanisms of $Y$ and $\mathbf{X}_S$ unchanged while allowing the $\mathbf{X}_M$ given their parents to vary arbitrarily, which can well mimic the distributional shifts among deployed environments in $\{P^e\}_{e \in \mathcal{E}}$. Particularly, we show that the worst-case risk $\mathcal{R}_{S^\prime}$ can be attained at some $P_h$, where $h$ is a Borel measurable function. Formally, denote $\mathcal{B}$ as the Borel function set, we have: 

\begin{theorem}[Identify the worst-case risk]
\label{thm:min-max}
Let $\mathcal{L}_{S^\prime}:=\max_{h \in  \mathcal{B}}\mathbb{E}_{P_h}[(Y \!-\! f_{S^\prime}(\boldsymbol{x}))^2]$ be the maximal population loss over $\{P_h\}_{h \in \mathcal{B}}$ for subset $S^\prime$. Then, we have $\mathcal{L}_{S^\prime}=\mathcal{R}_{S^\prime}$ for each $S^\prime \subseteq S$. Therefore, we have $S^*= \mathop{\mathrm{argmin}}_{S^\prime \subseteq S} \mathcal{L}_{S^\prime}$.
\end{theorem}


This result inspires the following optimization problem over the function $h \in  \mathcal{B}$ to estimate $\mathcal{R}_{S^\prime}$: 
\begin{align*}
    \max_{h \in  \mathcal{B}} \mathcal{L}_{S^\prime}(h) := \mathbb{E}_{P_h}[(Y \!-\! f_{S^\prime}(\boldsymbol{x}))^2],
\end{align*}
as the optimality of which is assured to attain $\mathcal{R}_{S^\prime}$. To implement, we parameterize the $h:\mathcal{P}a(\mathcal{X}_M)\!\to\!\mathcal{X}_M$ with a multilayer perceptron (MLP) for optimization, due to the ability of MLP to approximate any Borel function \cite{hornik1989multilayer}. To show the tractability of this optimization, we have the following identifiability result for $\mathcal{L}_{S^\prime}(h)$. 


\begin{proposition}
	\label{prop.thm3.3 justifiability}
	Under Asm.~\ref{eq:assum-dag}-\ref{assum:e-train}, the  $P_h$, $f_{S^\prime}$, and hence $\mathcal{L}_{S^\prime}(h)$ are identifiable. 
\end{proposition}


%\textbf{Summary.} Our results answer the two questions raised in Sec.~\ref{sec.background}. Specifically, Thm.~\ref{thm:graph degenerate} provides an equivalent but a more intuitive graphical condition for $S^*=S$; while Thm.~\ref{thm:min-max} motivates an optimization-based approach to identify the optimal subset $S^*$ with theoretical guarantees. 






==> icml23_paras/wang_advice/preliminary_wang_mz_v1.tex <==
\section{Problem setting and notation} 
\label{sec.background}

We consider the supervised regression scenario, where the system includes a target variable $Y \!\in\! \mathcal{Y}$, covariates $\mathbf{X}\!:=\! [X_1,...,X_d] \!\in\! \mathcal{X}$, and data collected from heterogeneous environments. In practice, different ``environments" can refer to different groups of subjects or different experimental settings. We denote the set of training environments as $\mathcal{E}_{\mathrm{tr}}$, and the broader set of environments for deployment as $\mathcal{E}$. We denote $E$ as the environmental indicator variable with support $\mathcal{E}$. Our data are collected from multiple training environments $\{\mathcal{D}_{e}\}_{e\in\mathcal{E}_{\text{tr}}}$, where ${\mathcal{D}_{e}\!:=\!\{(\boldsymbol{x}_{k}^e, {y}_{k}^e)\}_{k=1}^{n_e} \sim_{i.i.d} P^e(\mathbf{X},Y)}$ are data collected from environment $e$. In a directed acyclic graph (DAG) $G$, we denote the parents, children, neighbors, and descendants of the vertex $V_i$ as $\mathbf{Pa}(V_i)$, $\mathbf{Ch}(V_i)$, $\mathbf{Neig}(V_i)$, and $\mathbf{De}(V_i)$, respectively. We denote $G_{\overline{V_i}}$ as the graph attained via deleting all arrows pointing into $V_i$. 

Our goal is to find the most robust predictor $f^*$ among stable predictors with data from $\mathcal{E}_{\mathrm{tr}}$. Here, we say a predictor $f \!:\! \mathcal{X} \to \mathcal{Y}$ is stable if it is independent of $E$. We denote the set of stable predictors as $\mathcal{F}_S$. For robustness, a commonly adopted measurement \cite{peters2016causal,ahuja2021invariance} is to investigate a predictor's worst-case risk, which provides a safeguard for deployment in unseen environments. That is, we want $f^*$ to have the following minimax property:
\begin{align}
    f^{*}(\boldsymbol{x})=\mathop{\mathrm{argmin}}\limits_{f \in \mathcal{F}_S}        \max_{e\in\mathcal{E}}
    \mathbb{E}_{P^e}[(Y-f(\boldsymbol{x}))^2].
\label{eq.robust}
\end{align}
Next, we introduce some basic assumptions, which are commonly made in causal inference and learning \cite{pearl2009causality,spirtes2000causation,arjovsky2019invariant}.
\begin{assumption}[Causal Graphical Model (CGM)]
\label{eq:assum-dag}
We assume that $P^e(\mathbf{X},Y)$ is entailed by an \emph{unknown} DAG $G$ over $\mathbf{V}$ for all $e \in \mathcal{E}$, where $\mathbf{V}:= \mathbf{X} \cup Y$. Each variable $V_i \in \mathbf{V}$ is generated via a structural equation $V_i=g^e_{i}(\mathbf{Pa}({V_i}), U_i)$, where $U_i$ denotes an exogenous variable. We assume  
each $g^e_{i}$ is continuous and bounded. Each edge $V_i \to V_j$ in $G$ means $V_i$ is a direct causal of $V_j$. Besides, we assume the model is Markovian which states that $\mathbf{A} \ind_G \mathbf{B} | \mathbf{Z} \Rightarrow \mathbf{A} \ind \mathbf{B} | \mathbf{Z}$ for disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, where $\ind_G$ denotes \emph{d}-separation in $G$. 
\end{assumption}

According to the Causal Markov Condition theorem \cite{pearl2009causality}, the joint distribution can be causally factorized into $P^e(\mathbf{V})=\prod_i P^e(V_i|\mathbf{Pa}(V_i)))$, where $P^e(V_i|\mathbf{Pa}(V_i)))$ denotes the causal factor of $V_i$. Based on the principle of independent causal mechanisms \cite{scholkopf2021toward}, these causal factors are autonomous of each other. On the basis of this, the interventional distribution is defined as $P(\mathbf{V}|do(V_i\!=\!v_i)):=\prod_{j \neq i} P^e(V_j|\mathbf{Pa}(V_j)))\mathbbm{1}_{V_i=v_i}$. Here $do(V_i\!=\!v_i)$ means lifting $V_i$ from its original causal mechanism $g_{i}(\mathbf{Pa}({V_i}), U_i)$ and setting it to a constant value $v_i$. 

In addition to the Markovian assumption, we also assume the causal faithfulness assumption, which enables us to infer the graph structure from probability properties:

\begin{assumption}[Causal faithfulness]
\label{asm:faithfulness}
    For disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, $\mathbf{A} \ind \mathbf{B} | \mathbf{Z} \Rightarrow \mathbf{A} \ind_G \mathbf{B} | \mathbf{Z}$. 
\end{assumption}


\textbf{Sparse mechanism shift hypothesis across $\mathcal{E}$.} To build the connection between seen and unseen environments for transfer, we adopt the \emph{sparse mechanism shift hypothesis} \cite{scholkopf2021toward}, \emph{i.e.}, distributional shifts in $P^e(\mathbf{X},Y)$ are the results of changes in only a subset of causal factors. Formally, 
\begin{align}
\label{eq: causal factorization}
    & P^e(\mathbf{X},Y) = P(Y|\mathbf{Pa}(Y)) \prod_{i \in S} P\left(X_i|\mathbf{Pa}(X_i)\right) \nonumber \\
    & \prod_{i \in M} P^e(X_i|\mathbf{Pa}(X_i)), d_S:=|S|, d_M:=|M|,
\end{align}
where $S, M$ respectively denote stable and mutable sets such that each $X_i \in \mathbf{X}_S$ has invariant causal mechanism $P(X_i|\mathbf{Pa}(X_i))$; while the mechanism of each $X_i \in \mathbf{X}_M$ varies across $\mathcal{E}$. Correspondingly, we call $\mathbf{X}_S$ as stable variables and $\mathbf{X}_M$ as mutable variables. In addition to $\mathbf{X}_S$, we also assume the causal mechanism of $Y$ keeps invariant across $\mathcal{E}$, as widely adopted by the existing literature \cite{arjovsky2019invariant,sun2021recovering,mitrovic2021representation}.


To recover the $\mathbf{X}_M$ from the training distribution, it is also necessary to assume that $\mathcal{E}_{\mathrm{tr}}$ can reflect the mutation of $\mathbf{X}_M$ across $\mathcal{E}$. This is formally stated as follows:
\begin{assumption}[Consistent heterogeneity]
\label{assum:e-train}
For each $X_i \in \mathbf{X}_M$, there exists two different environments $e, e^\prime \in \mathcal{E}_{\mathrm{tr}}$ such that $P^{e}(X_i|\mathbf{Pa}(X_i)) \neq P^{e^\prime}(X_i|\mathbf{Pa}(X_i))$.
\end{assumption}



==> icml23_paras/wang_advice/preliminary_wang_xw_v3.tex <==
\vspace{-0.2cm}
\section{Preliminary} 
\label{sec.background}
\vspace{-0.2cm}

We consider the supervised regression scenario, where the system includes a target variable $Y \!\in\! \mathcal{Y}$, covariates $\mathbf{X}\!:=\! [X_1,...,X_d] \!\in\! \mathcal{X}$, and data collected from heterogeneous environments. In practice, different ``environments" can refer to different groups of subjects or different experimental settings. We denote the set of training environments as $\mathcal{E}_{\mathrm{tr}}$, and the broader set of environments for deployment as $\mathcal{E}$. We denote $E$ as the environmental indicator variable with support $\mathcal{E}$. Our data are collected from multiple training environments $\{\mathcal{D}_{e}\}_{e\in\mathcal{E}_{\text{tr}}}$, where ${\mathcal{D}_{e}\!:=\!\{(\boldsymbol{x}_{k}^e, {y}_{k}^e)\}_{k=1}^{n_e} \sim_{i.i.d} P^e(\mathbf{X},Y)}$ are data collected from environment $e$. In a directed acyclic graph (DAG) $G$, we denote the parents, children, neighbors, and descendants of the vertex $V_i$ as $\mathbf{Pa}(V_i)$, $\mathbf{Ch}(V_i)$, $\mathbf{Neig}(V_i)$, and $\mathbf{De}(V_i)$, respectively. We denote $G_{\overline{V_i}}$ as the graph attained via deleting all arrows pointing into $V_i$. 

Our goal is to find the most robust predictor $f^*$ among stable predictors with data from $\mathcal{E}_{\mathrm{tr}}$. Here, we say a predictor $f \!:\! \mathcal{X} \to \mathcal{Y}$ is stable if it is independent of $E$. We denote the set of stable predictors as $\mathcal{F}_S$. For robustness, a commonly adopted measurement \cite{peters2016causal,ahuja2021invariance} is to investigate a predictor's worst-case risk, which provides a safeguard for deployment in unseen environments. That is, we want $f^*$ to have the following minimax property:
\begin{align}
    f^{*}(\boldsymbol{x})=\mathop{\mathrm{argmin}}\limits_{f \in \mathcal{F}_S}        \max_{e\in\mathcal{E}}
    \mathbb{E}_{P^e}[(Y-f(\boldsymbol{x}))^2].
\label{eq.robust}
\end{align}
Next, we introduce some basic assumptions, which are commonly made in causal inference and learning \cite{pearl2009causality,spirtes2000causation,arjovsky2019invariant}.
\begin{assumption}[Structural Causal Model]
\label{eq:assum-dag}
We assume that $P^e(\mathbf{X},Y)$ is entailed by an \emph{unknown} DAG $G$ over $\mathbf{V}$ for all $e \in \mathcal{E}$, where $\mathbf{V}:= \mathbf{X} \cup Y$. Each variable $V_i \in \mathbf{V}$ is generated via a structural equation $V_i=g^e_{i}(\mathbf{Pa}({V_i}), U_i)$, where $U_i$ denotes an exogenous variable. We assume  
each $g^e_{i}$ is continuous and bounded. Each edge $V_i \to V_j$ in $G$ means $V_i$ is a direct causal of $V_j$. Besides, we assume the model is Markovian which states that $\mathbf{A} \ind_G \mathbf{B} | \mathbf{Z} \Rightarrow \mathbf{A} \ind \mathbf{B} | \mathbf{Z}$ for disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, where $\ind_G$ denotes \emph{d}-separation in $G$. 
\end{assumption}

According to the Causal Markov Condition theorem \cite{pearl2009causality}, the joint distribution can be causally factorized into $P^e(\mathbf{V})=\prod_i P^e(V_i|\mathbf{Pa}(V_i)))$, where $P^e(V_i|\mathbf{Pa}(V_i)))$ denotes the causal factor of $V_i$. Based on the principle of independent causal mechanisms \cite{scholkopf2021toward}, these causal factors are autonomous of each other. On the basis of this, the interventional distribution is defined as $P(\mathbf{V}|do(V_i\!=\!v_i)):=\prod_{j \neq i} P^e(V_j|\mathbf{Pa}(V_j)))\mathbbm{1}_{V_i=v_i}$. Here $do(V_i\!=\!v_i)$ means lifting $V_i$ from its original causal mechanism $g_{i}(\mathbf{Pa}({V_i}), U_i)$ and setting it to a constant value $v_i$. 

In addition to the Markovian assumption, we also assume the causal faithfulness assumption, which enables us to infer the graph structure from probability properties:

\begin{assumption}[Causal faithfulness]
\label{asm:faithfulness}
    For disjoint vertex sets $\mathbf{A},\mathbf{B},\mathbf{Z} \subseteq \mathbf{V}$, $\mathbf{A} \ind \mathbf{B} | \mathbf{Z} \Rightarrow \mathbf{A} \ind_G \mathbf{B} | \mathbf{Z}$. 
\end{assumption}


\textbf{Sparse mechanism shift hypothesis across $\mathcal{E}$.} To build the connection between seen and unseen environments for transfer, we adopt the \emph{sparse mechanism shift hypothesis} \cite{scholkopf2021toward}, \emph{i.e.}, distributional shifts in $P^e(\mathbf{X},Y)$ are the results of changes in only a subset of causal factors. Formally, 
\begin{align}
\label{eq: causal factorization}
    & P^e(\mathbf{X},Y) = P(Y|\mathbf{Pa}(Y)) \prod_{i \in S} P\left(X_i|\mathbf{Pa}(X_i)\right) \nonumber \\
    & \prod_{i \in M} P^e(X_i|\mathbf{Pa}(X_i)), d_S:=|S|, d_M:=|M|,
\end{align}
where $S, M$ respectively denote stable and mutable sets such that each $X_i \in \mathbf{X}_S$ has invariant causal mechanism $P(X_i|\mathbf{Pa}(X_i))$; while the mechanism of each $X_i \in \mathbf{X}_M$ varies across $\mathcal{E}$. Correspondingly, we call $\mathbf{X}_S$ as stable variables and $\mathbf{X}_M$ as mutable variables. In addition to $\mathbf{X}_S$, we also assume the causal mechanism of $Y$ keeps invariant across $\mathcal{E}$, as widely adopted by the existing literature \cite{arjovsky2019invariant,sun2021recovering,mitrovic2021representation}.


To recover the $\mathbf{X}_M$ from the training distribution, it is also necessary to assume that $\mathcal{E}_{\mathrm{tr}}$ can reflect the mutation of $\mathbf{X}_M$ across $\mathcal{E}$. This is formally stated as follows:
\begin{assumption}[Consistent heterogeneity]
\label{assum:e-train}
For each $X_i \in \mathbf{X}_M$, there exists two different environments $e, e^\prime \in \mathcal{E}_{\mathrm{tr}}$ such that $P^{e}(X_i|\mathbf{Pa}(X_i)) \neq P^{e^\prime}(X_i|\mathbf{Pa}(X_i))$.
\end{assumption}


\textbf{Stable predictor set $\mathcal{F}_S$ via $do(\mathbf{X}_M)$.} On the basis of Eq.~\eqref{eq: causal factorization}, the recently proposed graph-surgery estimators \cite{subbaswamy2019preventing, subbaswamy2020spec} obtained a \emph{stable predictor} set $\mathcal{F}_S:=\{f_{S^\prime}(\boldsymbol{x})|S^\prime\!\subseteq \!{S}\}, f_{S^\prime}(\boldsymbol{x})\!:=\!\mathbb{E}[Y|\boldsymbol{x}_{S^\prime}, do(\boldsymbol{x}_M)]$ over the interventional distribution, by intervening on mutable variables $\mathbf{X}_M$. Compared to \cite{peters2016causal, rojas2018invariant} that only exploits causal features, these stable predictors in $\mathcal{F}_S$ can additionally leverage the invariance from $Y$'s effect, enabling them to be potentially applied to more general scenarios where the mechanism of $Y$'s cause and effect are both allowed to be invariant \cite{huang2006correcting, zhang2013domain, arjovsky2019invariant}. 

% we first detect mutable variables $\mathbf{X}_M$ by leveraging the heterogeneity from multiple domains \cite{huang2020causal}; then we intervene on $\mathbf{X}_M$ to obtain the \emph{stable predictor} set $\mathcal{F}_S:=\{f_{S^\prime}(\boldsymbol{x})|S^\prime\!\subseteq \!{S}\}, f_{S^\prime}(\boldsymbol{x})\!:=\!\mathbb{E}[Y|\boldsymbol{x}_{S^\prime}, do(\boldsymbol{x}_M)]$ over the interventional distribution, following recently proposed graph surgery estimator \cite{subbaswamy2019preventing,subbaswamy2020spec}.

% we can intervene on mutable variables $\mathbf{X}_M$ to obtain 

However, regarding robustness, it still remains open to which predictor among $\mathcal{F}_S$ is min-max optimal. As identifying $f^* \in \mathcal{F}_S$ is equivalent to selecting the optimal stable subset $S^* \subseteq S$ such that $f_{S^*}=f^*$, it turns to the following question: \emph{which subset of $S$ should we transfer in terms of out-of-distribution robustness?} 




==> icml23_paras/wang_advice/related_works_wang_mz_v1.tex <==
\section{Related works}
\textbf{Causality-based domain generalization.} There are emerging works that consider the domain generalization problems from a causal perspective. One line of works \cite{arjovsky2019invariant,liu2021heterogeneous,ahuja2021invariance,ausset2022empirical} promoted invariance as a key surrogate feature of causation where the causal graph is mode of a motivation. Another line of works \cite{peters2016causal,rojas2018invariant,gamella2020active,martinet2022variance} assumed and used the invariance assumption regarding the causal mechanism. The works most relevant to us are \citep{subbaswamy2019preventing,rothenhausler2021anchor}, which also proposed causal attribution of the distributional shifts and obtained invariance by removing the shifted features. Particularly, the \citep{subbaswamy2019preventing} assumed the mutable set to be known and removed its mutation via intervention. However, they did not provide any theoretical analysis for robust subset selection.

\textbf{Optimization-based domain generalization.}  Recently, there are works \cite{sinha2018certifiable,sagawa2019distributionally,wu2022generalization,slowik2022distributionally} that viewed domain generalization as an optimization problem. These methods formulated the objective of robustness and directly optimized the predictor for generalizability. To achieve optimization convenience, they usually constrained the dataset shifts to a limited extend, which limits their application in the real world. In contrast, we adopt optimization to estimate the worst-case error for each stable predictor, then select the optimal one via comparison. Benefit from the causal interpretation of dataset shifts, our method can achieve consistent estimation and hence optimal selection, even when the dataset is allowed to shift arbitrarily.

\textbf{Causal discovery in heterogeneous data.} Our work benefits from the recent progress in heterogeneous causal discovery \cite{ghassami2018multi,huang2020causal,perry2022causal}, a field that seeks to learn causal graphs with data from multiple environments. However, unlike causal discovery that seeks to recover as many as causal structures, we are only interested in the causal structures that aid minimax analysis and robust subset selection.
